Harness-1: Reinforcement Learning for Search Agents with State-Externalizing Harnesses

Search agents are often trained as policies over growing transcripts: the model must decide how to search while also remembering what it has seen, which evidence is useful, which constraints remain open, and which claims have actually been checked. We argue that this formulation puts too much routine state management inside the policy: reinforcement learning is forced to optimize both semantic search decisions and recoverable bookkeeping that the environment can maintain more reliably. We introduce Harness-1, a 20B search agent (retrieval subagent) trained with reinforcement learning inside a stateful search harness. The harness maintains environment-side working memory, including a candidate pool, an importance-tagged curated set, compact evidence links, verification records, compressed and deduplicated observations, and budget-aware context rendering. The policy retains the semantic decisions: what to search, which documents to keep or discard, what to verify, and when to stop. Across eight retrieval benchmarks spanning web, finance, patents, and multi-hop QA, Harness-1 achieves 0.730 average curated recall, outperforming the next strongest open search subagent by +11.4 points and remaining competitive with much larger frontier-model searchers. Its gains are especially strong on held-out transfer benchmarks, suggesting that reinforcement learning over explicit search state can produce retrieval behaviors that generalize beyond the training domains. Our code is available at https://github.com/pat-jj/harness-1.

==> case_study_bc643_long.tex <==
\subsection{Full Trajectory A: BrowseComp+ Query 643}
\label{app:case-bc643}

\begin{promptbox}{browsecompplus query 643}
\textbf{Query.} An agent is not indicated for patients who weigh 30 kg or are 10 years old. It can be taken via oral administration, and one of the side effects reported is nausea. A study from 2022 mentions that its half-life is less than 10 hours and that the liver primarily eliminates it. The study is authored by two people, published in December, and features 31 references. The application for tablets containing the agent was received on March 23, and it was approved eight months later by a letter. What is the full name (as mentioned in the letter) of the Regulatory Project Manager to be called in case of any questions?\\[2pt]
\textbf{Gold answer.} Alicia Moruf\\[2pt]
\textbf{Trajectory.} 18 turns, tool diversity $6$, curated recall $1.0$, final-answer recall $1.0$.
\end{promptbox}

\paragraph{Color legend.}
\CaseTool{toolFanout}{fan\_out\_search} \CaseTool{toolSearch}{search\_corpus} \CaseTool{toolGrep}{grep\_corpus} \CaseTool{toolRead}{read\_document} \CaseTool{toolReview}{review\_docs} \CaseTool{toolCurate}{curate} \CaseTool{toolVerify}{verify} \CaseTool{toolStop}{end\_search}

\paragraph{Clipping rule.}
The transcript below preserves reasoning, tool calls, parameters, tool-return metadata, and harness state snapshots. Only individual document-text blocks longer than 2600 characters are shortened, with a marker showing the omitted length.

\begin{trajectorylisting}{toolNeutral}{System prompt used for this trajectory}
You are a retrieval subagent. Find and retrieve the most relevant documents from a corpus to help answer a question. You do NOT answer questions yourself - you only find relevant documents.

<query>
An agent is not indicated for patients who weigh 30 kg or are 10 years old. It can be taken via oral administration, and one of the side effects reported is nausea. A study from 2022 mentions that its half-life is less than 10 hours and that the liver primarily eliminates it. The study is authored by two people, published in December, and features 31 references. The application for tablets containing the agent was received on March 23, and it was approved eight months later by a letter. What is the full name (as mentioned in the letter) of the Regulatory Project Manager to be called in case of any questions?
</query>

**Available Tools:**
- **fan_out_search**(queries): Run up to 5 diverse queries in parallel.
- **search_corpus**(query): Single semantic + keyword search.
- **grep_corpus**(pattern): Exact regex pattern matching on the corpus. Use for specific names, dates, numbers, or exact phrases.
- **read_document**(doc_id): Read a document's full content. Use liberally - seeing full text reveals connections that snippets miss.
- **review_docs**(doc_ids): Re-read previously-found documents from memory (free, no corpus call).
- **curate**(add_ids, remove_ids, importance): Update your curated set (max 30 docs). These are your final output.
- **verify**(doc_ids, claim): Check if docs support a specific claim. Use before tagging as very_high.
- **end_search**(reasoning): Submit your curated set and conclude.

**Context:**
Your context has two parts:
1. **Working Memory** - curated set with snippets, document pool with snippets, and search history.
2. **Recent Turns** - full detail of your last 5 actions and results.

**Two-Tier Memory:**
- Your Working Memory shows doc IDs + brief snippets for ALL previously found docs.
- Use **review_docs** to re-read the full text of any document from memory without re-searching.
- This is useful when you want to revisit a doc you found earlier.

**Step 1 - Decompose the Query:**
Before your first search, identify the key constraints in the query (entities, dates, relationships, distinctive facts). Use the most specific/unique constraint for your first search.

**Step 2 - Core Loop (ALWAYS follow this rhythm):**
1. **Search** - use fan_out_search, search_corpus, or grep_corpus.
2. **Curate immediately** - after EVERY search, call curate to add ALL plausibly relevant docs from the results. Do NOT do two searches in a row without curating in between.
3. **Repeat** - search a different angle, then curate again.
4. **Refine** - use review_docs or read_document to revisit docs, then curate to adjust.
5. **End** - call end_search when you've thoroughly covered the query.

You have up to **35 turns**. Use them - thorough coverage matters more than speed. Don't end early if there are unexplored angles.

The search -> curate rhythm is critical. Results are freshest right after a search. If you delay curation, those results scroll out of your recent context and you lose the detail needed to decide relevance.

**Search Strategy:**
- Keep queries SHORT (5-12 words). Vary angles - don't repeat similar queries.
- **NEVER repeat queries** from your search history. Use completely different wording.
- **Decompose complex queries** into distinct searchable facets. Search each facet separately.
- **Use grep_corpus** for specific names, dates, numbers, codes, or exact phrases from the query. grep often finds what semantic search misses.
- **Use read_document liberally** - full text reveals connections that snippets hide. If a doc partially matches, read it fully. High-recall agents read more documents.

**Curation Strategy:**
- **Curate aggressively** - add ALL plausibly relevant docs. Include borderline docs. It's ALWAYS better to over-curate than under-curate. Aim for 3-8 adds per curate call.
- **Never remove** docs unless you are certain they are completely irrelevant after reading their full text.
- Keep analysis concise (2-3 paragraphs max). Focus on what to do next.

**Backtracking - Critical Reasoning Skill:**
When you notice signs of being stuck, you MUST backtrack in your reasoning:
- **Stale pool**: If your last 2-3 searches added few or no new docs, STOP. In your reasoning, explicitly state: "My current search angle is exhausted. Let me rethink." Then try a completely different query decomposition.
- **Re-reading loop**: If you find yourself reading/reviewing the same docs repeatedly, STOP. Reason about what specific information you're missing and search for it directly.
- **Wrong entity**: If results consistently don't match, question your assumptions. The query may require interpreting an entity differently (e.g., a person's maiden name, an alternate spelling, a related entity).
- **Missed facet**: Re-read the query carefully. Identify any constraint you haven't explicitly searched for yet.

Backtracking is a REASONING step: in your analysis, explain (1) what isn't working, (2) why, and (3) your new strategy. Then act on it.

**Importance Tagging (v8d):** When you call `curate`, tag each added doc with an `importance` level in {very_high, high, fair, low}. Rules:
  - very_high: you have VERIFIED the doc directly answers the query (ideally after a `verify` call).
  - high: strongly relevant, hits most query constraints.
  - fair: plausible but not confirmed (default tag if omitted).
  - low: marginal; will be evicted first when the set is full.
The curated set is capped at 30 - when full, the lowest-importance docs are evicted first to make room for higher-tagged ones.

**Auto-populate (v8d):** After your first successful search, the top-ranked 8 docs are AUTOMATICALLY added to your curated set at `fair` importance. Your job is NOT to re-add them - instead, promote the good ones to `high`/`very_high` and REMOVE the bad ones. This is subtractive curation.

**Evidence Graph (v8d):** The Working Memory shows `[Evidence Graph]` - entities (names, dates, years) and which docs they appear in. Bridge entities (in multiple docs) are high-value signals. Singleton entities (in only 1 doc) often indicate gaps - consider follow-up searches for related entities.

**Verify tool (v8d):** Use `verify(doc_ids, claim)` BEFORE tagging docs as `very_high` on multi-constraint queries. It returns yes/no for each doc, letting you confirm a doc actually satisfies ALL criteria rather than just one.

**Context budget (v8d):** Each observation ends with `[Context: X/Y]`. When X/Y is above 75%, wrap up your search within 2-3 more turns. When above 90%, call `end_search` NOW.

\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Top-level trajectory fields}
{
  "query_id": "643",
  "query_text": "An agent is not indicated for patients who weigh 30 kg or are 10 years old. It can be taken via oral administration, and one of the side effects reported is nausea. A study from 2022 mentions that its half-life is less than 10 hours and that the liver primarily eliminates it. The study is authored by two people, published in December, and features 31 references. The application for tablets containing the agent was received on March 23, and it was approved eight months later by a letter. What is the full name (as mentioned in the letter) of the Regulatory Project Manager to be called in case of any questions?",
  "dataset": "browsecompplus",
  "curated_ids": [
    "59631",
    "66387",
    "97801",
    "25814",
    "15546",
    "50858",
    "83797",
    "17183",
    "73877",
    "72434"
  ],
  "curated_importance": {
    "59631": "high",
    "66387": "low",
    "97801": "low",
    "25814": "high",
    "15546": "fair",
    "50858": "fair",
    "83797": "low",
    "17183": "high",
    "73877": "fair",
    "72434": "low"
  },
  "evidence_graph": {
    "entity_to_docs": {},
    "doc_to_entities": {}
  },
  "reward": 3.0384615384615383,
  "metrics": {
    "recall": 1.0,
    "precision": 0.4,
    "f_beta": 0.7692307692307692,
    "final_answer_recall": 1.0,
    "final_answer_found": 1.0,
    "trajectory_recall": 1.0,
    "trajectory_fa_recall": 1.0,
    "final_answer_bonus": 1.0,
    "fa_dense_reward": 1.2000000000000002,
    "fa_miss_gap": 0.0,
    "fa_miss_penalty": 0.0,
    "pool_curated_gap": 0.0,
    "gap_penalty": 0.0,
    "turn_penalty": 0.0,
    "pre_penalty_reward": 3.0384615384615383,
    "num_curated_docs": 10.0,
    "used_curate": 1.0,
    "total_curate_calls": 9.0,
    "curate_rate": 0.5,
    "curate_rate_bonus": 0.0,
    "tool_diversity": 6.0,
    "tool_diversity_bonus": 0.0,
    "num_turns": 18,
    "final_reward": 3.0384615384615383,
    "no_error": 1.0,
    "max_turns_reached": 0.0
  }
}
\end{trajectorylisting}

\subsubsection*{Turn 0: \CaseTool{toolSearch}{search\_corpus}}
\begin{trajectorylisting}{toolNeutral}{Turn 0 model reasoning}
Key constraints: agent not indicated for patients >=30kg or 10y; oral administration; side effect nausea; 2022 study mentions half-life <10h, primarily liver elimination; study by two authors, December, 31 references; tablet application received 23 Mar; approved 8 months later via letter identifying a Regulatory Project Manager. Likely a US FDA approval letter for an oral drug for weight >=30kg/age >=10y contraindication. The unique medicine clue is the age/weight contraindication plus nausea side effect. Search angle: distinct clinical label and side effect plus half-life/liver elimination trait.
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 0 tool call(s)}
[
  {
    "tool": "search_corpus",
    "params": {
      "query": "oral contraindicated for under 30 kg age 10 nausea half-life less than 10 hours liver eliminated 2022 study December 31 references FDA approval letter Regulatory Project Manager March 23 seventeen Feb 2023 app tablets received March 23 approved eight months letter"
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 0 tool return 0}
RETURN 0.text:

# DOCUMENT ID: 59631_0 (743 tokens) 
CENTER FOR DRUG EVALUATION AND RESEARCH Approval Package for: APPLICATION NUMBER: 215596Orig1s000 Trade Name: LIVTENCITY oral tablets Generic or Proper Name: maribavir Sponsor: Takeda Pharmaceuticals USA, Inc. Approval Date: November 23, 2021 Indication: For the treatment of adults and pediatric patients 12 years of age and older and weighing at least 35 kg with post-transplant cytomegalovirus (CMV) infection/disease that is refractory to treatment (with or without genotypic resistance) with ganciclovir, valganciclovir, cidofovir or foscarnet. CENTER FOR DRUG EVALUATION AND RESEARCH 215596Orig1s000 CONTENTS Reviews / Information Included in this NDA Review. Approval Letter X Other Action Letters Labeling X REMS Officer/Employee List X Integrated Review(s) X Product Quality Review(s) X Other Reviews X Risk Assessment and Risk Mitigation Review(s) X Proprietary Name Review(s) X Administrative/Correspondence Document(s) X CENTER FOR DRUG EVALUATION AND RESEARCH APPLICATION NUMBER: 215596Orig1s000 APPROVAL LETTER NDA 215596 NDA APPROVAL Takeda Pharmaceuticals USA, Inc. Attention: Michael A. Cronin, PharmD Director, Global Regulatory Affairs 650 East Kendall Street Cambridge, MA 02142 Dear Dr. Cronin: Please refer to your new drug application (NDA) dated and received on March 23, 2021, and your amendments, submitted under section 505(b) of the Federal Food, Drug, and Cosmetic Act (FDCA) for Livtencity (maribavir) oral tablets. This NDA provides for the use of Livtencity (maribavir) oral tablets for the treatment of adults and pediatric patients 12 years of age and older and weighing at least 35 kg with post-transplant cytomegalovirus (CMV) infection/disease that is refractory to treatment (with or without genotypic resistance) with ganciclovir, valganciclovir, cidofovir or foscarnet. We have completed our review of this application, as

[DOCUMENT TEXT CLIPPED: omitted 996 characters; showing beginning and end.]

d and Drug Administration Silver Spring, MD 20993  CARTON AND CONTAINER LABELING Submit final printed carton and container labeling that are identical to the enclosed carton and container labeling as soon as they are available, but no more than 30 days after they are printed. Please submit these labeling electronically according to the guidance for industry Providing Regulatory Submissions in Electronic Format - Certain Human Pharmaceutical Product Applications and Related Submissions Using the

# DOCUMENT ID: 66387_7 (570 tokens) 
If child is younger than 3 months old, use of oseltamivir for chemoprophylaxis is not recommended unless situation is judged critical due to limited data in this age group. If child is 3 months or older and younger than 1 yr old2 3 mg/ kg/dose once daily3 If 1 yr or older, dose varies by child's weight: 15 kg or less, the dose is 30 mg once a day >15 to 23 kg, the dose is 45 mg once a day >23 to 40 kg, the dose is 60 mg once a day >40 kg, the dose is 75 mg once a day

Inhaled Zanamivir6

Treatment (5 days)

10 mg (two 5-mg inhalations) twice daily

(FDA approved and recommended for use in children 7 yrs or older)

Chemoprophylaxis (7 days)5

10 mg (two 5-mg inhalations) once daily

(FDA approved for and recommended for use in children 5 yrs or older)

Intravenous Peramivir7

Treatment (1 day)1

(6 months to 12 yrs of age) One 12 mg/kg dose, up to 600 mg maximum, via intravenous infusion for a minimum of 15 minutes

(FDA approved and recommended for use in children 6 months or older)

Chemoprophylaxis8

Not recommended

Oral Baloxavir9

Treatment (1 day)

(5 yrs and older weighing <20 kg: single dose of 2 mg/kg by suspension; weighing 20 kg to <80 kg: single dose of 40 mg by tablet or suspension; weighing >=80 kg: single dose of 80 mg by tablet or suspension)

FDA approved and recommended for use in otherwise healthy children 5 yrs and older.

Chemoprophylaxis9

FDA approved for post-exposure prophylaxis for persons aged 5 years and older. Dosage is the same as for treatment.

Abbreviations: N/A = not approved

- Longer treatment duration may be needed for severely ill patients.

- Oral oseltamivir is approved by the FDA for treatment of acute uncomplicated influenza within 2 days of illness onset with twice-daily dosing in people 14 days and older, and for chemoprophylaxis with once-daily dosing in people 1 year and older. Although not part of the FDA-approved indications, use of oral oseltamivir for treatment of influenza in infants less than 14 days old, and for chemoprophylaxis in infants 3 months to 1 year of age, is recommended by CDC and the American Academy of Pediatrics (Recommendations for Prevention and Control of Influenza in Children, 2023-2024).

# DOCUMENT ID: 97801_7 (750 tokens) 
Acesulfame potassium injected intravenously in rats has a blood elimination half-life of about 14 minutes, which demonstrates that ACK is rapidly cleared from the general circulation. In rats given ACK orally at 10 mg/kg, maximum blood levels (0.7 ug/mL) occurred about 0.5 hour after dosing and then declined slowly, likely because of continued absorption from the gastrointestinal tract (resulting in a blood elimination half-life = 4.8 hours). Rapid absorption and excretion of ACK also occurs in humans: blood levels (0.2-0.3 ug/mL) peak 1 to 1.5 hours after ingestion of a single oral dose of 30 mg (about 0.4 mg per kilogram of body weight) followed by a blood elimination half-life of 2.5 hours. In dogs, maximum blood levels (about 7 ug/mL) occur 1 to 1.5 hours after ingestion of a single oral dose of 10 mg per kilogram of body weight, followed by a blood elimination half-life of 1.3 hours.15,18,20 Acesulfame potassium absorption in pigs was also relatively rapid, with maximum blood levels (0.35-0.72 ug/mL) reached 1 to 2 hours after oral administration of a single dose of 3.6 to 4.5 mg/kg.15,16

Repeated exposures did not alter the fast absorption profiles of ACK in rats and dogs. Unlabeled ACK was administered either as part of the diet in rats (840 or 1325 mg/kg/d) or as daily bolus doses in dogs (900 or 1500 mg/kg/d) for 2 weeks prior to 24-hour toxicokinetic assessments. The 24-hour areas under the curve in both species were proportional to dose and were 848 to 934 ug * h/mL and 1521 to 1671 ug * h/mL in rats and 2149 to 3819 ug * h/mL and 3065 to 5722 ug * h/mL in dogs for the lower-dose and the higher-dose group, respectively. Dogs, whose bolus exposure regimen allowed assessment of peak plasma concentrations, exhibited peak levels of 180 to 311 ug/mL and 273 to 491 ug/mL for the lower dose and the higher dose, respectively. F

[DOCUMENT TEXT CLIPPED: omitted 642 characters; showing beginning and end.]

highest exposure concentration in the study that included evaluation of all rat life stages, 3% ACK in diet (or 1500 mg per kilogram of body weight per day), is the NOAEL used for the basis of ADIs set by the JEFCA and the FDA. Species and age differences are accounted for in safety assessments through the use of a 100-fold uncertainty factor to convert the NOAEL observed in an animal study to the ADI (ie, the ADI is calculated by dividing the NOAEL by 100).

Potassium in acesulfame potassium.

# DOCUMENT ID: 25814_8 (656 tokens) 
Olaparib(4-(3-{[4-(Cyclopropylcarbonyl)-1-piperazinyl]carbonyl}-4-fluorobenzyl)-1(2H)-phthalazinone) was the first drug from the family of PARP inhibitors that was approved by the FDA in 2014 for the treatment of ovarian cancer [140]. It inhibits PARP1 and PARP 2 which results in double-stranded DNA breaks that produces apoptosis in cancer cells [140,141]. Olaparib contains oxygen atoms which forms hydrogen bonds with backbone atoms in the catalytic domain of Arginine and also water mediated hydrogen bonds with aspartic acid and Van der Waals Force interaction with aliphatic side chain of glutamic acid in the regulatory domain [142]. Olaparib was approved both in Europe and USA as maintainence treatment in platinum-sensitive ovarian cancer patients, independent of their BRCA1/2 mutation status [143].

Olaparib can be administered orally at daily doses amounting 200-600 mg, depending on the renal function of the patient [141]. Its peak plasma concentration occurs 1-3 hours after administration [144] and it has a terminal elimination half-life of 11.9 h following a 400 mg dose [141]. Olaparib has an apparent volume of distribution 167 L and is primarily metabolized in the liver by dehydrogenation and oxidation, and it undergoes glucuronide and sulfide conjugation [144]. Olaparib is primarily excreted unchanged in the urine and consequently, olaparib's renal clearance is decreased in patients with diminished renal function [141]. Furthermore, in patients with mild (GFR = 51-80 mL/min) to moderate renal impairment (GFR = 31-50 ml/min), there was a decrease in the volume of distribution and terminal half-life compared to patients with normal renal function [145,146]. The most common adverse events of any grade reported following treatment with olaparib were nausea, fatigue, vomiting, anemia and diarrhea, although severe grade 3 or 4 ane

[DOCUMENT TEXT CLIPPED: omitted 466 characters; showing beginning and end.]

e models [151]. Data from a Phase I study (NCT00494442) has shown that olaparib alone has antitumor efficacy in pretreated BRCA1 and BRCA2-deficient patients with recurrent ovarian cancer [152]. Phase III trials with olaparib have shown a significant increase in the quality of life and a longer PFS in: 1) ovarian cancer patients with a germline BRCA1/2 mutation who were previously treated with platinum chemotherapy [153] and 2) patients with platinum-sensitive relapsed ovarian cancer [143,148].

# DOCUMENT ID: 15546_15 (709 tokens) 
| Orlistat, prescription (120 mg) | 120 mg TID | Pancreatic and gastric lipase inhibitor | 2.9-3.4 kg (6.5-7.5 lb), 2.9-3.4%; 1 y | FDA approved in 1999 for chronic weight management | Decreased absorption of fat-soluble vitamins, steatorrhrea, oily spotting, flatulence with discharge, fecal urgency, oily evacuation, increased defecation, fecal incontinence | Cyclosporine (taken 2 h before or after orlistat dose), chronic malabsorption syndrome, pregnancy and breastfeeding, cholestasis, levothyroxine, warfarin, antiepileptic drugs |

| Orlistat, over-the-counter (60 mg) | 60-120 mg TID | Pancreatic and gastric lipase inhibitor | 2.9-3.4 kg (6.5-7.5 lb), 2.9-3.4%; 1 y | FDA approved in 1999 for chronic weight management | See Orlistat, prescription | See Orlistat, prescription |

| Lorcaserin (10 mg) | 10 mg BID | 5HT2c receptor agonist | 3.6 kg (7.9 lb), 3.6%; 1 y | FDA approved in 2012 for chronic weight management | Headache, nausea, dry mouth, dizziness, fatigue, constipation | Pregnancy and breastfeeding Use with caution: SSRI, SNRI/MAOI, St John's wort, triptans, buproprion, dextromethorphan |

| Phentermine (P)/topiramate (T) | 3.75 mg P/23 mg T ER QD (starting dose) 7.5 mg P/46 mg T ER daily (recommended dose) 15 mg P/92 mg P/T ER daily (high dose) | GABA receptor modulation (T) plus norepinephrine-releasing agent (P) | 6.6 kg (14.5 lb) (recommended dose), 6.6% 8.6 kg (18.9 lb) (high dose), 8.6%; 1 y | FDA approved in 2012 for chronic weight management | Insomnia, dry mouth, constipation, paraesthesia, dizziness, dysgeusia | Pregnancy and breastfeeding, hyperthyroidism, glaucoma, MAO inhibitor, sympathomimetic amines |

| Naltrexone/bupropion | 32 mg/360 mg 2 tablets QID (high dose) | Reuptake inhibitor of dopamine and norepinephrine (bupropion) and opioid antagonist (naltrexone) | 4.8%; 1y (Ref. 79) | FDA approved in 2014 for chronic weight management | Nausea, constipation, headache, vomiting, dizziness | Uncontrolled hypertension, seizure disorders, anorexia nervosa or bulimia, drug or alcohol withdrawal, MAO inhibitors |

| Liraglutide | 3.0 mg injectable | GLP-1 agonist | 5.8 kg; 1 y (Ref. 30, 31) | FDA approved in 2014 for chronic weight management | Nausea, vomiting, pancreatitis | Medullary thyroid cancer history, multiple endocrine neoplasia type 2 history |

# DOCUMENT ID: 50858_8 (666 tokens) 
| Half-life: five to 12 hours | ||||

| Excretion: feces | ||||

| Safety | Adverse effects: | Adverse effects: | ||

| More common: fever, hypokalemia, injury to intravenous site, orthostatic hypotension | More common: nausea, pollakiuria, polyuria, thirst, xerostomia | |||

| Less common: anemia, atrial fibrillation, confusion, constipation, dehydration, diarrhea, dry mouth, electrocardiographic abnormalities, erythema, headache, hematuria, hyperglycemia, hypertension, hypoglycemia, hypomagnesia, hyponatremia, hypotension, insomnia, nausea, oral candidiasis, pain, peripheral edema, pharyngolaryngitis, phlebitis, pneumonia, polyuria, pruritus, thirst, urinary tract infection, vomiting | Less common: anorexia, constipation, fever, gastrointestinal bleeding, hepatotoxicity, hyperglycemia, hypernatremia, weakness | |||

| Change intravenous site every 24 hours; avoid corn products | Do not use for more than 30 days or in patients with underlying liver disease because of risk of hepatotoxicity; avoid consumption of grapefruit juice | |||

| Contraindicated in patients with anuria or concurrent use of CYP3A inhibitors | Liver function should be monitored frequently | |||

| Not recommended for patients with creatinine clearance less than 30 mL per minute per 1.73 m2 (0.50 mL per second per m2) | Contraindicated in patients with hypovolemic hyponatremia, anuria, or concurrent use of CYP3A inhibitors, or when there is an urgent need to increase sodium levels | |||

| Not recommended for patients with creatinine clearance less than 10 mL per minute per 1.732 (0.17 mL per second per m2) | ||||

| Price* | $687 for 100 mL of solution (20 mg of conivaptan) | $3,440 for 10 15- or 30-mg tablets | ||

| Considerations | Vaptans should be initiated in the inpatient setting to monitor sodium levels | |||

| No reports of osmotic demyelination; ho

[DOCUMENT TEXT CLIPPED: omitted 623 characters; showing beginning and end.]

mia is caused by net water loss (increased loss or decreased intake) or, rarely, sodium gain. Patients at increased risk include those with an impaired thirst mechanism or restricted access to water (e.g., those with altered mental status, intubated patients, infants, older adults).

[AUTO-POPULATED] Top 6 docs from this search have been added to your curated set at 'fair' importance. Use `curate` with `importance` to promote/demote and `remove_ids` to drop irrelevant ones.
[Context: 4231/30720]

RETURN 0.metadata:
{
  "metadata": {
    "returned_chunk_ids": [
      "59631_0",
      "66387_7",
      "97801_7",
      "25814_8",
      "15546_15",
      "50858_8"
    ],
    "pre_rerank_chunk_ids": null
  }
}
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 0 working-memory snapshot after harness update}
pool_size: 6
curated_size: 6 / 30
importance_counts: very_high=0, high=0, fair=6, low=0
curated_set:
  - 15546 [fair]
  - 25814 [fair]
  - 50858 [fair]
  - 59631 [fair]
  - 66387 [fair]
  - 97801 [fair]
\end{trajectorylisting}

\subsubsection*{Turn 1: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolCurate}{Turn 1 tool call(s)}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [
        "59631_0",
        "66387_7",
        "97801_7",
        "25814_8",
        "50858_8"
      ],
      "importance": {
        "59631_0": "high",
        "66387_7": "low",
        "97801_7": "low",
        "25814_8": "high",
        "50858_8": "fair"
      }
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 1 tool return 0}
RETURN 0.text:
Curated set updated (6/30): 25814[high], 59631[high], 15546[fair], 50858[fair], 66387[low], 97801[low]
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 1 working-memory snapshot after harness update}
pool_size: 6
curated_size: 6 / 30
importance_counts: very_high=0, high=2, fair=2, low=2
curated_set:
  - 25814 [high]
  - 59631 [high]
  - 15546 [fair]
  - 50858 [fair]
  - 66387 [low]
  - 97801 [low]
\end{trajectorylisting}

\subsubsection*{Turn 2: \CaseTool{toolSearch}{search\_corpus}}
\begin{trajectorylisting}{toolNeutral}{Turn 2 model reasoning}
The first search hit a known FDA submission doc for Livtencity (maribavir). That fits oral administration, nausea side effect, and contraindication at 30kg/10y, but the drug class/youth contraindication constraint is strong. We need the 2022 study page and the approval letter identifying the Regulatory Project Manager. The search angle using the study constraints is still relevant; I'll first search for the 2022 study on maribavir to bridge to the approval letter.
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 2 tool call(s)}
[
  {
    "tool": "search_corpus",
    "params": {
      "query": "maribavir 2022 study liver eliminated half-life less than 10 hours oral migration 31 references December two authors"
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 2 tool return 0}
RETURN 0.text:

# DOCUMENT ID: 83797_4 (723 tokens) 
As a postmarketing commitment, the FDA is requiring the manufacturer to conduct phenotypic analysis of maribavir against human CMV. Substitutions designated as a high priority for analysis are pUL97 M460I/T, A594E/P/T/V, L595F/W, and C603R/W/Y. Substitutions designated as medium priority are pUL97 A440V, V466M, A591V, E596G, K599E, and C607F/Y. Substitutions designated as low priority are pUL97 P132L, L405P, C518Y, I610T, and A613V; pUL27 P10L, N289D, H29Y, D298G, N300G, P307L, V310A, D351N, and I367V; and pUL54 S290R and K475S.18
Maribavir does not prolong the QT interval to a clinically important extent.1,19
Pharmacokinetics
Following oral administration, median T max is 1 to 3 hours.1,19,20 Plasma exposure (C max and AUC) increased approximately dose proportionally following a single dose of 50 to 1600 mg and multiple doses of up to 2400 mg/day.1,20 Compared with administration in the fasted state, administration with a moderate-fat meal resulted in a small reduction in AUC 0-infinity (geometric mean ratio, 0.864; 90% CI, 0.804-0.929) and C max (0.722; 90% CI, 0.656-0.793). Steady state is reached within 2 days with twice-daily dosing.1 Mean steady-state volume of distribution is 27.3 L. Maribavir is 98% plasma protein bound. The blood-to-plasma ratio is 1.37.1,20 Maribavir does not appear to cross the blood-brain barrier.9
Maribavir, the parent drug, is responsible for the pharmacologic activity. Mean maribavir half-life is 4.32 hours in transplant recipients.1 A half-life of 3 to 5 hours has been reported in healthy subjects and patients with HIV infection.20 Maribavir is primarily eliminated by hepatic metabolism via CYP3A4 (major) and CYP1A2 (minor). An N-dealkylated metabolite (VP 44469) is the major circulating inactive metabolite; metabolite levels peak at 2 to 4 hours after maribavir administration.1,19 The majority of the maribavir dose is excreted in the urine (61%, with less than 2% as unchanged drug); 14% of the dose is excreted in the feces (5.7% as unchanged drug).1,20
No clinically important differences in maribavir pharmacokinetics were observed based on age (18-79 years), sex, race (White, Black, Asian, or other), ethnicity (Hispanic/Latino or non-Hispanic/Latino), body weight (36-141 kg), mild to severe renal impairment (creatinine clearance 12-70 mL/minute), or mild to moderate hepatic impairment (Child-Pugh class A or B). Maribavir has not been studied in patients with end-stage renal disease, including patients on dialysis, or in patients with severe hepatic impairment.1,21

# DOCUMENT ID: 83797_15 (717 tokens) 
1.Livtencity (maribavir) [prescribing information]. Takeda Pharmaceuticals America Inc; 2021. [Google Scholar]
2.Razonable RR, Humar A. Cytomegalovirus in solid organ transplant recipients-Guidelines of the American Society of Transplantation Infectious Diseases Community of practice. Clin Transplant. 2019;33(9):e13512. doi: 10.1111/ctr.13512 [DOI] [PubMed] [Google Scholar]
3.Cidofovir [Prescribing Information]. Mylan Institutional LLC; 2021. [Google Scholar]
4.Orange Book. Approved Drug Products with Therapeutic Equivalence Evaluations. Food and Drug Administration. Updated January 2022. Accessed January 19, 2022. [Google Scholar]
5.Foscavir (foscarnet sodium) [prescribing information]. Hospira Inc; 2020. [Google Scholar]
6.Ganciclovir sodium injection [prescribing information]. Fresenius Kabi; 2020. [Google Scholar]
7.Prevymis (letermovir) [prescribing information]. Merck & Co Inc; 2021. [Google Scholar]
8.Valcyte (valganciclovir) [prescribing information]. Genentech USA Inc; 2021. [Google Scholar]
9.Avery RK, Alain S, Alexander BD, et al.; SOLSTICE Trial Investigators. Maribavir for refractory cytomegalovirus infections with or without resistance post-transplant: results from a phase 3 randomized clinical trial. Clin Infect Dis. Published online December 2, 2021. doi: 10.1093/cid/ciab988 [DOI] [PMC free article] [PubMed] [Google Scholar]
10.Wang FZ, Roy D, Gershburg E, Whitehurst CB, Dittmer DP, Pagano JS. Maribavir inhibits Epstein-Barr virus transcription in addition to viral DNA replication. J Virol. 2009;83(23):12108-12117. doi: 10.1128/JVI.01575-09 [DOI] [PMC free article] [PubMed] [Google Scholar]
11.Whitehurst CB, Sanders MK, Law M, et al. Maribavir inhibits Epstein-Barr virus transcription through the EBV protein kinase. J Virol. 2013;87(9):5311-5315. doi: 10.1128/JVI.03505-12 [DOI] [PMC free article] [PubMed] [Google Scholar]
12.Chou S, Marousek GI. Maribavir antagonizes the antiviral action of ganciclovir on human cytomegalovirus. Antimicrob Agents Chemother. 2006;50(10):3470-3472. doi: 10.1128/AAC.00577-06 [DOI] [PMC free article] [PubMed] [Google Scholar]
13.Chou S, Ercolani RJ, Derakhchan K. Antiviral activity of maribavir in combination with other drugs active against human cytomegalovirus. Antiviral Res. 2018;157:128-133. doi: 10.1016/j.antiviral.2018.07.013 [DOI] [PMC free article] [PubMed] [Google Scholar]

# DOCUMENT ID: 17183_8 (746 tokens) 
due to the parent drug. Following oral administration, plasma maribavir exposure (Cmax and AUC) increased approximately dose-proportionally following a single dose of 50 to 1600 mg (0.125 to four times the recommended dose) and multiple doses up to 2400 mg per day (three times the recommended daily dose). Maribavir PK is time-independent. With twice-daily dosing, steady state is reached within 2 days, with mean accumulation ratios of Cmax and AUC ranging from 1.37 to 1.47. The pharmacokinetic properties of maribavir following administration of LIVTENCITY are displayed in Table 4. The multiple-dose pharmacokinetic parameters are provided in Table 5. 9 Reference ID: 4893709 This label may not be the latest approved by FDA. For current labeling information, please visit Table 4: Pharmacokinetic Properties of Maribavir Absorptiona Tmax (h), median 1.0 to 3.0 Distribution Mean apparent steady-state volume of distribution (Vss, L) 27.3 % bound to human plasma proteins 98.0 across the concentration range of 0.05-200 ug/mL Blood-to plasma ratio 1.37 Elimination Major route of elimination Hepatic metabolism Half-life (t1/2) in transplant patients (h), mean 4.32 Oral clearance (CL/F) in transplant patients (L/h), mean 2.85 Metabolism Metabolic pathwaysb CYP3A4 (major) and CYP1A2 (minor) Excretion % of dose excreted as total 14C (unchanged drug) in urinec 61 (<2) % of dose excreted as total 14C (unchanged drug) in fecesc 14 (5.7) a When taken orally with a moderate fat meal versus fasted, the AUC0-infinity and Cmax (geometric mean ratio [90% CI] of maribavir are 0.864 [0.804, 0.929] and 0.722 [0.656, 0.793], respectively. b In vitro studies have shown that maribavir is biotransformed into a major circulating inactive metabolite: VP 44469 (N-dealkylated metabolite), with a metabolic ratio of 0.15 - 0.20 c Dosing in mass balance study: single-d

[DOCUMENT TEXT CLIPPED: omitted 410 characters; showing beginning and end.]

u = Concentration at the end of a dosing interval. a Pharmacokinetic parameter values based on post-hoc estimates from maribavir population pharmacokinetic model in transplant patients with CMV receiving 400 mg of LIVTENCITY twice daily with or without food. b tau is maribavir dosing interval: 12 hours Specific Populations There were no clinically significant differences in the pharmacokinetics of maribavir based on age (18-79 years), gender, race (Caucasian, Black, Asian, or others), ethnicity

# DOCUMENT ID: 83797_18 (333 tokens) 
29.Goldwater DR, Dougherty C, Schumacher M, Villano SA. Effect of ketoconazole on the pharmacokinetics of maribavir in healthy adults. Antimicrob Agents Chemother. 2008;52(5):1794-1798. doi: 10.1128/AAC.00951-07 [DOI] [PMC free article] [PubMed] [Google Scholar]
30.Song IH, Ilic K, Murphy J, Lasseter K, Martin P. Effects of maribavir on P-glycoprotein and CYP2D6 in healthy volunteers. J Clin Pharmacol. 2020;60(1):96-106. doi: 10.1002/jcph.1504 [DOI] [PMC free article] [PubMed] [Google Scholar]
31.Ma JD, Nafziger AN, Villano SA, Gaedigk A, Bertino JS., Jr.Maribavir pharmacokinetics and the effects of multiple-dose maribavir on cytochrome P450 (CYP) 1A2, CYP 2C9, CYP 2C19, CYP 2D6, CYP 3A, N-acetyltransferase-2, and xanthine oxidase activities in healthy adults. Antimicrob Agents Chemother. 2006;50(4):1130-1135. doi: 10.1128/AAC.50.4.1130-1135.2006 [DOI] [PMC free article] [PubMed] [Google Scholar]

# DOCUMENT ID: 83797_17 (708 tokens) 
22.Papanicolaou GA, Silveira FP, Langston AA, et al. Maribavir for refractory or resistant cytomegalovirus infections in hematopoietic-cell or solid-organ transplant recipients: a randomized, dose-ranging, double-blind, phase 2 study. Clin Infect Dis. 2019;68(8):1255-1264. doi: 10.1093/cid/ciy706 [DOI] [PMC free article] [PubMed] [Google Scholar]
23.Maertens J, Cordonnier C, Jaksch P, et al. Maribavir for preemptive treatment of cytomegalovirus reactivation. New Engl J Med. 2019;381(12):1136-1147. doi: 10.1056/NEJMoa1714656 [DOI] [PubMed] [Google Scholar]
24.Avery RK, Marty FM, Strasfeld L, et al. Oral maribavir for treatment of refractory or resistant cytomegalovirus infections in transplant recipients. Transpl Infect Dis. 2010;12(6):489-496. doi: 10.1111/j.1399-3062.2010.00550.x [DOI] [PubMed] [Google Scholar]
25.Marty FM, Ljungman P, Papanicolaou GA, et al. Maribavir prophylaxis for prevention of cytomegalovirus disease in recipients of allogeneic stem-cell transplants: a phase 3, double-blind, placebo-controlled, randomised trial. Lancet Infect Dis. 2011;11(4):284-292. doi: 10.1016/S1473-3099(11)70024-X [DOI] [PubMed] [Google Scholar]
26.Winston DJ, Young JA, Pullarkat V, et al. Maribavir prophylaxis for prevention of cytomegalovirus infection in allogeneic stem cell transplant recipients: a multicenter, randomized, double-blind, placebo-controlled, dose-ranging study. Blood. 2008;111(11):5403-5410. doi: 10.1182/blood-2007-11-121558 [DOI] [PMC free article] [PubMed] [Google Scholar]
27.Winston DJ, Saliba F, Blumberg E, et al.; 1263-301 Clinical Study Group. Efficacy and safety of maribavir dosed at 100 mg orally twice daily for the prevention of cytomegalovirus disease in liver transplant recipients: a randomized, double-blind, multicenter controlled trial. Am J Transplant. 2012;12(11):3021-3030. doi: 10.1111/j.1600-6143.2012.04231.x [DOI] [PubMed] [Google Scholar]
28.Pescovitz MD, Bloom R, Pirsch J, Johnson J, Gelone S, Villano SA. A randomized, double-blind, pharmacokinetic study of oral maribavir with tacrolimus in stable renal transplant recipients. Am J Transplant. 2009;9(10):2324-2330. doi: 10.1111/j.1600-6143.2009.02768.x [DOI] [PubMed] [Google Scholar]

# DOCUMENT ID: 73877_2 (477 tokens) 
B: May be acceptable. Either animal studies show no risk but human studies not available or animal studies showed minor risks and human studies done and showed no risk. C: Use with caution if benefits outweigh risks. Animal studies show risk and human studies not available or neither animal nor human studies done. D: Use in LIFE-THREATENING emergencies when no safer drug available. Positive evidence of human fetal risk. X: Do not use in pregnancy. Risks involved outweigh potential benefits. Safer alternatives exist. NA: Information not available.Pharmacology

Mechanism of Action

Antiviral activity mediated by competitive inhibition of the protein kinase activity of human CMV enzyme pUL97, which inhibits protein phosphorylation

Maribavir inhibited human CMV replication in virus yield reduction, DNA hybridization, and plaque reduction assays in human lung fibroblast cell line, human embryonic kidney, and human foreskin fibroblast cells

Absorption

Peak plasma time: 1-3 hr

AUC: 128 ug*hr/mL

Peak plasma concentration: 17.2 ug*hr/mL

Distribution

Vd (steady-state): 27.3 L

Plasma bound: 98%

Blood-to-plasma ratio: 1.37

Metabolism

Metabolized by CYP3A4 (major) and CYP1A2 minor

Elimination

Clearance: 2.85 L/hr

Half-life: 4.32 hr

Excretion: Urine (61% [<2% unchanged]); feces (14% [5.7%])

Administration

Oral Administration

Take with or without food

Storage

Store at 20-25oC (68-77oF); excursions permitted to 15-30oC (59-86oF)

Images

Formulary

Adding plans allows you to compare formulary status to other drugs in the same class.

To view formulary information first create a list of plans. Your list will be saved and can be edited at any time.

Adding plans allows you to:

- View the formulary and any restrictions for each plan.

- Manage and view all your plans together - even plans in different states.

- Compare formulary status to other drugs in the same class.

- Access your plan list on any device - mobile or desktop.
[Context: 10346/30720]

RETURN 0.metadata:
{
  "metadata": {
    "returned_chunk_ids": [
      "83797_4",
      "83797_15",
      "17183_8",
      "83797_18",
      "83797_17",
      "73877_2"
    ],
    "pre_rerank_chunk_ids": null
  }
}
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 2 working-memory snapshot after harness update}
pool_size: 9
curated_size: 6 / 30
importance_counts: very_high=0, high=2, fair=2, low=2
curated_set:
  - 25814 [high]
  - 59631 [high]
  - 15546 [fair]
  - 50858 [fair]
  - 66387 [low]
  - 97801 [low]
\end{trajectorylisting}

\subsubsection*{Turn 3: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolNeutral}{Turn 3 model reasoning}
The angle is still specific enough: maribavir definitely fits the drug class and indicated age/weight constraint. The search just found a study document portion on marcibavir pharmacokinetics, likely the 2022 study, and better links to the approval letter. What isn't working is the last search angle is not new; it just reinforced maribavir pharmacokinetics but not the approval-responsible-regulatory-manager doc. Before refining further, I must curate the fresh maribavir study results.
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 3 tool call(s)}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [
        "83797_4",
        "17183_8",
        "73877_2"
      ],
      "importance": {
        "83797_4": "high",
        "17183_8": "high",
        "73877_2": "fair"
      }
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 3 tool return 0}
RETURN 0.text:
Curated set updated (9/30): 17183[high], 25814[high], 59631[high], 83797[high], 15546[fair], 50858[fair], 73877[fair], 66387[low], 97801[low]
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 3 working-memory snapshot after harness update}
pool_size: 9
curated_size: 9 / 30
importance_counts: very_high=0, high=4, fair=3, low=2
curated_set:
  - 17183 [high]
  - 25814 [high]
  - 59631 [high]
  - 83797 [high]
  - 15546 [fair]
  - 50858 [fair]
  - 73877 [fair]
  - 66387 [low]
  - 97801 [low]
\end{trajectorylisting}

\subsubsection*{Turn 4: \CaseTool{toolSearch}{search\_corpus}}
\begin{trajectorylisting}{toolNeutral}{Turn 4 model reasoning}
We have maribavir as the likely agent. The unsolved gap is the approval letter and specifically the Regulatory Project Manager name. A paper in the search results strongly supports maribavir pharmacokinetics; now the missing angle is the regulatory letter/application behind the FDA approval based on the March 23 NDA receipt and December 2022 study references. Most likely the letter is an FDA approval letter for maribavir tablets (Livtencity). I should search the regulatory/doc approval language directly, using the NDA date and the unique concession name (Regulatory Project Manager).
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 4 tool call(s)}
[
  {
    "tool": "search_corpus",
    "params": {
      "query": "FDA approval letter Regulatory Project Manager December 2021 March 23 NDA application number reg.mari.maribavir tablets"
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 4 tool return 0}
RETURN 0.text:

# DOCUMENT ID: 59631_1 (754 tokens) 
eCTD Specifications. For administrative purposes, designate this submission "Final Printed Carton and Container Labeling for approved NDA 215596." Approval of this submission by FDA is not required before the labeling is used. DATING PERIOD Based on the stability data submitted to date, the expiry dating period for Livtencity (maribavir) tablets shall be 30 months from the date of manufacture when stored at 20 degrees C to 25 degrees C (68 degrees F to 77 degrees F). Results of ongoing stability should be submitted throughout the dating period in your annual report, as they become available, including the results of stability studies from the first three production lots. REQUIRED PEDIATRIC ASSESSMENTS Under the Pediatric Research Equity Act (PREA) (21 U.S.C. 355c), all applications for new active ingredients (which includes new salts and new fixed combinations), new indications, new dosage forms, new dosing regimens, or new routes of administration are required to contain an assessment of the safety and effectiveness of the product for the claimed indication in pediatric patients unless this requirement is waived, deferred, or inapplicable Because this drug product for this indication has an orphan drug designation, you are exempt from this requirement. POSTMARKETING REQUIREMENTS UNDER 505(o) Section 505(o)(3) of the Federal Food, Drug, and Cosmetic Act (FDCA) authorizes FDA to require holders of approved drug and biological product applications to conduct postmarketing studies and clinical trials for certain purposes, if FDA makes certain findings required by the statute. We have determined that an analysis of spontaneous postmarketing adverse events reported under subsection 505(k)(1) of the FDCA will not be sufficient to assess a signal of serious risk of virologic failure due to resistance to maribavir. Reference ID: 4893709 ND

[DOCUMENT TEXT CLIPPED: omitted 892 characters; showing beginning and end.]

ule: Final Protocol Submission: 01/2022 High Priority Phenotyping Submission: 06/2023 Medium/low Priority Phenotyping Submission: 12/2023 Study Completion: 12/2023 Final Report Submission: 01/2024 4182-2 Determine the human cytomegalovirus gB subtype for each of the subjects in study SHP620-303 "A Phase 3, Multicenter, Randomized, Open-label, Active controlled Study to Assess the Efficacy and Safety of Maribavir Treatment Compared to Investigator assigned Treatment in Transplant Recipients with

# DOCUMENT ID: 17183_0 (732 tokens) 
HIGHLIGHTS OF PRESCRIBING INFORMATION These highlights do not include all the information needed to use LIVTENCITY safely and effectively. See full prescribing information for LIVTENCITY LIVTENCITY (maribavir) tablets, for oral use Initial U.S. Approval: 2021 ----------------------------- INDICATIONS AND USAGE--------------------------- LIVTENCITY is a cytomegalovirus (CMV) pUL97 kinase inhibitor indicated for the treatment of adults and pediatric patients (12 years of age and older and weighing at least 35 kg) with post-transplant CMV infection/disease that is refractory to treatment (with or without genotypic resistance) with ganciclovir, valganciclovir, cidofovir or foscarnet. (1, 8.4 ) -------------------------DOSAGE AND ADMINISTRATION ---------------------- 400 mg (two 200 mg tablets) orally twice daily with or without food. (2.1, 2.2, 8.4) ----------------------- DOSAGE FORMS AND STRENGTHS--------------------- Tablets: 200 mg of maribavir. (3) -------------------------------- CONTRAINDICATIONS ----------------------------- None. (4) ------------------------- WARNINGS AND PRECAUTIONS----------------------- - LIVTENCITY may antagonize the antiviral activity of ganciclovir and valganciclovir. Coadministration is not recommended. (5.1, 7.1) - Virologic failure can occur during and after treatment with LIVTENCITY. Monitor CMV DNA levels and check for resistance if patient does not respond to treatment. Some maribavir pUL97 resistance-associated substitutions confer cross-resistance to ganciclovir and valganciclovir. (5.2, 12.4, 14.1) - The concomitant use of LIVTENCITY and certain drugs may result in potentially significant drug interactions, some of which may lead to reduced therapeutic effect of LIVTENCITY or adverse reactions of concomitant drugs. (5.1, 5.3, 7.1, 7.2, 7.3) - LIVTENCITY has the potential to increase the drug con

[DOCUMENT TEXT CLIPPED: omitted 665 characters; showing beginning and end.]

D ADVERSE REACTIONS, contact Takeda Pharmaceuticals America, Inc. at 1-877-TAKEDA-7 (1-877-825-3327) or FDA at 1-800-FDA-1088 or  ------------------------------- DRUG INTERACTIONS------------------------------ - Refer to the full prescribing information for important drug interactions with LIVTENCITY. (5.1, 5.3, 7) - Coadministration with strong CYP3A4 inducers: not recommended. Refer to full prescribing information for dosage modification when coadministered with certain anticonvulsants. (2.2,

# DOCUMENT ID: 83797_16 (723 tokens) 
14.Chou S, Song K, Wu J, Bo T, Crumpacker C. Drug resistance mutations and associated phenotypes detected in clinical trials of maribavir for treatment of cytomegalovirus infection. J Infect Dis. 2020. Published online July 29, 2020. doi: 10.1093/infdis/jiaa462 [DOI] [PMC free article] [PubMed] [Google Scholar]
15.Chou S, Wu J, Song K, Bo T. Novel UL97 drug resistance mutations identified at baseline in a clinical trial of maribavir for resistant or refractory cytomegalovirus infection. Antiviral Res. 2019;172:104616. doi: 10.1016/j.antiviral.2019.104616 [DOI] [PMC free article] [PubMed] [Google Scholar]
16.Santos Bravo M, Plault N, Sanchez Palomino S, et al. Phenotype and genotype study of novel C480F maribavir-ganciclovir cross-resistance mutation detected in hematopoietic stem cell and solid organ transplant recipients. J Infect Dis. 2021;224(6):1024-1028. doi: 10.1093/infdis/jiab029 [DOI] [PubMed] [Google Scholar]
17.Chou S, Watters M, Sinha R, Kleiboeker S. Ganciclovir and maribavir susceptibility phenotypes of cytomegalovirus UL97 ATP binding region mutations detected by expanded genotypic testing. Antiviral Res. 2021;193:105139. doi: 10.1016/j.antiviral.2021.105139 [DOI] [PMC free article] [PubMed] [Google Scholar]
18.Farley J. NDA approval letter: Livtencity (maribavir) (NDA 215596). Food and Drug Administration. Published November 23, 2021. Accessed January 19, 2022. [Google Scholar]
19.Ilic K, Song I, Wu J, Martin P. Evaluation of the effect of maribavir on cardiac repolarization in healthy participants: thorough QT/QTc study. Clin Transl Sci. 2020;13(6):1260-1270. doi: 10.1111/cts.12814 [DOI] [PMC free article] [PubMed] [Google Scholar]
20.Wang LH, Peck RW, Yin Y, Allanson J, Wiggs R, Wire MB. Phase I safety and pharmacokinetic trials of 1263W94, a novel oral anti-human cytomegalovirus agent, in healthy and human immunodeficiency virus-infected subjects. Antimicrob Agents Chemother. 2003;47(4):1334-1342. doi: 10.1128/AAC.47.4.1334-1342.2003 [DOI] [PMC free article] [PubMed] [Google Scholar]
21.Swan SK, Smith WB, Marbury TC, et al. Pharmacokinetics of maribavir, a novel oral anticytomegalovirus agent, in subjects with varying degrees of renal impairment. J Clin Pharmacol. 2007;47(2):209-217. doi: 10.1177/0091270006296765 [DOI] [PubMed] [Google Scholar]

# DOCUMENT ID: 83797_1 (692 tokens) 
Generic Name: MARIBAVIR
Proprietary Name:Livtencity (Takeda)
Approval Rating: 1P (Orphan)
Therapeutic Class: Antiviral Agent; Benzimidazole Riboside
Similar Drugs: Ganciclovir, Letermovir, Valganciclovir
Sound-/Look-Alike Names:Livmarli, Lumify, Lumigan, Lumoxiti
Indications
Maribavir is indicated for the treatment of posttransplant cytomegalovirus (CMV) infection/disease that is refractory to treatment (with or without genotypic resistance) with ganciclovir, valganciclovir, foscarnet, or cidofovir in adults and pediatric patients 12 years and older and weighing at least 35 kg.1
Other antiviral agents approved for treatment of CMV infection/disease include cidofovir, foscarnet, intravenous (IV) ganciclovir, and valganciclovir. Letermovir has been used off-label in the treatment of CMV infection/disease.2 See Table 1 for a comparison of these agents. Agents used for CMV prophylaxis in transplant recipients include valganciclovir, IV ganciclovir, high-dose valacyclovir, letermovir, and adjunctive immunoglobulin preparations.2
Table 1.
Comparison of Antiviral Agents Approved for the Treatment of Cytomegalovirus.1,3-8
| | Maribavir | Cidofovir | Foscarnet | Ganciclovir | Letermovir | Valganciclovir |
| --- | :---: | :---: | :---: | :---: | :---: | :---: |
| Brand name (manufacturer) | Livtencity (Takeda) | (Various) | Foscavir (Hospira) | (Various) | Prevymis (Merck & Co.) | Valcyte (Genentech) |
| Generic availability | No | Yes | Yes | Yes | No | Yes |
| Doseform(s)/route of administration | Oral tablets | IV injection | IV injection | IV injection | IV injection and oral tablets | Oral tablets and oral solution |
| Approved population | Adults Pediatric patients >=12 years and weighing >=35 kg | Adults | Adults | Adults | Adults | Adults Pediatric patients (for prophylaxis indication [kidney and heart transplant patients]) |
| FDA-approved indications |
| Treatment of posttransplant CMV refractory to treatment with ganciclovir, valganciclovir, foscarnet, or cidofovir | X | | | | | |
| Treatment of CMV retinitis in patients with AIDS | | X | X | X | | X |
| Treatment of CMV retinitis in immunocompromised patients | | | | X | | |
| Treatment of acyclovir-resistant mucocutaneous herpes simplex virus infection in immunocompromised patients | | | X | | | |
| Prevention of CMV disease in transplant recipients at risk for CMV disease | | | | X | | |
| Prevention of CMV disease in high-risk patients (donor CMV seropositive/recipient CMV seronegative) undergoing solid organ transplant | | | | | | X |

# DOCUMENT ID: 83797_0 (688 tokens) 
---
title: Maribavir
author: Terri L Levien; Danial E Baker
date: 2022-12-21
---
Maribavir - PMC 
===============
Skip to main content

An official website of the United States government
Here's how you know
Here's how you know

Official websites use .gov
A .gov website belongs to an official government organization in the United States.

Secure .gov websites use HTTPS
A lock ( ) or https:// means you've safely connected to the .gov website. Share sensitive information only on official, secure websites.

Search 
Log in
 Dashboard
 Publications
 Account settings
 Log out 
Search... Search NCBI 
Primary site navigation
 Search 
Logged in as:

Dashboard
Publications
Account settings

Log in 

Search PMC Full-Text Archive 
Search in PMC

Advanced Search
Journal List
User Guide

New Try this search in PMC Beta Search

View on publisher site
Download PDF
Add to Collections
Cite
Permalink PERMALINK

Copy 
As a library, NLM provides access to scientific literature. Inclusion in an NLM database does not imply endorsement of, or agreement with, the contents by NLM or the National Institutes of Health.
Learn more: PMC Disclaimer | PMC Copyright Notice

Hosp Pharm
. 2022 Dec 21;58(4):336-344. doi: 10.1177/00185787221101480

Search in PMC
Search in PubMed
View in NLM Catalog
Add to search

Maribavir
Terri L Levien
Terri L Levien
1 Washington State University, Spokane, WA, USA
Find articles by Terri L Levien
1,[email], Danial E Baker
Danial E Baker
1 Washington State University, Spokane, WA, USA
Find articles by Danial E Baker
1

Author information
Article notes
Copyright and License information

1 Washington State University, Spokane, WA, USA
[email]
Terri L. Levien, Pharmacotherapy Department, College of Pharmacy and Pharmaceutical Sciences, Washington State University, 412 E. Spokane Falls Boulevard, Spokane, WA 99202-2131, USA. Email: levien

[DOCUMENT TEXT CLIPPED: omitted 524 characters; showing beginning and end.]

luation/medication use evaluation (DUE/MUE) is also provided each month. With a subscription, the monographs are available online to subscribers. Monographs can be customized to meet the needs of a facility. Through the cooperation of The Formulary, Hospital Pharmacy publishes selected reviews in this column. For more information about The Formulary Monograph Service, contact Wolters Kluwer customer service at 866-397-3433.
Keywords: drug information, formulary management/P & T, anti-infectives

# DOCUMENT ID: 83797_14 (413 tokens) 
No dosage adjustment is necessary in patients older than 65 years; in patients with mild, moderate, or severe renal impairment; or in patients with mild (Child-Pugh class A) or moderate (Child-Pugh class B) hepatic impairment. Administration of maribavir has not been studied in patients with end-stage renal disease, including patients on dialysis, or in patients with severe hepatic impairment.1
Product Availability and Storage
Maribavir was approved by the FDA on November 23, 2021.18 Maribavir is available as 200 mg tablets in bottles of 28 and 56.1
Store maribavir tablets at 20 degrees C to 25 degrees C (68 degrees F-77 degrees F); brief exposure to 15 degrees C to 30 degrees C (59 degrees F-86 degrees F) is permitted.1
Drug Safety/REMS
No REMS is required for maribavir.18
Conclusion
Maribavir, a benzimidazole antiviral, is indicated for the treatment of patients 12 years and older and weighing at least 35 kg with posttransplant CMV infection/disease that is refractory to treatment with ganciclovir, valganciclovir, foscarnet, or cidofovir (with or without genotypic resistance). Maribavir offers an oral treatment alternative with a unique mechanism of antiviral activity; however, cross-resistance may occur, and phenotyping is advised for patients who do not respond or who relapse during treatment. Screening for potential drug interactions is important before initiating therapy. The most common adverse event associated with maribavir is taste disturbance; neutropenia and renal toxicity occurred more frequently with comparator agents.
Footnotes
The author(s) declared no potential conflicts of interest with respect to the research, authorship, and/or publication of this article.
Funding: The author(s) received no financial support for the research, authorship, and/or publication of this article.
ORCID iDs: Terri L. Levien 
Danial E. Baker 
References
[Context: 14972/30720]

RETURN 0.metadata:
{
  "metadata": {
    "returned_chunk_ids": [
      "59631_1",
      "17183_0",
      "83797_16",
      "83797_1",
      "83797_0",
      "83797_14"
    ],
    "pre_rerank_chunk_ids": null
  }
}
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 4 working-memory snapshot after harness update}
pool_size: 9
curated_size: 9 / 30
importance_counts: very_high=0, high=4, fair=3, low=2
curated_set:
  - 17183 [high]
  - 25814 [high]
  - 59631 [high]
  - 83797 [high]
  - 15546 [fair]
  - 50858 [fair]
  - 73877 [fair]
  - 66387 [low]
  - 97801 [low]
\end{trajectorylisting}

\subsubsection*{Turn 5: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolNeutral}{Turn 5 model reasoning}
We've just found the fellowship-manual letter snippet for the FDA approval and stronger maribavir documents; the main unsolved gap is the Regulatory Project Manager name in the approval letter. The search angle worked - evidence for maribavir clarifies the drug and approval pathway - but I missed curation immediately after the last search, so we must curate the returned documents before any further search.
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 5 tool call(s)}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [
        "59631_0",
        "59631_1",
        "17183_0",
        "83797_0",
        "83797_1",
        "83797_16"
      ],
      "importance": {
        "59631_0": "high",
        "59631_1": "high",
        "17183_0": "high",
        "83797_0": "fair",
        "83797_1": "high",
        "83797_16": "low"
      }
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 5 tool return 0}
RETURN 0.text:
Curated set updated (9/30): 17183[high], 25814[high], 59631[high], 15546[fair], 50858[fair], 73877[fair], 66387[low], 83797[low], 97801[low]
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 5 working-memory snapshot after harness update}
pool_size: 9
curated_size: 9 / 30
importance_counts: very_high=0, high=3, fair=3, low=3
curated_set:
  - 17183 [high]
  - 25814 [high]
  - 59631 [high]
  - 15546 [fair]
  - 50858 [fair]
  - 73877 [fair]
  - 66387 [low]
  - 83797 [low]
  - 97801 [low]
\end{trajectorylisting}

\subsubsection*{Turn 6: \CaseTool{toolSearch}{search\_corpus}}
\begin{trajectorylisting}{toolNeutral}{Turn 6 model reasoning}
We have uncovered the drug and a likely approval letter, but the remaining gap is the exact Regulatory Project Manager name in that letter. The current angle via generic study/approval docs is exhausted; my last two searches were weak because they approached the match via drug constraints rather than the unique regulatory letter date clue. Let me backtrack: March 23 is likely the NDA received date and eight months later is the approval date in late November/early December. The missed facet is the Reg. Project Manager named in the FDA approval letter itself; grep on 'Regulatory Project Manager' or the month/date clue may surface the official approval notice or letter doc containing the contact.
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 6 tool call(s)}
[
  {
    "tool": "search_corpus",
    "params": {
      "query": "FDA approval letter regulatory project manager maribavir March 23 2021"
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 6 tool return 0}
RETURN 0.text:

# DOCUMENT ID: 72434_275 (707 tokens) 
refractory CMV infection and disease. The applicant provided a table that included the therapy, transplant type, mechanism of action, approved indications that were CMV-related, and the formulation(s).

With respect to the newness criterion, the applicant stated that LIVTENCITYTM

was granted Breakthrough Therapy, Priority Review, and Orphan Drug designations from FDA, and subsequently received FDA approval for its New Drug Application on November 23, 2021. LIVTENCITYTM

is indicated for the treatment of adults and pediatric patients (12 years of age or older and weighing at least 35 kg) with post-transplant CMV infection/disease that is refractory to treatment (with or without genotypic resistance) with ganciclovir, valganciclovir, cidofovir, or foscarnet. Per the applicant, LIVTENCITYTM

became commercially available on December 2, 2021. The applicant did not explain the reason for the delay between market authorization and commercial availability. The recommended dosing is 400 mg (two 200 mg tablets) orally twice daily with or without food. The applicant stated that if LIVTENCITY[TM]

is co-administered with carbamazepine, then the dosage is increased to 800 mg twice daily; if co-administered with phenytoin or phenobarbital, the dosage is increased to 1,200 mg twice daily.

According to the applicant, ICD-10-PCS code 3E0DX29 (Introduction of other anti-infective into mouth and pharynx, external approach) may be used to identify administration of LIVTENCITYTM

but does not uniquely identify it. The following ICD-10-PCS procedure codes were created to uniquely describe the use of LIVTENCITYTM, effective October 1, 2022: XW0DX38 (Introduction of

( printed page 48950)

maribavir anti-infective into mouth and pharynx, external approach, new technology group 8), XW0G738 (Introduction of maribavir anti-infective into upper gi, via n

[DOCUMENT TEXT CLIPPED: omitted 761 characters; showing beginning and end.]

resistant or refractory to conventional therapy. Specifically, LIVTENCITYTM

inhibits CMV DNA replication, encapsidation, and nuclear egress of viral capsids through inhibition of pUL97 and its natural substrates. The applicant provided the mechanisms of action for the other existing anti-CMV drugs, namely valganciclovir ganciclovir, foscarnet, and cidofovir in the table previously listed and concluded that LIVTENCITYTM

uses a different mechanism of action compared to existing anti-CMV drugs.

# DOCUMENT ID: 72434_274 (697 tokens) 
In its application, the applicant estimated that the cost of Hemolung RAS is $10,000, which includes the $7,500 cost of the cartridge and the $2,500 cost of the catheter. Under  412.88(a)(2), we limit new technology add-on payments to the lesser of 65% of the average cost of the technology, or 65% of the costs in excess of the MS-DRG payment for the case. As a result, the maximum new technology add-on payment for a case involving the use of Hemolung RAS is $6,500 for FY 2023.

d. LIVTENCITYTM

(Maribavir)

Takeda Pharmaceuticals U.S.A., Inc. submitted an application for new technology add-on payments for LIVTENCITYTM

(maribavir) for FY 2023. LIVTENCITYTM

is a cytomegalovirus (CMV) pUL97 kinase inhibitor indicated for the treatment of adults and pediatrics (12 years of age and older and weighing at least 35 kg) with post-transplant CMV infection/disease that is refractory to treatment (with or without genotypic resistance) to ganciclovir, valganciclovir, cidofovir, or foscarnet.

According to the applicant, LIVTENCITYTM

is the only antiviral therapy indicated to treat post-transplant patients with CMV in solid organ transplant (SOT) and hematopoietic stem cell transplant (HCT). Per the applicant, LIVTENCITYTM

provides multi-targeted anti-CMV activity by inhibiting protein kinase UL97 and its natural substrates, which subsequently inhibits CMV DNA replication, encapsidation, and nuclear egress of viral capsids.

The applicant stated that CMV is one of the most common viral infections experienced by transplant recipients, with an estimated incidence rate between 16%-56% in SOT recipients and 30%-70% in HCT recipients.[158]

CMV is a beta herpesvirus that commonly infects humans; serologic evidence of prior infection can be found in 40%-100% of various populations.[159]

CMV typically resides latent and asymptomatic in the body b

[DOCUMENT TEXT CLIPPED: omitted 580 characters; showing beginning and end.]

iclovir, foscarnet, and cidofovir. The applicant stated that ganciclovir and valganciclovir are approved for prevention of CMV disease in transplant recipients and for treatment of CMV retinitis in immunocompromised hosts, including those with Acquired Immune Deficiency Syndrome (AIDS); and foscarnet and cidofovir are approved for treatment of CMV retinitis in AIDS patients. Per the applicant, none of these four therapies are FDA-approved for the treatment of resistant or

( printed page 48949)

# DOCUMENT ID: 17183_11 (748 tokens) 
deoxynucleoside triphosphates by human CMV DNA polymerase. At a concentration of 100 uM, neither maribavir nor its 5' triphosphate derivative inhibited CMV DNA polymerase delta, however the 5'-monophosphate derivative inhibited incorporation by polymerase delta of all 4 natural dNTPs by approximately 55%. Antiviral Activity Maribavir inhibited human CMV replication in virus yield reduction, DNA hybridization, and plaque reduction assays in human lung fibroblast cell line (MRC-5), human embryonic kidney (HEK), and human foreskin fibroblast (MRHF) cells. The EC50 values ranged from 0.03 to 2.2 uM depending on the cell line and assay endpoint. The cell culture antiviral activity of maribavir has also been evaluated against CMV clinical isolates. The median EC50 values were 0.1 uM (n=10, range 0.03-0.13 uM) and 0.28 uM (n=10, range 0.12-0.56 uM) using DNA hybridization and plaque reduction assays, respectively. No significant difference in EC50 values across the four human CMV glycoprotein B genotypes (N = 2, 1, 4, and 1 for gB1, gB2, gB3, and gB4, respectively) was seen. 12 Reference ID: 4893709 This label may not be the latest approved by FDA. For current labeling information, please visit Combination Antiviral Activity When maribavir was tested in combination with other antiviral compounds, antagonism of the antiviral activity was seen in combination with ganciclovir. No antagonism was observed with cidofovir, foscarnet, letermovir and rapamycin at the drugs EC50 values. The pUL97 kinase activity inhibited by maribavir is necessary to activate valganciclovir/ganciclovir. Viral Resistance In Cell Culture Selection of maribavir resistant virus in cell culture and genotypic plus phenotypic characterization of these has identified amino acid substitutions that confer reduced susceptibility to maribavir. Substitutions identified in pUL9

[DOCUMENT TEXT CLIPPED: omitted 464 characters; showing beginning and end.]

ell transplant (HSCT) or solid organ transplant (SOT) recipients with phenotypic resistance to valganciclovir/ganciclovir, DNA sequence analysis of a select region of pUL97 (amino acids 270 to 482) and pUL27 (amino acids 108 to 424) was performed on 34 paired virologic failure samples. There were 25 patients with treatment-emergent maribavir resistance-associated substitution(s) in pUL97 F342Y (4.5-fold reduction in susceptibility), T409M (78-fold reduction), H411L/Y (69- and 12-fold reduction)

# DOCUMENT ID: 17183_7 (737 tokens) 
Pharmacology (12.3) and Clinical Studies (14)]. The safety and effectiveness of LIVTENCITY have not been established in children younger than 12 years of age. 8.5 Geriatric Use No dosage adjustment is required for patients over 65 years of age based on the results from population pharmacokinetics analysis [see Clinical Pharmacology (12.3)] and efficacy and safety data from the clinical studies. In the clinical Study 303, 54 patients aged 65 years and over were treated with LIVTENCITY. Safety, effectiveness, and pharmacokinetics were consistent between elderly patients (>=65 years) and younger patients (<65 years). 8.6 Impaired Renal Function No dose adjustment of LIVTENCITY is needed for patients with mild, moderate, or severe renal impairment [see Clinical Pharmacology (12.3)]. Administration of LIVTENCITY in patients with end stage renal disease (ESRD), including patients on dialysis, has not been studied. 8.7 Impaired Hepatic Function No dose adjustment of LIVTENCITY is needed for patients with mild (Child-Pugh Class A) or moderate (Child-Pugh Class B) hepatic impairment [see Clinical Pharmacology (12.3)]. Administration of LIVTENCITY in patients with severe hepatic impairment has not been studied. 10 OVERDOSAGE There is no known specific antidote for LIVTENCITY. In case of overdose, it is recommended that the patient be monitored for adverse reactions and appropriate symptomatic treatment instituted. Due to the high plasma protein binding of LIVTENCITY, dialysis is unlikely to reduce plasma concentrations of LIVTENCITY significantly. 11 DESCRIPTION LIVTENCITY tablets contain maribavir, a benzimidazole riboside CMV pUL97 protein kinase inhibitor. The chemical name of maribavir is 5,6-Dichloro-N-(1-methylethyl)-1--L-ribofuranosyl-1H-benzimidazol-2-amine and the structural formula is: The molecular formula for maribavir is C15H19C

[DOCUMENT TEXT CLIPPED: omitted 858 characters; showing beginning and end.]

03 that evaluated a maribavir dose of 400 mg twice daily, increasing maribavir exposure was not associated with increased probability of confirmed plasma CMV DNA < LLOQ (lower limit of quantification) at Week 8. Cardiac Electrophysiology At three times the recommended dose (approximately twice the peak concentration observed following the recommended dose), LIVTENCITY does not prolong the QT interval to any clinically relevant extent. 12.3 Pharmacokinetics LIVTENCITY pharmacological activity is

# DOCUMENT ID: 59631_2 (760 tokens) 
Cytomegalovirus (CMV) Infections that are Refractory or Resistant to Treatment with Ganciclovir, Valganciclovir, Foscarnet, or Cidofovir." The timetable you submitted on November 8, 2021, states that you will conduct this study according to the following schedule: Final Protocol Submission: 01/2022 Study Completion: 03/2022 Final Report Submission: 04/2022 Reference ID: 4893709 NDA 215596 Page 4 U.S. Food and Drug Administration Silver Spring, MD 20993  FDA considers the term final to mean that the applicant has submitted a protocol, the FDA review team has sent comments to the applicant, and the protocol has been revised as needed to meet the goal of the study or clinical trial.3 Submit clinical protocol(s) to your IND 051001 with a cross-reference letter to this NDA. Submit nonclinical and chemistry, manufacturing, and controls protocols and all final report(s) to your NDA. Prominently identify the submission with the following wording in bold capital letters at the top of the first page of the submission, as appropriate: Required Postmarketing Protocol Under 505(o), Required Postmarketing Final Report Under 505(o), Required Postmarketing Correspondence Under 505(o). Section 505(o)(3)(E)(ii) of the FDCA requires you to report periodically on the status of any study or clinical trial required under this section. This section also requires you to periodically report to FDA on the status of any study or clinical trial otherwise undertaken to investigate a safety issue. Section 506B of the FDCA, as well as 21 CFR 314.81(b)(2)(vii) requires you to report annually on the status of any postmarketing commitments or required studies or clinical trials. FDA will consider the submission of your annual report under section 506B and 21 CFR 314.81(b)(2)(vii) to satisfy the periodic reporting requirement under section 505(o)(3)(E)(ii) provided

[DOCUMENT TEXT CLIPPED: omitted 935 characters; showing beginning and end.]

tes that you will conduct this study according to the following schedule: Trial Completion: 11 /2022 Final Report Submission: 05 /2023 3 See the guidance for Industry Postmarketing Studies and Clinical Trials-Implementation of Section 505(o)(3) of the Federal Food, Drug, and Cosmetic Act (October 2019). Reference ID: 4893709 NDA 215596 Page 5 U.S. Food and Drug Administration Silver Spring, MD 20993  A final submitted protocol is one that the FDA has reviewed and commented
[Context: 15260/30720]

RETURN 0.metadata:
{
  "metadata": {
    "returned_chunk_ids": [
      "72434_275",
      "72434_274",
      "17183_11",
      "17183_7",
      "59631_2"
    ],
    "pre_rerank_chunk_ids": null
  }
}
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 6 working-memory snapshot after harness update}
pool_size: 10
curated_size: 9 / 30
importance_counts: very_high=0, high=3, fair=3, low=3
curated_set:
  - 17183 [high]
  - 25814 [high]
  - 59631 [high]
  - 15546 [fair]
  - 50858 [fair]
  - 73877 [fair]
  - 66387 [low]
  - 83797 [low]
  - 97801 [low]
\end{trajectorylisting}

\subsubsection*{Turn 7: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolNeutral}{Turn 7 model reasoning}
We just searched the regulatory letter date facet and found several maribavir/Civtencity related approvals/documents, including FDA approval letter style documents. The gap still is the exact Regulatory Project Manager name, but candidates themselves are not expected here because we just searched; my current angle on approval-letter specific dates is weak because it kept returning generic Socrata/documents rather than the letter itself, but some docs are plausibly relevant to the approval and study/date facets. I am curating immediately per the rhythm before any new search.
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 7 tool call(s)}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [
        "72434_275",
        "72434_274",
        "59631_2",
        "59631_0",
        "59631_1"
      ],
      "importance": {
        "72434_275": "fair",
        "72434_274": "low",
        "59631_2": "fair",
        "59631_0": "high",
        "59631_1": "high"
      }
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 7 tool return 0}
RETURN 0.text:
Curated set updated (10/30): 17183[high], 25814[high], 59631[high], 15546[fair], 50858[fair], 73877[fair], 66387[low], 72434[low], 83797[low], 97801[low]
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 7 working-memory snapshot after harness update}
pool_size: 10
curated_size: 10 / 30
importance_counts: very_high=0, high=3, fair=3, low=4
curated_set:
  - 17183 [high]
  - 25814 [high]
  - 59631 [high]
  - 15546 [fair]
  - 50858 [fair]
  - 73877 [fair]
  - 66387 [low]
  - 72434 [low]
  - 83797 [low]
  - 97801 [low]
\end{trajectorylisting}

\subsubsection*{Turn 8: \CaseTool{toolGrep}{grep\_corpus}}
\begin{trajectorylisting}{toolNeutral}{Turn 8 model reasoning}
We have maribavir/Civtencity and approval quote docs, but the last search angle via March 23 dates was exhausted: it produced generic approval-documents and not the exact regulatory letter name. The missed facet is the letter itself and the Regulatory Project Manager contact line. I am choosing grep now because the query asks for an exact person/date phrase in an FDA letter, and grep is best for specific names/dates rather than broad document searching.
\end{trajectorylisting}

\begin{trajectorylisting}{toolGrep}{Turn 8 tool call(s)}
[
  {
    "tool": "grep_corpus",
    "params": {
      "pattern": "Maribavir.*Regulatory Project Manager"
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolGrep}{Turn 8 tool return 0}
RETURN 0.text:
No results found
[Context: 11553/30720]

RETURN 0.metadata:
{
  "metadata": {
    "returned_chunk_ids": []
  }
}
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 8 working-memory snapshot after harness update}
pool_size: 10
curated_size: 10 / 30
importance_counts: very_high=0, high=3, fair=3, low=4
curated_set:
  - 17183 [high]
  - 25814 [high]
  - 59631 [high]
  - 15546 [fair]
  - 50858 [fair]
  - 73877 [fair]
  - 66387 [low]
  - 72434 [low]
  - 83797 [low]
  - 97801 [low]
\end{trajectorylisting}

\subsubsection*{Turn 9: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolNeutral}{Turn 9 model reasoning}
I just used grep and got no results, which is likely because the regex misspecification landed in non-terminology or a different doc. The key missed facet remains the exact FDA approval letter, especially the Regulatory Project Manager contact. What isn't working: the Messearch failed because the last 2 searches were generic review-letter/date/documents, so that angle looks exhausted. Re-reading the query: the last facet is the specific letter produced eight months after the March 23 application, which points to a letter likely labeled with NDA 215596 and containing a Regulatory Project Manager name. I need to curate now because I just searched via grep and must follow the required rhythm before trying another angle.
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 9 tool call(s)}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [],
      "remove_ids": [],
      "importance": {}
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 9 tool return 0}
RETURN 0.text:
Curated set updated (10/30): 17183[high], 25814[high], 59631[high], 15546[fair], 50858[fair], 73877[fair], 66387[low], 72434[low], 83797[low], 97801[low]
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 9 working-memory snapshot after harness update}
pool_size: 10
curated_size: 10 / 30
importance_counts: very_high=0, high=3, fair=3, low=4
curated_set:
  - 17183 [high]
  - 25814 [high]
  - 59631 [high]
  - 15546 [fair]
  - 50858 [fair]
  - 73877 [fair]
  - 66387 [low]
  - 72434 [low]
  - 83797 [low]
  - 97801 [low]
\end{trajectorylisting}

\subsubsection*{Turn 10: \CaseTool{toolSearch}{search\_corpus}}
\begin{trajectorylisting}{toolNeutral}{Turn 10 model reasoning}
The current search angle via dates and generic approval docs is exhausted. Re-reading the query, the unique facet we still need is the exact FDA approval letter containing the Regulatory Project Manager name and contact line. The missed facet is that the regulator letter is likely an FDA "Letter of Approval" for NDA 215596; the name hasn't emerged yet because prior searches were on product indications, author-studies, and approval-date documents. My current search angle is exhausted. Let me rethink. A completely different strategy is to search the full approval letter itself, using the NDA number/date plus regulator contact phrasing.
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 10 tool call(s)}
[
  {
    "tool": "search_corpus",
    "params": {
      "query": "NDA 215596 letter to maribavir regulatory project manager NDA 215596"
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 10 tool return 0}
RETURN 0.text:

# DOCUMENT ID: 83797_10 (708 tokens) 
Comments: The study was conducted at 101 sites in 12 countries. A multicenter, randomized, double-dummy, active-controlled study comparing maribavir with valganciclovir for the treatment of nonresistant or nonrefractory CMV infection in HSCT recipients is underway, with a scheduled study completion date of November 2022.18
A phase 2, randomized, double-blind study of 120 HSCT or solid organ transplant recipients with CMV infection refractory or resistant to at least one antiviral agent evaluated maribavir 400, 800, and 1200 mg doses administered twice daily for up to 24 weeks. Undetectable CMV DNA was reached within 6 weeks of treatment initiation in 80 of 120 patients (67%; 95% CI, 57% to 75%), with rates of 70% for maribavir 400 mg, 63% for maribavir 800 mg, and 68% for maribavir 120 mg.22
Another phase 2, randomized, open-label study of 161 HSCT or solid organ transplant recipients with CMV reactivation (but not refractory or resistant CMV) evaluated maribavir 400, 800, and 1200 mg doses administered twice daily compared with valganciclovir for up to 12 weeks. Undetectable CMV DNA in plasma was achieved within 3 weeks of treatment initiation in 62% of patients treated with maribavir and 56% treated with valganciclovir, and within 6 weeks in 79% and 67%, respectively. Serious adverse events and adverse events prompting discontinuation of treatment were more common in the maribavir group.23 Experience in a small number of patients treated with maribavir under individual emergency investigational New Drug Applications has also been described, with 4 of 6 patients achieving undetectable CMV DNA levels within 6 weeks of starting maribavir therapy.24
Results of a phase 2 CMV prophylaxis study suggested efficacy with maribavir compared with placebo in CMV-seropositive allogeneic stem cell transplant recipients. However, in phase 3 CMV

[DOCUMENT TEXT CLIPPED: omitted 659 characters; showing beginning and end.]

r any of its inactive ingredients (ie, FD&C Blue No. 1, magnesium stearate, microcrystalline cellulose, polyethylene glycol, polyvinyl alcohol, sodium starch glycolate, titanium dioxide, talc).1
Warnings and Precautions
Maribavir may antagonize the antiviral activity of ganciclovir and valganciclovir by inhibiting CMV pUL97 kinase, which is required for the activation/phosphorylation of these antiviral agents. Coadministration of maribavir with ganciclovir or valganciclovir is not recommended.1

# DOCUMENT ID: 59631_3 (605 tokens) 
upon, and you have revised as needed to meet the goal of the study or clinical trial. Submit clinical protocols to your IND 051001 for this product. Submit nonclinical and chemistry, manufacturing, and controls protocols and all postmarketing final reports to this NDA. In addition, under 21 CFR 314.81(b)(2)(vii) and 314.81(b)(2)(viii) you should include a status summary of each commitment in your annual report to this NDA. The status summary should include expected summary completion and final report submission dates, any changes in plans since the last annual report, and, for clinical studies/trials, number of patients entered into each study/trial. All submissions, including supplements, relating to these postmarketing commitments should be prominently labeled "Postmarketing Commitment Protocol," "Postmarketing Commitment Final Report," or "Postmarketing Commitment Correspondence." PROMOTIONAL MATERIALS You may request advisory comments on proposed introductory advertising and promotional labeling. For information about submitting promotional materials, see the final guidance for industry Providing Regulatory Submissions in Electronic and Non-Electronic Format-Promotional Labeling and Advertising Materials for Human Prescription Drugs.4 As required under 21 CFR 314.81(b)(3)(i), you must submit final promotional materials, and the Prescribing Information, at the time of initial dissemination or publication, accompanied by a Form FDA 2253. Form FDA 2253 is available at FDA.gov.5 Information and Instructions for completing the form can be found at FDA.gov.6 REPORTING REQUIREMENTS We remind you that you must comply with reporting requirements for an approved NDA (21 CFR 314.80 and 314.81). POST APPROVAL FEEDBACK MEETING New molecular entities qualify for a post approval feedback meeting. Such meetings are used to discuss the quality

[DOCUMENT TEXT CLIPPED: omitted 736 characters; showing beginning and end.]

ice of Infectious Diseases Office of New Drugs Center for Drug Evaluation and Research ENCLOSURE(S): - Content of Labeling o Prescribing Information o Patient Package Insert - Carton and Container Labeling Reference ID: 4893709 --------------------------------------------------------------------------------------------This is a representation of an electronic record that was signed electronically. Following this are manifestations of any and all electronic signatures for this electronic record.

# DOCUMENT ID: 73877_0 (719 tokens) 
---
title: maribavir (Rx)
date: 2025-01-01
---
Dosing & Uses

Dosage Forms & Strengths

tablet

- 200mg

Cytomegalovirus Infection

Indicated for treatment of posttransplant CMV infection/disease that is refractory to treatment with or without genotypic resistance (eg, ganciclovir, valganciclovir, cidofovir, foscarnet) in adults and pediatric patients aged >=12 years who weigh >=35 kg

400 mg PO BID with or without food

Dosage Modifications

Coadministration with anticonvulsants

- Coadministered with carbamazepine: Increase dose to 800 mg PO BID

- Coadministered with phenytoin or phenobarbital: Increase dosage to 1,200 mg PO BID

Renal impairment

- Mild-to-severe (CrCl 12-70 mL/min): No dosage adjustment necessary

- End-stage renal disease: Not studied

Hepatic impairment

- Mild-to-moderate (Child-Pugh A or B): No dosage adjustment necessary

- Severe (Child-Pugh C): Not studied

Dosage Forms & Strengths

tablet

- 200mg

Cytomegalovirus Infection

Indicated for treatment of posttransplant CMV infection/disease that is refractory to treatment with or without genotypic resistance (eg, ganciclovir, valganciclovir, cidofovir, foscarnet) in adults and pediatric patients aged >=12 years who weigh >=35 kg

400 mg PO BID with or without food

Dosage Modifications

Coadministration with anticonvulsants

- Coadministered with carbamazepine: Increase dose to 800 mg PO BID

- Coadministered with phenytoin or phenobarbital: Increase dosage to 1,200 mg PO BID

Renal impairment

- Mild-to-severe (CrCl 12-70 mL/min): No dosage adjustment necessary

- End-stage renal disease: Not studied

Hepatic impairment

- Mild-to-moderate (Child-Pugh A or B): No dosage adjustment necessary

- Severe (Child-Pugh C): Not studied

Adverse Effects

>10%

*Denotes incidence slightly less than investigator-assigned treatment that was compared with maribavir

Taste disturbance (46%)

Creatinine >=1.5 to <2.5 mg/dL (33%)

Hemoglobin >=8 to <9.5 g/dL (32%)

Nausea (21%)*

Diarrhea (19%)*

Platelet cell count >=50,000 to <100,000 cells/uL (18%)

Hemoglobin >=6.5 to <8 g/dL (15%)

Vomiting (14%)*

Fatigue (12%)

Platelet cell count >=25,000 to <50,000 cells/uL (12%)

1-10%

Creatinine >2.5 mg/dL (7%)

Platelet cell count <25,000 cells/uL (5%)

Neutrophils >=750 to <1,000 cells/uL (4%)

Neutrophils >=500 to <750 cells/uL (3%)

Neutrophils <500 cells/uL (2%)

Hemoglobin <6.5 g/dL (1%)

Warnings

Contraindications

None

Cautions

# DOCUMENT ID: 83797_11 (720 tokens) 
Virologic failure due to resistance can occur during or after therapy with maribavir. Virologic relapse during the posttreatment period has generally occurred within 4 to 8 weeks after treatment discontinuation. Some maribavir pUL97 resistance-associated substitutions confer cross-resistance to ganciclovir and valganciclovir. If a patient relapses or is not responding to treatment, monitor CMV DNA levels and check for maribavir resistance.1
Drug interactions may result in reduced therapeutic effect of maribavir or adverse reactions of concomitant drugs. Concomitant medication must be reviewed during therapy, and dosing recommendations must be followed to prevent or manage potential drug interactions (see Drug Interactions section). Maribavir is primarily metabolized by CYP3A4. Drugs that are strong inducers of CYP3A4 are expected to decrease maribavir concentrations and result in reduced virologic response. Coadministration with strong inducers should be avoided, except for select anticonvulsants for which dosing recommendations are available.1
Maribavir has the potential to increase the concentrations of immunosuppressant drugs that are CYP3A4 and/or P-gp substrates (eg, tacrolimus, cyclosporine, sirolimus, everolimus) for which minimal concentration changes could lead to serious adverse events. Immunosuppressant drug levels should be monitored frequently during maribavir therapy, especially during initiation and after discontinuation of maribavir, and immunosuppressant doses should be adjusted as needed.1,28
There are no adequate and well-controlled studies of maribavir use during pregnancy. In some animal reproduction studies, embryo-fetal survival was decreased at maribavir exposures less than those observed in humans at the recommended human dose.1
Caution should be used when administering maribavir to a breastfeeding patient

[DOCUMENT TEXT CLIPPED: omitted 1125 characters; showing beginning and end.]

ared with IAT (consisting of monotherapy or dual therapy with ganciclovir, valganciclovir, foscarnet, or cidofovir). Taste disturbance occurred in 46% of patients treated with maribavir. Taste disturbance resolved during therapy in 37% of these patients (median duration, 43 days; range, 7-59 days). For the patients with ongoing taste disturbance after maribavir discontinuation, resolution occurred in 89%; median duration of symptoms after discontinuation was 6 days (range, 2-85 days).1
Table 2.

# DOCUMENT ID: 99609_0 (738 tokens) 
---
title: New Drug Application (NDA)
date: 2022-01-21
---
New Drug Application (NDA)

Introduction

For decades, the regulation and control of new drugs in the United States has been based on the New Drug Application (NDA). Since 1938, every new drug has been the subject of an approved NDA before U.S. commercialization. The NDA application is the vehicle through which drug sponsors formally propose that the FDA approve a new pharmaceutical for sale and marketing in the U.S. The data gathered during the animal studies and human clinical trials of an Investigational New Drug (IND) become part of the NDA.

The goals of the NDA are to provide enough information to permit FDA reviewer to reach the following key decisions:

- Whether the drug is safe and effective in its proposed use(s), and whether the benefits of the drug outweigh the risks.

- Whether the drug's proposed labeling (package insert) is appropriate, and what it should contain.

- Whether the methods used in manufacturing the drug and the controls used to maintain the drug's quality are adequate to preserve the drug's identity, strength, quality, and purity.

The documentation required in an NDA is supposed to tell the drug's whole story, including what happened during the clinical tests, what the ingredients of the drug are, the results of the animal studies, how the drug behaves in the body, and how it is manufactured, processed and packaged. The following resources provide summaries on NDA content, format, and classification, plus the NDA review process:

Resources for NDA Submissions

The following resources have been gathered to provide you with the legal requirements of a new drug application, assistance from CDER to help you meet those requirements, and internal NDA review principles, policies and procedures.

Guidance Documents for NDAs

Guidance documents represe

[DOCUMENT TEXT CLIPPED: omitted 1498 characters; showing beginning and end.]

ent of the Summary for New Drug and Antibiotic Applications

- Formatting, Assembling and Submitting New Drug and Antibiotic Applications,

- GUIDELINE FOR SUBMITTING SUPPORTING DOCUMENTATION IN DRUG APPLICATIONS FOR THE MANUFACTURE OF DRUG PRODUCTS

- NDAs: Impurities in Drug Substances

- Format and Content of the Human Pharmacokinetics and Bioavailability Section of an Application

- Format and Content of the Nonclinical Pharmacology/Toxicology Section of an Application
[Context: 11262/30720]

RETURN 0.metadata:
{
  "metadata": {
    "returned_chunk_ids": [
      "83797_10",
      "59631_3",
      "73877_0",
      "83797_11",
      "99609_0"
    ],
    "pre_rerank_chunk_ids": null
  }
}
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 10 working-memory snapshot after harness update}
pool_size: 11
curated_size: 10 / 30
importance_counts: very_high=0, high=3, fair=3, low=4
curated_set:
  - 17183 [high]
  - 25814 [high]
  - 59631 [high]
  - 15546 [fair]
  - 50858 [fair]
  - 73877 [fair]
  - 66387 [low]
  - 72434 [low]
  - 83797 [low]
  - 97801 [low]
\end{trajectorylisting}

\subsubsection*{Turn 11: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolNeutral}{Turn 11 model reasoning}
The last search was via NDA/letter facet and found a partially relevant approval/contact document plus a monitor of the previously found drug result. What isn't working: we still haven't zeroed in the exact approval letter with the Regulatory Project Manager contact line. What is missing explicitly is whether the front-loader search term NDA 215596 returned the full approval letter form; the last result 59631_3 looks like it already contains the contact line, which is likely the answer doc. I am curating now before any further search, per the required rhythm, and highlighting the plausibly relevant letter/document.
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 11 tool call(s)}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [
        "59631_3",
        "59631_0",
        "59631_1"
      ],
      "remove_ids": [],
      "importance": {
        "59631_3": "high",
        "59631_0": "fair",
        "59631_1": "fair"
      }
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 11 tool return 0}
RETURN 0.text:
Curated set updated (10/30): 17183[high], 25814[high], 15546[fair], 50858[fair], 59631[fair], 73877[fair], 66387[low], 72434[low], 83797[low], 97801[low]
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 11 working-memory snapshot after harness update}
pool_size: 11
curated_size: 10 / 30
importance_counts: very_high=0, high=2, fair=4, low=4
curated_set:
  - 17183 [high]
  - 25814 [high]
  - 15546 [fair]
  - 50858 [fair]
  - 59631 [fair]
  - 73877 [fair]
  - 66387 [low]
  - 72434 [low]
  - 83797 [low]
  - 97801 [low]
\end{trajectorylisting}

\subsubsection*{Turn 12: \CaseTool{toolRead}{read\_document}}
\begin{trajectorylisting}{toolNeutral}{Turn 12 model reasoning}
We have a solid candidate letter/document already in the curated set that likely contains the Regulatory Project Manager line. The main gap is to confirm its completeness and extract the full name as stated. The current angle on general NDA/letter terms is not working because we still need a more precise grasp of the exact document text/location. What isn't working: repeated letter searches by general NDA term are exhausted; the missed facet is that the query explicitly calls for the letter, so maybe searching the exact regulatory phrase directly in the document or extracting from the letter itself is better than searching a new doc. I'm choosing read_document on the most plausible doc to confirm/locate the exact contact line.
\end{trajectorylisting}

\begin{trajectorylisting}{toolRead}{Turn 12 tool call(s)}
[
  {
    "tool": "read_document",
    "params": {
      "doc_id": "59631_3"
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolRead}{Turn 12 tool return 0}
RETURN 0.text:
# Document (2903 tokens)
CENTER FOR DRUG EVALUATION AND RESEARCH Approval Package for: APPLICATION NUMBER: 215596Orig1s000 Trade Name: LIVTENCITY oral tablets Generic or Proper Name: maribavir Sponsor: Takeda Pharmaceuticals USA, Inc. Approval Date: November 23, 2021 Indication: For the treatment of adults and pediatric patients 12 years of age and older and weighing at least 35 kg with post-transplant cytomegalovirus (CMV) infection/disease that is refractory to treatment (with or without genotypic resistance) with ganciclovir, valganciclovir, cidofovir or foscarnet. CENTER FOR DRUG EVALUATION AND RESEARCH 215596Orig1s000 CONTENTS Reviews / Information Included in this NDA Review. Approval Letter X Other Action Letters Labeling X REMS Officer/Employee List X Integrated Review(s) X Product Quality Review(s) X Other Reviews X Risk Assessment and Risk Mitigation Review(s) X Proprietary Name Review(s) X Administrative/Correspondence Document(s) X CENTER FOR DRUG EVALUATION AND RESEARCH APPLICATION NUMBER: 215596Orig1s000 APPROVAL LETTER NDA 215596 NDA APPROVAL Takeda Pharmaceuticals USA, Inc. Attention: Michael A. Cronin, PharmD Director, Global Regulatory Affairs 650 East Kendall Street Cambridge, MA 02142 Dear Dr. Cronin: Please refer to your new drug application (NDA) dated and received on March 23, 2021, and your amendments, submitted under section 505(b) of the Federal Food, Drug, and Cosmetic Act (FDCA) for Livtencity (maribavir) oral tablets. This NDA provides for the use of Livtencity (maribavir) oral tablets for the treatment of adults and pediatric patients 12 years of age and older and weighing at least 35 kg with post-transplant cytomegalovirus (CMV) infection/disease that is refractory to treatment (with or without genotypic resistance) with ganciclovir, valganciclovir, cidofovir or foscarnet. We have completed our review of this application, as amended. It is approved, effective on the date of this letter, for use as recommended in the enclosed agreed-upon labeling. CONTENT OF LABELING As soon as possible, but no later than 14 days from the date of this letter, submit the content of labeling [21 CFR 314.50(l)] in structured product labeling (SPL) format using the FDA automated drug registration and listing system (eLIST), as described at FDA.gov.1 Content of labeling must be identical to the enclosed labeling (Prescribing Information and Patient Package Insert) as well as annual reportable changes not included in the enclosed labeling. Information on submitting SPL files using eLIST may be found in the guidance for industry SPL Standard for Content of Labeling Technical Qs and As.2 The SPL will be accessible via publicly available labeling repositories. 1 2 We update guidances periodically. For the most recent version of a guidance, check the FDA Guidance Documents Database Reference ID: 4893709 NDA 215596 Page 2 U.S. Food and Drug Administration Silver Spring, MD 20993  CARTON AND CONTAINER LABELING Submit final printed carton and container labeling that are identical to the enclosed carton and container labeling as soon as they are available, but no more than 30 days after they are printed. Please submit these labeling electronically according to the guidance for industry Providing Regulatory Submissions in Electronic Format - Certain Human Pharmaceutical Product Applications and Related Submissions Using theeCTD Specifications. For administrative purposes, designate this submission "Final Printed Carton and Container Labeling for approved NDA 215596." Approval of this submission by FDA is not required before the labeling is used. DATING PERIOD Based on the stability data submitted to date, the expiry dating period for Livtencity (maribavir) tablets shall be 30 months from the date of manufacture when stored at 20 degrees C to 25 degrees C (68 degrees F to 77 degrees F). Results of ongoing stability should be submitted throughout the dating period in your annual report, as they become available, including the results of stability studies from the first three production lots. REQUIRED PEDIATRIC ASSESSMENTS Under the Pediatric Research Equity Act (PREA) (21 U.S.C. 355c), all applications for new active ingredients (which includes new salts and new fixed combinations), new indications, new dosage forms, new dosing regimens, or new routes of administration are required to contain an assessment of the safety and effectiveness of the product for the claimed indication in pediatric patients unless this requirement is waived, deferred, or inapplicable Because this drug product for this indication has an orphan drug designation, you are exempt from this requirement. POSTMARKETING REQUIREMENTS UNDER 505(o) Section 505(o)(3) of the Federal Food, Drug, and Cosmetic Act (FDCA) authorizes FDA to require holders of approved drug and biological product applications to conduct postmarketing studies and clinical trials for certain purposes, if FDA makes certain findings required by the statute. We have determined that an analysis of spontaneous postmarketing adverse events reported under subsection 505(k)(1) of the FDCA will not be sufficient to assess a signal of serious risk of virologic failure due to resistance to maribavir. Reference ID: 4893709 NDA 215596 Page 3 U.S. Food and Drug Administration Silver Spring, MD 20993  Furthermore, the active postmarket risk identification and analysis system as available under section 505(k)(3) of the FDCA will not be sufficient to assess this serious risk. Therefore, based on appropriate scientific data, FDA has determined that you are required to conduct the following studies: 4182-1 Conduct phenotypic analysis of maribavir against human cytomegalovirus carrying the following substitutions: - High priority: pUL97 M460I/T, A594E/P/T/V, L595F/W, C603R/W/Y - Medium priority: pUL97 A440V, V466M, A591V, E596G, K599E, C607F/Y - Low priority: o pUL97 P132L, L405P, C518Y , I610T, A613V o pUL27 P10L, N289D, H297Y, D298G, N300G, P307L,V310A, D351N, I367V o pUL54 S290R, K475S The timetable you submitted on November 8, 2021, states that you will conduct this study according to the following schedule: Final Protocol Submission: 01/2022 High Priority Phenotyping Submission: 06/2023 Medium/low Priority Phenotyping Submission: 12/2023 Study Completion: 12/2023 Final Report Submission: 01/2024 4182-2 Determine the human cytomegalovirus gB subtype for each of the subjects in study SHP620-303 "A Phase 3, Multicenter, Randomized, Open-label, Active controlled Study to Assess the Efficacy and Safety of Maribavir Treatment Compared to Investigator assigned Treatment in Transplant Recipients withCytomegalovirus (CMV) Infections that are Refractory or Resistant to Treatment with Ganciclovir, Valganciclovir, Foscarnet, or Cidofovir." The timetable you submitted on November 8, 2021, states that you will conduct this study according to the following schedule: Final Protocol Submission: 01/2022 Study Completion: 03/2022 Final Report Submission: 04/2022 Reference ID: 4893709 NDA 215596 Page 4 U.S. Food and Drug Administration Silver Spring, MD 20993  FDA considers the term final to mean that the applicant has submitted a protocol, the FDA review team has sent comments to the applicant, and the protocol has been revised as needed to meet the goal of the study or clinical trial.3 Submit clinical protocol(s) to your IND 051001 with a cross-reference letter to this NDA. Submit nonclinical and chemistry, manufacturing, and controls protocols and all final report(s) to your NDA. Prominently identify the submission with the following wording in bold capital letters at the top of the first page of the submission, as appropriate: Required Postmarketing Protocol Under 505(o), Required Postmarketing Final Report Under 505(o), Required Postmarketing Correspondence Under 505(o). Section 505(o)(3)(E)(ii) of the FDCA requires you to report periodically on the status of any study or clinical trial required under this section. This section also requires you to periodically report to FDA on the status of any study or clinical trial otherwise undertaken to investigate a safety issue. Section 506B of the FDCA, as well as 21 CFR 314.81(b)(2)(vii) requires you to report annually on the status of any postmarketing commitments or required studies or clinical trials. FDA will consider the submission of your annual report under section 506B and 21 CFR 314.81(b)(2)(vii) to satisfy the periodic reporting requirement under section 505(o)(3)(E)(ii) provided that you include the elements listed in 505(o) and 21 CFR 314.81(b)(2)(vii). We remind you that to comply with 505(o), your annual report must also include a report on the status of any study or clinical trial otherwise undertaken to investigate a safety issue. Failure to submit an annual report for studies or clinical trials required under 505(o) on the date required will be considered a violation of FDCA section 505(o)(3)(E)(ii) and could result in enforcement action. POSTMARKETING COMMITMENTS SUBJECT TO REPORTING REQUIREMENTS UNDER SECTION 506B We remind you of your postmarketing commitments: 4182-3 A Multicenter, Randomized, Double-blind, Double dummy, Active- controlled Study to Assess the Efficacy and Safety of Maribavir Compared to Valganciclovir for the Treatment of Cytomegalovirus (CMV) Infection in Hematopoietic Stem Cell Transplant Recipients (NCT02927067). The timetable you submitted on September 21, 2021, states that you will conduct this study according to the following schedule: Trial Completion: 11 /2022 Final Report Submission: 05 /2023 3 See the guidance for Industry Postmarketing Studies and Clinical Trials-Implementation of Section 505(o)(3) of the Federal Food, Drug, and Cosmetic Act (October 2019). Reference ID: 4893709 NDA 215596 Page 5 U.S. Food and Drug Administration Silver Spring, MD 20993  A final submitted protocol is one that the FDA has reviewed and commentedupon, and you have revised as needed to meet the goal of the study or clinical trial. Submit clinical protocols to your IND 051001 for this product. Submit nonclinical and chemistry, manufacturing, and controls protocols and all postmarketing final reports to this NDA. In addition, under 21 CFR 314.81(b)(2)(vii) and 314.81(b)(2)(viii) you should include a status summary of each commitment in your annual report to this NDA. The status summary should include expected summary completion and final report submission dates, any changes in plans since the last annual report, and, for clinical studies/trials, number of patients entered into each study/trial. All submissions, including supplements, relating to these postmarketing commitments should be prominently labeled "Postmarketing Commitment Protocol," "Postmarketing Commitment Final Report," or "Postmarketing Commitment Correspondence." PROMOTIONAL MATERIALS You may request advisory comments on proposed introductory advertising and promotional labeling. For information about submitting promotional materials, see the final guidance for industry Providing Regulatory Submissions in Electronic and Non-Electronic Format-Promotional Labeling and Advertising Materials for Human Prescription Drugs.4 As required under 21 CFR 314.81(b)(3)(i), you must submit final promotional materials, and the Prescribing Information, at the time of initial dissemination or publication, accompanied by a Form FDA 2253. Form FDA 2253 is available at FDA.gov.5 Information and Instructions for completing the form can be found at FDA.gov.6 REPORTING REQUIREMENTS We remind you that you must comply with reporting requirements for an approved NDA (21 CFR 314.80 and 314.81). POST APPROVAL FEEDBACK MEETING New molecular entities qualify for a post approval feedback meeting. Such meetings are used to discuss the quality of the application and to evaluate the communication process during drug development and marketing application review. The purpose is to 4 For the most recent version of a guidance, check the FDA guidance web page at 5 6 Reference ID: 4893709 NDA 215596 Page 6 U.S. Food and Drug Administration Silver Spring, MD 20993  learn from successful aspects of the review process and to identify areas that could benefit from improvement. If you would like to have such a meeting with us, call the Regulatory Project Manager for this application. If you have any questions, call Alicia Moruf, PharmD, MPH, RAC-US, Regulatory Project Manager, at 301-796-3953. Sincerely, {See appended electronic signature page} John Farley, MD, MPH Director Office of Infectious Diseases Office of New Drugs Center for Drug Evaluation and Research ENCLOSURE(S): - Content of Labeling o Prescribing Information o Patient Package Insert - Carton and Container Labeling Reference ID: 4893709 --------------------------------------------------------------------------------------------This is a representation of an electronic record that was signed electronically. Following this are manifestations of any and all electronic signatures for this electronic record.--------------------------------------------------------------------------------------------/s/ ------------------------------------------------------------JOHN J FARLEY 11/23/2021 03:34:13 PM Signature Page 1 of 1 Reference ID: 4893709 (
[Context: 10329/30720]
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 12 working-memory snapshot after harness update}
pool_size: 11
curated_size: 10 / 30
importance_counts: very_high=0, high=2, fair=4, low=4
curated_set:
  - 17183 [high]
  - 25814 [high]
  - 15546 [fair]
  - 50858 [fair]
  - 59631 [fair]
  - 73877 [fair]
  - 66387 [low]
  - 72434 [low]
  - 83797 [low]
  - 97801 [low]
\end{trajectorylisting}

\subsubsection*{Turn 13: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolNeutral}{Turn 13 model reasoning}
I just read a document but the missing step is the required curate after that search/read cycle. We found the exact approval letter text and confirmed contact line with Regulatory Project Manager, which is the key facet we needed; this read itself counts as the last search results because it revealed the matching doc. The key remaining gap is just extracting the full name aloud, but for retrieval the curated document is enough. What isn't working: current angle via date and approval docs is exhausted; we need to cement the key document rather than find another one. Re-reading is no longer needed. I am curating the exact approval letter doc now before any further search.
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 13 tool call(s)}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [
        "59631_3"
      ],
      "remove_ids": [],
      "importance": {
        "59631_3": "high"
      }
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 13 tool return 0}
RETURN 0.text:
Curated set updated (10/30): 17183[high], 25814[high], 59631[high], 15546[fair], 50858[fair], 73877[fair], 66387[low], 72434[low], 83797[low], 97801[low]
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 13 working-memory snapshot after harness update}
pool_size: 11
curated_size: 10 / 30
importance_counts: very_high=0, high=3, fair=3, low=4
curated_set:
  - 17183 [high]
  - 25814 [high]
  - 59631 [high]
  - 15546 [fair]
  - 50858 [fair]
  - 73877 [fair]
  - 66387 [low]
  - 72434 [low]
  - 83797 [low]
  - 97801 [low]
\end{trajectorylisting}

\subsubsection*{Turn 14: \CaseTool{toolVerify}{verify}}
\begin{trajectorylisting}{toolNeutral}{Turn 14 model reasoning}
We already found the exact approval letter for maribavir/Livtencity, including the Regulatory Project Manager contact line. The remaining gap is minimal: we just need the exact full name as stated in that letter. The current search angle is exhausted. Re-reading the query, the missed facet is not an entity but the exact wording format: 'full name (as mentioned in the letter) of the Regulatory Project Manager to be called in case of any questions.' We already have the letter text in 59631_3 with the line: 'If you have any questions, call Alicia Moruf, PharmD, MPH, RAC-US, Regulatory Project Manager, at 301-796-3953.' So the answer should be Alicia Moruf. No further search is needed; we should verify and then end search.
\end{trajectorylisting}

\begin{trajectorylisting}{toolVerify}{Turn 14 tool call(s)}
[
  {
    "tool": "verify",
    "params": {
      "doc_ids": [
        "59631_3"
      ],
      "claim": "Document 59631_3 contains the FDA approval letter for maribavir, and in the letter, the Regulatory Project Manager to be called for questions is Alicia Moruf, PharmD, MPH, RAC-US, Regulatory Project Manager."
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolVerify}{Turn 14 tool return 0}
RETURN 0.text:
verify: no matching docs found in memory.
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 14 working-memory snapshot after harness update}
pool_size: 11
curated_size: 10 / 30
importance_counts: very_high=0, high=3, fair=3, low=4
curated_set:
  - 17183 [high]
  - 25814 [high]
  - 59631 [high]
  - 15546 [fair]
  - 50858 [fair]
  - 73877 [fair]
  - 66387 [low]
  - 72434 [low]
  - 83797 [low]
  - 97801 [low]
\end{trajectorylisting}

\subsubsection*{Turn 15: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolNeutral}{Turn 15 model reasoning}
The last read did not generate new documents, but the system still requires a curate action after the last search/read cycle. The remaining gap is trivial: we must add/confirm any new/remaining plausibly relevant documents rather than search again because the approval letter is already identified. I am using curate to satisfy the rhythm; since the last read found no new docs, we'll curate none (no-op).
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 15 tool call(s)}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [],
      "remove_ids": [],
      "importance": {}
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 15 tool return 0}
RETURN 0.text:
Curated set updated (10/30): 17183[high], 25814[high], 59631[high], 15546[fair], 50858[fair], 73877[fair], 66387[low], 72434[low], 83797[low], 97801[low]
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 15 working-memory snapshot after harness update}
pool_size: 11
curated_size: 10 / 30
importance_counts: very_high=0, high=3, fair=3, low=4
curated_set:
  - 17183 [high]
  - 25814 [high]
  - 59631 [high]
  - 15546 [fair]
  - 50858 [fair]
  - 73877 [fair]
  - 66387 [low]
  - 72434 [low]
  - 83797 [low]
  - 97801 [low]
\end{trajectorylisting}

\subsubsection*{Turn 16: \CaseTool{toolReview}{review\_docs}}
\begin{trajectorylisting}{toolNeutral}{Turn 16 model reasoning}
We have almost the answer: the letter text shows the Regulatory Project Manager contact line. What isn't working is our last few searches-they were trying different facets but the gap is not document search but just extracting the needed name from the already-found letter. Re-reading the query, the missed facet was the Regulatory Project Manager contact itself, which we already saw in the letter. So we don't need another web search; instead, we should use review_docs/read_document to get the exact full name as it appears. We almost completed the evidence graph.
\end{trajectorylisting}

\begin{trajectorylisting}{toolReview}{Turn 16 tool call(s)}
[
  {
    "tool": "review_docs",
    "params": {
      "doc_ids": [
        "59631_3"
      ]
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolReview}{Turn 16 tool return 0}
RETURN 0.text:
# DOCUMENT ID: 59631_3
(not found in memory)
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 16 working-memory snapshot after harness update}
pool_size: 11
curated_size: 10 / 30
importance_counts: very_high=0, high=3, fair=3, low=4
curated_set:
  - 17183 [high]
  - 25814 [high]
  - 59631 [high]
  - 15546 [fair]
  - 50858 [fair]
  - 73877 [fair]
  - 66387 [low]
  - 72434 [low]
  - 83797 [low]
  - 97801 [low]
\end{trajectorylisting}

\subsubsection*{Turn 17: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolNeutral}{Turn 17 model reasoning}
I just performed a review action without curation, violating the required search->curate rhythm. The last result movement was a review, not a search. Curating is needed now, but after a review we don't add new docs; we simply follow the rhythm. The gap is minimal: we already have the exact letter in hand; we just need to wrap up and preserve evidence.
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 17 tool call(s)}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [],
      "remove_ids": [],
      "importance": {}
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 17 tool return 0}
RETURN 0.text:
Curated set updated (10/30): 17183[high], 25814[high], 59631[high], 15546[fair], 50858[fair], 73877[fair], 66387[low], 72434[low], 83797[low], 97801[low]
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 17 working-memory snapshot after harness update}
pool_size: 11
curated_size: 10 / 30
importance_counts: very_high=0, high=3, fair=3, low=4
curated_set:
  - 17183 [high]
  - 25814 [high]
  - 59631 [high]
  - 15546 [fair]
  - 50858 [fair]
  - 73877 [fair]
  - 66387 [low]
  - 72434 [low]
  - 83797 [low]
  - 97801 [low]
\end{trajectorylisting}



==> case_study_frames461_long.tex <==
\subsection{Full Trajectory B: FRAMES Query 461}
\label{app:case-frames461}

\begin{promptbox}{frames query 461}
\textbf{Query.} Which university did the actor who has appeared in the most movies in the American pie film series (including spinoffs, as of 2020) deliver a commencement address at in 2012?\\[2pt]
\textbf{Gold answer.} Dalhousie University, in Halifax, Nova Scotia\\[2pt]
\textbf{Trajectory.} 16 turns, tool diversity $6$, curated recall $1.0$, final-answer recall $1.0$.
\end{promptbox}

\paragraph{Color legend.}
\CaseTool{toolFanout}{fan\_out\_search} \CaseTool{toolSearch}{search\_corpus} \CaseTool{toolGrep}{grep\_corpus} \CaseTool{toolRead}{read\_document} \CaseTool{toolReview}{review\_docs} \CaseTool{toolCurate}{curate} \CaseTool{toolVerify}{verify} \CaseTool{toolStop}{end\_search}

\paragraph{Clipping rule.}
The transcript below preserves reasoning, tool calls, parameters, tool-return metadata, and harness state snapshots. Only individual document-text blocks longer than 2600 characters are shortened, with a marker showing the omitted length.

\begin{trajectorylisting}{toolNeutral}{System prompt used for this trajectory}
You are a retrieval subagent. Find and retrieve the most relevant documents from a corpus to help answer a question. You do NOT answer questions yourself - you only find relevant documents.

<query>
Which university did the actor who has appeared in the most movies in the American pie film series (including spinoffs, as of 2020) deliver a commencement address at in 2012?
</query>

**Available Tools:**
- **fan_out_search**(queries): Run up to 5 diverse queries in parallel.
- **search_corpus**(query): Single semantic + keyword search.
- **grep_corpus**(pattern): Exact regex pattern matching on the corpus. Use for specific names, dates, numbers, or exact phrases.
- **read_document**(doc_id): Read a document's full content. Use liberally - seeing full text reveals connections that snippets miss.
- **review_docs**(doc_ids): Re-read previously-found documents from memory (free, no corpus call).
- **curate**(add_ids, remove_ids, importance): Update your curated set (max 30 docs). These are your final output.
- **verify**(doc_ids, claim): Check if docs support a specific claim. Use before tagging as very_high.
- **end_search**(reasoning): Submit your curated set and conclude.

**Context:**
Your context has two parts:
1. **Working Memory** - curated set with snippets, document pool with snippets, and search history.
2. **Recent Turns** - full detail of your last 5 actions and results.

**Two-Tier Memory:**
- Your Working Memory shows doc IDs + brief snippets for ALL previously found docs.
- Use **review_docs** to re-read the full text of any document from memory without re-searching.
- This is useful when you want to revisit a doc you found earlier.

**Step 1 - Decompose the Query:**
Before your first search, identify the key constraints in the query (entities, dates, relationships, distinctive facts). Use the most specific/unique constraint for your first search.

**Step 2 - Core Loop (ALWAYS follow this rhythm):**
1. **Search** - use fan_out_search, search_corpus, or grep_corpus.
2. **Curate immediately** - after EVERY search, call curate to add ALL plausibly relevant docs from the results. Do NOT do two searches in a row without curating in between.
3. **Repeat** - search a different angle, then curate again.
4. **Refine** - use review_docs or read_document to revisit docs, then curate to adjust.
5. **End** - call end_search when you've thoroughly covered the query.

You have up to **35 turns**. Use them - thorough coverage matters more than speed. Don't end early if there are unexplored angles.

The search -> curate rhythm is critical. Results are freshest right after a search. If you delay curation, those results scroll out of your recent context and you lose the detail needed to decide relevance.

**Search Strategy:**
- Keep queries SHORT (5-12 words). Vary angles - don't repeat similar queries.
- **NEVER repeat queries** from your search history. Use completely different wording.
- **Decompose complex queries** into distinct searchable facets. Search each facet separately.
- **Use grep_corpus** for specific names, dates, numbers, codes, or exact phrases from the query. grep often finds what semantic search misses.
- **Use read_document liberally** - full text reveals connections that snippets hide. If a doc partially matches, read it fully. High-recall agents read more documents.

**Curation Strategy:**
- **Curate aggressively** - add ALL plausibly relevant docs. Include borderline docs. It's ALWAYS better to over-curate than under-curate. Aim for 3-8 adds per curate call.
- **Never remove** docs unless you are certain they are completely irrelevant after reading their full text.
- Keep analysis concise (2-3 paragraphs max). Focus on what to do next.

**Backtracking - Critical Reasoning Skill:**
When you notice signs of being stuck, you MUST backtrack in your reasoning:
- **Stale pool**: If your last 2-3 searches added few or no new docs, STOP. In your reasoning, explicitly state: "My current search angle is exhausted. Let me rethink." Then try a completely different query decomposition.
- **Re-reading loop**: If you find yourself reading/reviewing the same docs repeatedly, STOP. Reason about what specific information you're missing and search for it directly.
- **Wrong entity**: If results consistently don't match, question your assumptions. The query may require interpreting an entity differently (e.g., a person's maiden name, an alternate spelling, a related entity).
- **Missed facet**: Re-read the query carefully. Identify any constraint you haven't explicitly searched for yet.

Backtracking is a REASONING step: in your analysis, explain (1) what isn't working, (2) why, and (3) your new strategy. Then act on it.

**Importance Tagging (v8d):** When you call `curate`, tag each added doc with an `importance` level in {very_high, high, fair, low}. Rules:
  - very_high: you have VERIFIED the doc directly answers the query (ideally after a `verify` call).
  - high: strongly relevant, hits most query constraints.
  - fair: plausible but not confirmed (default tag if omitted).
  - low: marginal; will be evicted first when the set is full.
The curated set is capped at 30 - when full, the lowest-importance docs are evicted first to make room for higher-tagged ones.

**Auto-populate (v8d):** After your first successful search, the top-ranked 8 docs are AUTOMATICALLY added to your curated set at `fair` importance. Your job is NOT to re-add them - instead, promote the good ones to `high`/`very_high` and REMOVE the bad ones. This is subtractive curation.

**Evidence Graph (v8d):** The Working Memory shows `[Evidence Graph]` - entities (names, dates, years) and which docs they appear in. Bridge entities (in multiple docs) are high-value signals. Singleton entities (in only 1 doc) often indicate gaps - consider follow-up searches for related entities.

**Verify tool (v8d):** Use `verify(doc_ids, claim)` BEFORE tagging docs as `very_high` on multi-constraint queries. It returns yes/no for each doc, letting you confirm a doc actually satisfies ALL criteria rather than just one.

**Context budget (v8d):** Each observation ends with `[Context: X/Y]`. When X/Y is above 75%, wrap up your search within 2-3 more turns. When above 90%, call `end_search` NOW.

\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Top-level trajectory fields}
{
  "query_id": "461",
  "query_text": "Which university did the actor who has appeared in the most movies in the American pie film series (including spinoffs, as of 2020) deliver a commencement address at in 2012?",
  "dataset": "frames",
  "curated_ids": [
    "https://en.wikipedia.org/wiki/Tim_Reid",
    "https://en.wikipedia.org/wiki/Ben_Carson",
    "https://en.wikipedia.org/wiki/Steven_Curtis_Chapman",
    "https://en.wikipedia.org/wiki/Ellis_Paul",
    "https://en.wikipedia.org/wiki/Bradley_Cooper",
    "https://en.wikipedia.org/wiki/Tucker_Carlson",
    "https://en.wikipedia.org/wiki/Magic_Johnson",
    "https://en.wikipedia.org/wiki/Susan_Rice",
    "https://en.wikipedia.org/wiki/Seann_William_Scott",
    "https://en.wikipedia.org/wiki/American_Pie_(film_series)",
    "https://en.wikipedia.org/wiki/Jason_Biggs",
    "https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas",
    "https://en.wikipedia.org/wiki/Chris_Owen_(actor)",
    "https://en.wikipedia.org/wiki/List_of_American_Pie_characters",
    "https://en.wikipedia.org/wiki/Eugene_Levy",
    "https://en.wikipedia.org/wiki/American_Pie_(film)",
    "https://en.wikipedia.org/wiki/Shannon_Elizabeth",
    "https://en.wikipedia.org/wiki/John_Cho",
    "https://en.wikipedia.org/wiki/Dan_Petronijevic",
    "https://en.wikipedia.org/wiki/Heath_Ledger",
    "https://en.wikipedia.org/wiki/Jonathan_Franzen",
    "https://en.wikipedia.org/wiki/Joss_Whedon",
    "https://en.wikipedia.org/wiki/Wes_Craven",
    "https://en.wikipedia.org/wiki/List_of_NYU_Tisch_School_of_the_Arts_people",
    "https://en.wikipedia.org/wiki/David_Sutherland",
    "https://en.wikipedia.org/wiki/Donald_Sutherland",
    "https://en.wikipedia.org/wiki/John_Lithgow",
    "https://en.wikipedia.org/wiki/Bradley_Whitford",
    "https://en.wikipedia.org/wiki/Princeton_University",
    "https://en.wikipedia.org/wiki/Dalhousie_University"
  ],
  "curated_importance": {
    "https://en.wikipedia.org/wiki/Tim_Reid": "fair",
    "https://en.wikipedia.org/wiki/Ben_Carson": "fair",
    "https://en.wikipedia.org/wiki/Steven_Curtis_Chapman": "fair",
    "https://en.wikipedia.org/wiki/Ellis_Paul": "fair",
    "https://en.wikipedia.org/wiki/Bradley_Cooper": "fair",
    "https://en.wikipedia.org/wiki/Tucker_Carlson": "fair",
    "https://en.wikipedia.org/wiki/Magic_Johnson": "fair",
    "https://en.wikipedia.org/wiki/Susan_Rice": "fair",
    "https://en.wikipedia.org/wiki/Seann_William_Scott": "high",
    "https://en.wikipedia.org/wiki/American_Pie_(film_series)": "high",
    "https://en.wikipedia.org/wiki/Jason_Biggs": "fair",
    "https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas": "fair",
    "https://en.wikipedia.org/wiki/Chris_Owen_(actor)": "fair",
    "https://en.wikipedia.org/wiki/List_of_American_Pie_characters": "high",
    "https://en.wikipedia.org/wiki/Eugene_Levy": "very_high",
    "https://en.wikipedia.org/wiki/American_Pie_(film)": "high",
    "https://en.wikipedia.org/wiki/Shannon_Elizabeth": "fair",
    "https://en.wikipedia.org/wiki/John_Cho": "fair",
    "https://en.wikipedia.org/wiki/Dan_Petronijevic": "low",
    "https://en.wikipedia.org/wiki/Heath_Ledger": "low",
    "https://en.wikipedia.org/wiki/Jonathan_Franzen": "low",
    "https://en.wikipedia.org/wiki/Joss_Whedon": "low",
    "https://en.wikipedia.org/wiki/Wes_Craven": "low",
    "https://en.wikipedia.org/wiki/List_of_NYU_Tisch_School_of_the_Arts_people": "low",
    "https://en.wikipedia.org/wiki/David_Sutherland": "low",
    "https://en.wikipedia.org/wiki/Donald_Sutherland": "low",
    "https://en.wikipedia.org/wiki/John_Lithgow": "low",
    "https://en.wikipedia.org/wiki/Bradley_Whitford": "low",
    "https://en.wikipedia.org/wiki/Princeton_University": "fair",
    "https://en.wikipedia.org/wiki/Dalhousie_University": "high"
  },
  "evidence_graph": {
    "entity_to_docs": {},
    "doc_to_entities": {}
  },
  "reward": 2.6842105263157894,
  "metrics": {
    "recall": 1.0,
    "precision": 0.06666666666666667,
    "f_beta": 0.2631578947368421,
    "final_answer_recall": 1.0,
    "final_answer_found": 1.0,
    "trajectory_recall": 1.0,
    "trajectory_fa_recall": 1.0,
    "final_answer_bonus": 1.0,
    "fa_dense_reward": 1.2000000000000002,
    "fa_miss_gap": 0.0,
    "fa_miss_penalty": 0.0,
    "pool_curated_gap": 0.0,
    "gap_penalty": 0.0,
    "turn_penalty": 0.0,
    "pre_penalty_reward": 2.6842105263157894,
    "num_curated_docs": 30.0,
    "used_curate": 1.0,
    "total_curate_calls": 8.0,
    "curate_rate": 0.5,
    "curate_rate_bonus": 0.0,
    "tool_diversity": 6.0,
    "tool_diversity_bonus": 0.0,
    "num_turns": 16,
    "final_reward": 2.6842105263157894,
    "no_error": 1.0,
    "max_turns_reached": 0.0
  }
}
\end{trajectorylisting}

\subsubsection*{Turn 0: \CaseTool{toolFanout}{fan\_out\_search}}
\begin{trajectorylisting}{toolNeutral}{Turn 0 model reasoning}
We need: Which university did the actor who has appeared in the most movies in the American Pie film series (including spinoffs, as of 2020) deliver a commencement address at in 2012.

We can break it down.

Candidates: Need actor with most appearances in American Pie series.

List of movies: American Pie (1999), American Pie 2 (2001), American Pie 3 (2003), American Pie 4 (2008), American Wedding (2003?), Wait 2003? Actually American Wedding (2003) is the third? Let's check full series: American Pie (1999); American Pie 2 (2001); American Wedding (2003); American Reunion (2012); American Pie Presents: Band Party (2007); American Pie Presents: The Wedding (2009); American Pie Presents: The Book of Love (2010); American Pie Presents: The Naked Mile (2006); American Pie Presents: The First Kiss (2009). Also spinoffs: American Wedding (2003), American Reunion 2012. The actor who appears in the most movies: I recall Skyler or others? Let's recall main casts: Jason Biggs (Jim), Alyson Hannigan (Michelle), Natasha Lyonne (Stifler?), actually Stifler is Seann William Scott. He appears in many? Let's count: Stifler from first through fourth, plus spinoffs? Seann William Scott appears in 1) American Pie 2? Wait Stifler is in first: yes first. In American Pie 2? yes Stifler. In American Wedding? maybe he appears as Stifler. In American Pie Presents: The Book of Love? Not sure. Also spinoffs: He appears in American Pie Presents: The Book of Love? Let's recall: Seann William Scott as Stifler appears in original series plus the spin-offs? There's also his film within the series. Let's search.

So likely the actor is Seann William Scott, or maybe the actor is Tom Gills? No. The actor with most appearances likely is Seann William Scott or Jason Biggs? Jason Biggs appears first through first three? He appears also in reunion and maybe New movies. Let's verify counts.

We need actor with most appearances among all US movies up to 2020. Let's search for 'Seann William Scott American Pie appearances' or 'American Pie actor with most appearances'.

We also need commencement address in 2012 at a university. Which university? So Seann William Scott delivered commencement address in 2012 at some university. Need to find that.

So we need to find doc about Seann William Scott commencement address 2012. Alternatively, if actor is Jason Biggs, find if he delivered commencement address 2012. But Jason Biggs may have spoken at University of Notre Dame? Let's think: Jason Biggs Speech 2013? Wait.

Let's recall: Seann William Scott on his biography: He gave a commencement address at University of Kansas? Let's quickly search.

Given time, best to do fan_out_search queries.

First query: "Seann William Scott commencement address 2012 university".

Second query: "American Pie series actor most appearances".

Third: "American Pie spinoffs actor who appears in most films".

Fourth: "Jason Biggs commencement address 2012".

Fifth: "American Pie actor commencement 2012".

But my first size: "Seann William Scott commencement address 2012 university" should find doc. Let's do that.
\end{trajectorylisting}

\begin{trajectorylisting}{toolFanout}{Turn 0 tool call(s)}
[
  {
    "tool": "fan_out_search",
    "params": {
      "queries": [
        "Seann William Scott commencement address 2012 university",
        "most American Pie films actor",
        "American Pie actor who appeared most movies",
        "Seann William Scott 2012 commencement",
        "Jason Biggs commencement 2012"
      ]
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolFanout}{Turn 0 tool return 0}
RETURN 0.text:

# DOCUMENT ID: https://en.wikipedia.org/wiki/Tim_Reid (41 tokens)
Tim Reid - Wikipedia
Timothy Lee Reid Sr. (born December 19, 1944) is an American actor, comedian and film director best known for his roles in prime time American television ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Ben_Carson (43 tokens)
Ben Carson - Wikipedia
Benjamin Solomon Carson Sr. (born September 18, 1951) is an American retired neurosurgeon, academic, author, and government official who served as the 17th ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Steven_Curtis_Chapman (39 tokens)
Steven Curtis Chapman - Wikipedia
Steven Curtis Chapman (born November 21, 1962) is an American contemporary Christian music singer, songwriter, record producer, actor, author, and social ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Ellis_Paul (48 tokens)
Ellis Paul - Wikipedia
Ellis Paul (born Paul Plissey; January 14, 1965) is an American singer-songwriter and folk musician. Born in Presque Isle, Aroostook County, Maine, ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Bradley_Cooper (41 tokens)
Bradley Cooper - Wikipedia
Bradley Charles Cooper (born January 5, 1975) is an American actor and filmmaker. He is the recipient of various accolades, including a British Academy Film ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Tucker_Carlson (41 tokens)
Tucker Carlson - Wikipedia
Tucker Swanson McNear Carlson (born May 16, 1969) is an American conservative political commentator who hosts Tucker on X and The Tucker Carlson Show since ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Magic_Johnson (40 tokens)
Magic Johnson - Wikipedia
Earvin "Magic" Johnson Jr. (born August 14, 1959) is an American businessman and former professional basketball player. Often regarded as the greatest point ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Susan_Rice (40 tokens)
Susan Rice - Wikipedia
Susan Elizabeth Rice (born November 17, 1964) is an American former diplomat, policy advisor, and public official. As a member of the Democratic Party, ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Dick_Cheney (42 tokens)
Dick Cheney - Wikipedia
Richard Bruce Cheney (January 30, 1941 - November 3, 2025) was an American politician and businessman who was the vice president of the United States under ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/William_Gibson (38 tokens)
William Gibson - Wikipedia
William Ford Gibson (born March 17, 1948) is a speculative fiction writer and essayist widely credited with pioneering the science fiction subgenre known as ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Jason_Biggs (51 tokens)
Jason Biggs - Wikipedia
Jason Matthew Biggs (born May 12, 1978) is an American actor. He is best known for his lead role as Jim Levenstein in the American Pie film series (1999-2012).

# DOCUMENT ID: https://en.wikipedia.org/wiki/American_Pie_(film_series) (30 tokens)
American Pie (film series) - Wikipedia
Principal cast ; Seann William Scott * Thomas Ian Nicholas ; Seann William Scott * Thomas Ian Nicholas.

# DOCUMENT ID: https://en.wikipedia.org/wiki/Seann_William_Scott (49 tokens)
Seann William Scott - Wikipedia
Scott is best known for his breakout role as Steve Stifler in the American Pie film series (1999-2012). He also starred in a lead role as Doug Glatt in Goon ( ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas (44 tokens)
Thomas Ian Nicholas - Wikipedia
In film, Nicholas is best known for his lead roles as Kevin Meyers in the American Pie theatrical film series (1999-2012) and Henry Rowengartner in the sports ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Chris_Owen_(actor) (46 tokens)
Chris Owen (actor) - Wikipedia
Chris Owen (born September 25, 1980) is an American actor. He is best known for his supporting role as Chuck "Sherminator" Sherman in the American Pie ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/List_of_American_Pie_characters (50 tokens)
List of American Pie characters - Wikipedia
Noah Levenstein, played by Eugene Levy, has appeared in eight of the nine released films. Biggs, Hannigan, Scott, Nicholas, Thomas, Coolidge, Cho, Isfield, ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Tad_Hilgenbrink (52 tokens)
Tad Hilgenbrink - Wikipedia
Tad Hilgenbrink (born October 9, 1981) is an American actor, known for his role as Matt Stifler in American Pie Presents: Band Camp, Chance Marquis in The ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Chris_Klein_(actor) (49 tokens)
Chris Klein (actor) - Wikipedia
He reprised his role in two sequels: American Pie 2 (2001) and American Reunion (2012). Chris Klein. Klein in March 2012. Born. Frederick Christopher Klein.

# DOCUMENT ID: https://en.wikipedia.org/wiki/Eddie_Kaye_Thomas (41 tokens)
Eddie Kaye Thomas - Wikipedia
Thomas rose to prominence for his supporting role as Paul Finch in the teen sex comedy film American Pie (1999), which he reprised in a starring capacity in ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/John_White_(actor) (50 tokens)
John White (actor) - Wikipedia
John Michael White (born June 10, 1981) is a Canadian actor. He is best known for his role as Erik Stifler in American Pie Presents: The Naked Mile (2006)

# DOCUMENT ID: https://en.wikipedia.org/wiki/Eugene_Levy (47 tokens)
Eugene Levy - Wikipedia
He is best known for appearing in the sketch comedy series SCTV, which aired from 1976 until 1984, and the American Pie series of films. ... He was a close friend ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/List_of_Ithaca_College_alumni (35 tokens)
List of Ithaca College alumni - Wikipedia
Ithacans are persons affiliated with Ithaca College, especially alumni. The following is a list of notable Ithacans.

# DOCUMENT ID: https://en.wikipedia.org/wiki/List_of_Arizona_State_University_alumni_in_government_and_politics (40 tokens)
List of Arizona State University alumni in government and politics
Arizona State University (ASU) has graduated a number of notable people in government and politics. This includes graduates and non-graduate former students.

# DOCUMENT ID: https://en.wikipedia.org/wiki/University_of_Central_Florida (38 tokens)
University of Central Florida - Wikipedia
The University of Central Florida (UCF) is a public research university with its main campus in unincorporated Orange County, Florida, United States.

# DOCUMENT ID: https://en.wikipedia.org/wiki/St._Andrew%27s_School_(Delaware) (51 tokens)
St. Andrew's School (Delaware) - Wikipedia
St. Andrew's is a private, Episcopal, co-educational 100% boarding school near Middletown, Delaware. It is one of only three co-ed college preparatory schools ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Higher_education_in_the_United_States (36 tokens)
Higher education in the United States - Wikipedia
In the United States, higher education is an optional stage of formal learning following secondary education. It is also referred to as post-secondary ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Matt_Nagy (32 tokens)
Matt Nagy - Wikipedia
Matthew Nagy is an American professional football coach and former quarterback who is currently the offensive coordinator of the New York Giants of the ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Shakira (38 tokens)
Shakira - Wikipedia
Shakira Isabel Mebarak Ripoll is a Colombian singer, songwriter, dancer, and record producer. Referred to as the "Queen of Latin Music", ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Gavin_Newsom (42 tokens)
Gavin Newsom - Wikipedia
Gavin Christopher Newsom (born October 10, 1967) is an American politician and businessman serving as the 40th governor of California since 2019.

# DOCUMENT ID: https://en.wikipedia.org/wiki/Jim_Nantz (45 tokens)
Jim Nantz - Wikipedia
James William Nantz III (born May 17, 1959) is an American sportscaster who has worked on telecasts of the National Football League (NFL), NCAA Division I ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/John_Roberts (45 tokens)
John Roberts - Wikipedia
John Glover Roberts Jr. (born January 27, 1955) is an American jurist who has served since 2005 as the 17th chief justice of the United States.

# DOCUMENT ID: https://en.wikipedia.org/wiki/List_of_The_Tonight_Show_with_Jay_Leno_episodes_(2012) (66 tokens)
List of The Tonight Show with Jay Leno episodes (2012) - Wikipedia
Maya Rudolph, Jason Biggs * Gym Class Heroes featuring Ryan Tedder. Meal Or No ... Jay Gives A Commencement Address. 4,260, May 24, 2012 (2012-05-24), Glenn ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/James_Van_Der_Beek (54 tokens)
James Van Der Beek - Wikipedia
... (2012-2013), starred as FBI agent Elijah Mundo on CSI: Cyber (2015-2016) ... Jason Biggs as Silent Bob. In 2002, he portrayed Sean Bateman, younger ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/List_of_Brigham_Young_University_alumni (43 tokens)
List of Brigham Young University alumni - Wikipedia
This list of Brigham Young University alumni includes notable graduates, non-graduate former students, and current students of Brigham Young University (BYU)

# DOCUMENT ID: https://en.wikipedia.org/wiki/List_of_University_of_California,_Davis_alumni (38 tokens)
List of University of California, Davis alumni - Wikipedia
This page lists notable alumni of the University of California, Davis. Wikimedia Commons logo. Wikimedia Commons has media related to Alumni of the ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Wayne_Chang (45 tokens)
Wayne Chang - Wikipedia
Wayne Chang (born August 3, 1983) is an American entrepreneur, angel investor, film producer, and philanthropist. He is best known for founding Crashlytics, ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/115th_United_States_Congress (38 tokens)
115th United States Congress - Wikipedia
The 115th United States Congress was a meeting of the legislative branch of the United States of America federal government, composed of the Senate and the ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/State_of_emergency (32 tokens)
State of emergency - Wikipedia
A state of emergency is a situation in which a government is empowered to put through policies that it would normally not be permitted to do

# DOCUMENT ID: https://en.wikipedia.org/wiki/List_of_African_American_jurists (34 tokens)
List of African American jurists - Wikipedia
This list includes individuals self-identified as African Americans who have made prominent contributions to the field of law in the United States.

# DOCUMENT ID: https://en.wikipedia.org/wiki/List_of_television_performers_who_died_during_production (30 tokens)
List of television performers who died during production - Wikipedia
The following lists television performers who died during production of the television show in which they were appearing.

[AUTO-POPULATED] Top 8 docs from this search have been added to your curated set at 'fair' importance. Use `curate` with `importance` to promote/demote and `remove_ids` to drop irrelevant ones.
[Context: 2618/30720]

RETURN 0.metadata:
{
  "metadata": {
    "returned_chunk_ids": [
      "https://en.wikipedia.org/wiki/Tim_Reid",
      "https://en.wikipedia.org/wiki/Ben_Carson",
      "https://en.wikipedia.org/wiki/Steven_Curtis_Chapman",
      "https://en.wikipedia.org/wiki/Ellis_Paul",
      "https://en.wikipedia.org/wiki/Bradley_Cooper",
      "https://en.wikipedia.org/wiki/Tucker_Carlson",
      "https://en.wikipedia.org/wiki/Magic_Johnson",
      "https://en.wikipedia.org/wiki/Susan_Rice",
      "https://en.wikipedia.org/wiki/Dick_Cheney",
      "https://en.wikipedia.org/wiki/William_Gibson",
      "https://en.wikipedia.org/wiki/Jason_Biggs",
      "https://en.wikipedia.org/wiki/American_Pie_(film_series)",
      "https://en.wikipedia.org/wiki/Seann_William_Scott",
      "https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas",
      "https://en.wikipedia.org/wiki/Chris_Owen_(actor)",
      "https://en.wikipedia.org/wiki/List_of_American_Pie_characters",
      "https://en.wikipedia.org/wiki/Tad_Hilgenbrink",
      "https://en.wikipedia.org/wiki/Chris_Klein_(actor)",
      "https://en.wikipedia.org/wiki/Eddie_Kaye_Thomas",
      "https://en.wikipedia.org/wiki/John_White_(actor)",
      "https://en.wikipedia.org/wiki/Eugene_Levy",
      "https://en.wikipedia.org/wiki/List_of_Ithaca_College_alumni",
      "https://en.wikipedia.org/wiki/List_of_Arizona_State_University_alumni_in_government_and_politics",
      "https://en.wikipedia.org/wiki/University_of_Central_Florida",
      "https://en.wikipedia.org/wiki/St._Andrew%27s_School_(Delaware)",
      "https://en.wikipedia.org/wiki/Higher_education_in_the_United_States",
      "https://en.wikipedia.org/wiki/Matt_Nagy",
      "https://en.wikipedia.org/wiki/Shakira",
      "https://en.wikipedia.org/wiki/Gavin_Newsom",
      "https://en.wikipedia.org/wiki/Jim_Nantz",
      "https://en.wikipedia.org/wiki/John_Roberts",
      "https://en.wikipedia.org/wiki/List_of_The_Tonight_Show_with_Jay_Leno_episodes_(2012)",
      "https://en.wikipedia.org/wiki/James_Van_Der_Beek",
      "https://en.wikipedia.org/wiki/List_of_Brigham_Young_University_alumni",
      "https://en.wikipedia.org/wiki/List_of_University_of_California,_Davis_alumni",
      "https://en.wikipedia.org/wiki/Wayne_Chang",
      "https://en.wikipedia.org/wiki/115th_United_States_Congress",
      "https://en.wikipedia.org/wiki/State_of_emergency",
      "https://en.wikipedia.org/wiki/List_of_African_American_jurists",
      "https://en.wikipedia.org/wiki/List_of_television_performers_who_died_during_production"
    ],
    "queries_executed": 5
  }
}
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 0 working-memory snapshot after harness update}
pool_size: 40
curated_size: 8 / 30
importance_counts: very_high=0, high=0, fair=8, low=0
curated_set:
  - https://en.wikipedia.org/wiki/Ben_Carson [fair]
  - https://en.wikipedia.org/wiki/Bradley_Cooper [fair]
  - https://en.wikipedia.org/wiki/Ellis_Paul [fair]
  - https://en.wikipedia.org/wiki/Magic_Johnson [fair]
  - https://en.wikipedia.org/wiki/Steven_Curtis_Chapman [fair]
  - https://en.wikipedia.org/wiki/Susan_Rice [fair]
  - https://en.wikipedia.org/wiki/Tim_Reid [fair]
  - https://en.wikipedia.org/wiki/Tucker_Carlson [fair]
\end{trajectorylisting}

\subsubsection*{Turn 1: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolCurate}{Turn 1 tool call(s)}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [
        "https://en.wikipedia.org/wiki/Seann_William_Scott",
        "https://en.wikipedia.org/wiki/American_Pie_(film_series)",
        "https://en.wikipedia.org/wiki/Jason_Biggs",
        "https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas",
        "https://en.wikipedia.org/wiki/Chris_Owen_(actor)",
        "https://en.wikipedia.org/wiki/List_of_American_Pie_characters",
        "https://en.wikipedia.org/wiki/Chris_Klein_(actor)"
      ],
      "importance": {
        "https://en.wikipedia.org/wiki/Seann_William_Scott": "high",
        "https://en.wikipedia.org/wiki/American_Pie_(film_series)": "high",
        "https://en.wikipedia.org/wiki/Jason_Biggs": "fair",
        "https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas": "fair",
        "https://en.wikipedia.org/wiki/Chris_Owen_(actor)": "fair",
        "https://en.wikipedia.org/wiki/List_of_American_Pie_characters": "high",
        "https://en.wikipedia.org/wiki/Chris_Klein_(actor)": "low"
      }
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 1 tool return 0}
RETURN 0.text:
Curated set updated (15/30): https://en.wikipedia.org/wiki/American_Pie_(film_series)[high], https://en.wikipedia.org/wiki/List_of_American_Pie_characters[high], https://en.wikipedia.org/wiki/Seann_William_Scott[high], https://en.wikipedia.org/wiki/Ben_Carson[fair], https://en.wikipedia.org/wiki/Bradley_Cooper[fair], https://en.wikipedia.org/wiki/Chris_Owen_(actor)[fair], https://en.wikipedia.org/wiki/Ellis_Paul[fair], https://en.wikipedia.org/wiki/Jason_Biggs[fair], https://en.wikipedia.org/wiki/Magic_Johnson[fair], https://en.wikipedia.org/wiki/Steven_Curtis_Chapman[fair], https://en.wikipedia.org/wiki/Susan_Rice[fair], https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas[fair], https://en.wikipedia.org/wiki/Tim_Reid[fair], https://en.wikipedia.org/wiki/Tucker_Carlson[fair], https://en.wikipedia.org/wiki/Chris_Klein_(actor)[low]
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 1 working-memory snapshot after harness update}
pool_size: 40
curated_size: 15 / 30
importance_counts: very_high=0, high=3, fair=11, low=1
curated_set:
  - https://en.wikipedia.org/wiki/American_Pie_(film_series) [high]
  - https://en.wikipedia.org/wiki/List_of_American_Pie_characters [high]
  - https://en.wikipedia.org/wiki/Seann_William_Scott [high]
  - https://en.wikipedia.org/wiki/Ben_Carson [fair]
  - https://en.wikipedia.org/wiki/Bradley_Cooper [fair]
  - https://en.wikipedia.org/wiki/Chris_Owen_(actor) [fair]
  - https://en.wikipedia.org/wiki/Ellis_Paul [fair]
  - https://en.wikipedia.org/wiki/Jason_Biggs [fair]
  - https://en.wikipedia.org/wiki/Magic_Johnson [fair]
  - https://en.wikipedia.org/wiki/Steven_Curtis_Chapman [fair]
  - https://en.wikipedia.org/wiki/Susan_Rice [fair]
  - https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas [fair]
  - https://en.wikipedia.org/wiki/Tim_Reid [fair]
  - https://en.wikipedia.org/wiki/Tucker_Carlson [fair]
  - https://en.wikipedia.org/wiki/Chris_Klein_(actor) [low]
\end{trajectorylisting}

\subsubsection*{Turn 2: \CaseTool{toolSearch}{search\_corpus}}
\begin{trajectorylisting}{toolNeutral}{Turn 2 model reasoning}
We've learned the actor with most appearances in American Pie film series is likely Seann William Scott (Steve Stifler) or Eugene Levy (appearance in many). Need commencement address in 2012 at a university. Fowler loop indicates current angle: actor with most appearances + commencement address 2012. That result surfaced none from kickoff queries exactly showing commencement address. Most current search angle results include actor biographies but the 2012 commencement detail is separate. My current search angle is partially working: the actor identification is fine, but the commencement/pre-2012 angle is stale. Let me rethink. Re-read query: Which university did the actor deliver a commencement address at in 2012? So we need actor -> commencement address -> university. Might be Eugene Levy instead if he has more appearances than Seann Scott. First verify the most-appearances fact: which actor appears most? Use List_of_American_Pie_characters page likely enumerates appearances. Also maybe separate query for Eugene Levy commencement address. New search angle: actor in American Pie inclusive of spin-offs with most movies, check commencement 2012 universities for that actor.
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 2 tool call(s)}
[
  {
    "tool": "search_corpus",
    "params": {
      "query": "Eugene Levy 2012 commencement address university"
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 2 tool return 0}
RETURN 0.text:

# DOCUMENT ID: https://en.wikipedia.org/wiki/Eugene_Levy_(politician) (57 tokens)
Eugene Levy (politician) - Wikipedia
Eugene Levy (December 1, 1926 - July 12, 1990) was a member of the New York State Senate for the 38th District covering all of Rockland County and parts of ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Harlan_Ellison (48 tokens)
Harlan Ellison - Wikipedia
Harlan Jay Ellison (May 27, 1934 - June 28, 2018) was an American writer, known for his prolific and influential work in New Wave speculative fiction and ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Edith_Windsor (46 tokens)
Edith Windsor - Wikipedia
Edith Windsor [1] (nee Schlain; June 20, 1929 - September 12, 2017) was an American LGBT rights activist and a technology manager at IBM.

# DOCUMENT ID: https://en.wikipedia.org/wiki/Sonny_Rollins (45 tokens)
Sonny Rollins - Wikipedia
Walter Theodore "Sonny" Rollins (born September 7, 1930) is a retired American jazz tenor saxophonist who is widely recognized as one of the most important ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Second_Amendment_to_the_United_States_Constitution (46 tokens)
Second Amendment to the United States Constitution - Wikipedia
The Second Amendment (Amendment II) to the United States Constitution protects the right to keep and bear arms. It was ratified on December 15, 1791.

# DOCUMENT ID: https://en.wikipedia.org/wiki/Kenneth_Kiesler (36 tokens)
Kenneth Kiesler - Wikipedia
Kenneth Kiesler (born August 18, 1953) is an American symphony orchestra and opera conductor and mentor to conductors.

# DOCUMENT ID: https://en.wikipedia.org/wiki/History_of_Atlanta (41 tokens)
History of Atlanta - Wikipedia
The history of Atlanta dates back to 1836, when Georgia decided to build a railroad to the US Midwest and a location was chosen to be the line's terminus.

# DOCUMENT ID: https://en.wikipedia.org/wiki/Azores (38 tokens)
Azores - Wikipedia
The Azores is an archipelago composed of nine volcanic islands in the Macaronesia region of the North Atlantic Ocean. There are nine major Azorean islands and ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/History_of_the_United_States (32 tokens)
History of the United States - Wikipedia
The history of the present-day United States began in 1607 with the establishment of Jamestown in modern day Virginia.
[Context: 6271/30720]

RETURN 0.metadata:
{
  "metadata": {
    "returned_chunk_ids": [
      "https://en.wikipedia.org/wiki/Eugene_Levy_(politician)",
      "https://en.wikipedia.org/wiki/Harlan_Ellison",
      "https://en.wikipedia.org/wiki/Edith_Windsor",
      "https://en.wikipedia.org/wiki/Sonny_Rollins",
      "https://en.wikipedia.org/wiki/Second_Amendment_to_the_United_States_Constitution",
      "https://en.wikipedia.org/wiki/Kenneth_Kiesler",
      "https://en.wikipedia.org/wiki/History_of_Atlanta",
      "https://en.wikipedia.org/wiki/Azores",
      "https://en.wikipedia.org/wiki/History_of_the_United_States"
    ],
    "pre_rerank_chunk_ids": null
  }
}
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 2 working-memory snapshot after harness update}
pool_size: 49
curated_size: 15 / 30
importance_counts: very_high=0, high=3, fair=11, low=1
curated_set:
  - https://en.wikipedia.org/wiki/American_Pie_(film_series) [high]
  - https://en.wikipedia.org/wiki/List_of_American_Pie_characters [high]
  - https://en.wikipedia.org/wiki/Seann_William_Scott [high]
  - https://en.wikipedia.org/wiki/Ben_Carson [fair]
  - https://en.wikipedia.org/wiki/Bradley_Cooper [fair]
  - https://en.wikipedia.org/wiki/Chris_Owen_(actor) [fair]
  - https://en.wikipedia.org/wiki/Ellis_Paul [fair]
  - https://en.wikipedia.org/wiki/Jason_Biggs [fair]
  - https://en.wikipedia.org/wiki/Magic_Johnson [fair]
  - https://en.wikipedia.org/wiki/Steven_Curtis_Chapman [fair]
  - https://en.wikipedia.org/wiki/Susan_Rice [fair]
  - https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas [fair]
  - https://en.wikipedia.org/wiki/Tim_Reid [fair]
  - https://en.wikipedia.org/wiki/Tucker_Carlson [fair]
  - https://en.wikipedia.org/wiki/Chris_Klein_(actor) [low]
\end{trajectorylisting}

\subsubsection*{Turn 3: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolNeutral}{Turn 3 model reasoning}
Eugene Levy 2012 commencement address likely not surfaced, but we should curate whatever surfaced before next search. It surfaced mostly adverse noise and a politician page; only Eugene Levy is directly relevant. I'm curating it because last search was Eugene Levy + commencement address angle; according to rhythm we must curate before searching further.
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 3 tool call(s)}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [
        "https://en.wikipedia.org/wiki/Eugene_Levy_(politician)",
        "https://en.wikipedia.org/wiki/Eugene_Levy"
      ],
      "remove_ids": [],
      "importance": {
        "https://en.wikipedia.org/wiki/Eugene_Levy_(politician)": "low",
        "https://en.wikipedia.org/wiki/Eugene_Levy": "high"
      }
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 3 tool return 0}
RETURN 0.text:
Curated set updated (17/30): https://en.wikipedia.org/wiki/American_Pie_(film_series)[high], https://en.wikipedia.org/wiki/Eugene_Levy[high], https://en.wikipedia.org/wiki/List_of_American_Pie_characters[high], https://en.wikipedia.org/wiki/Seann_William_Scott[high], https://en.wikipedia.org/wiki/Ben_Carson[fair], https://en.wikipedia.org/wiki/Bradley_Cooper[fair], https://en.wikipedia.org/wiki/Chris_Owen_(actor)[fair], https://en.wikipedia.org/wiki/Ellis_Paul[fair], https://en.wikipedia.org/wiki/Jason_Biggs[fair], https://en.wikipedia.org/wiki/Magic_Johnson[fair], https://en.wikipedia.org/wiki/Steven_Curtis_Chapman[fair], https://en.wikipedia.org/wiki/Susan_Rice[fair], https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas[fair], https://en.wikipedia.org/wiki/Tim_Reid[fair], https://en.wikipedia.org/wiki/Tucker_Carlson[fair], https://en.wikipedia.org/wiki/Chris_Klein_(actor)[low], https://en.wikipedia.org/wiki/Eugene_Levy_(politician)[low]
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 3 working-memory snapshot after harness update}
pool_size: 49
curated_size: 17 / 30
importance_counts: very_high=0, high=4, fair=11, low=2
curated_set:
  - https://en.wikipedia.org/wiki/American_Pie_(film_series) [high]
  - https://en.wikipedia.org/wiki/Eugene_Levy [high]
  - https://en.wikipedia.org/wiki/List_of_American_Pie_characters [high]
  - https://en.wikipedia.org/wiki/Seann_William_Scott [high]
  - https://en.wikipedia.org/wiki/Ben_Carson [fair]
  - https://en.wikipedia.org/wiki/Bradley_Cooper [fair]
  - https://en.wikipedia.org/wiki/Chris_Owen_(actor) [fair]
  - https://en.wikipedia.org/wiki/Ellis_Paul [fair]
  - https://en.wikipedia.org/wiki/Jason_Biggs [fair]
  - https://en.wikipedia.org/wiki/Magic_Johnson [fair]
  - https://en.wikipedia.org/wiki/Steven_Curtis_Chapman [fair]
  - https://en.wikipedia.org/wiki/Susan_Rice [fair]
  - https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas [fair]
  - https://en.wikipedia.org/wiki/Tim_Reid [fair]
  - https://en.wikipedia.org/wiki/Tucker_Carlson [fair]
  - https://en.wikipedia.org/wiki/Chris_Klein_(actor) [low]
  - https://en.wikipedia.org/wiki/Eugene_Levy_(politician) [low]
\end{trajectorylisting}

\subsubsection*{Turn 4: \CaseTool{toolSearch}{search\_corpus}}
\begin{trajectorylisting}{toolNeutral}{Turn 4 model reasoning}
Current search angle is getting weak: Eugene Levy + commencement address angle hasn't surfaced. Gap: I haven't confirmed the actor with most appearances in the American Pie series precisely, nor identified commencement address docs. Missed facet: the actor could be Eugene Levy, not just Seann William Scott; need to search that name + commencement address. Also, maybe it's a commencement address by Gene Levy (not Eugene), or by another actor listed as most appearances. Let's try a completely different facet: identify most-appearances actor and then separate search for that actor's commencement address.
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 4 tool call(s)}
[
  {
    "tool": "search_corpus",
    "params": {
      "query": "most American Pie films actor appeared in most movies american pie series"
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 4 tool return 0}
RETURN 0.text:

# DOCUMENT ID: https://en.wikipedia.org/wiki/American_Pie_(film) (48 tokens)
American Pie (film) - Wikipedia
The film's main ensemble cast includes Jason Biggs, Chris Klein, Alyson Hannigan, Natasha Lyonne, Thomas Ian Nicholas, Tara Reid, Mena Suvari, Eddie Kaye Thomas ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Dan_Petronijevic (46 tokens)
Dan Petronijevic - Wikipedia
Dan Petronijevic is a Canadian actor who has appeared in various feature films, including the American Pie franchise, and in TV shows such as 19-2, Playmakers, ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/John_Cho (52 tokens)
John Cho - Wikipedia
He is known for his roles as John/MILF guy #2 in the American Pie film series (1999-2012), Harold Lee in the Harold & Kumar film series (2004-2011), and Hikaru ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Shannon_Elizabeth (49 tokens)
Shannon Elizabeth - Wikipedia
... American actress, activist, and poker player. Her roles in the Scary Movie (2000) and the American Pie film series (1999-2001; 2012) solidified her status ...
[Context: 7340/30720]

RETURN 0.metadata:
{
  "metadata": {
    "returned_chunk_ids": [
      "https://en.wikipedia.org/wiki/American_Pie_(film)",
      "https://en.wikipedia.org/wiki/Dan_Petronijevic",
      "https://en.wikipedia.org/wiki/John_Cho",
      "https://en.wikipedia.org/wiki/Shannon_Elizabeth"
    ],
    "pre_rerank_chunk_ids": null
  }
}
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 4 working-memory snapshot after harness update}
pool_size: 53
curated_size: 17 / 30
importance_counts: very_high=0, high=4, fair=11, low=2
curated_set:
  - https://en.wikipedia.org/wiki/American_Pie_(film_series) [high]
  - https://en.wikipedia.org/wiki/Eugene_Levy [high]
  - https://en.wikipedia.org/wiki/List_of_American_Pie_characters [high]
  - https://en.wikipedia.org/wiki/Seann_William_Scott [high]
  - https://en.wikipedia.org/wiki/Ben_Carson [fair]
  - https://en.wikipedia.org/wiki/Bradley_Cooper [fair]
  - https://en.wikipedia.org/wiki/Chris_Owen_(actor) [fair]
  - https://en.wikipedia.org/wiki/Ellis_Paul [fair]
  - https://en.wikipedia.org/wiki/Jason_Biggs [fair]
  - https://en.wikipedia.org/wiki/Magic_Johnson [fair]
  - https://en.wikipedia.org/wiki/Steven_Curtis_Chapman [fair]
  - https://en.wikipedia.org/wiki/Susan_Rice [fair]
  - https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas [fair]
  - https://en.wikipedia.org/wiki/Tim_Reid [fair]
  - https://en.wikipedia.org/wiki/Tucker_Carlson [fair]
  - https://en.wikipedia.org/wiki/Chris_Klein_(actor) [low]
  - https://en.wikipedia.org/wiki/Eugene_Levy_(politician) [low]
\end{trajectorylisting}

\subsubsection*{Turn 5: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolNeutral}{Turn 5 model reasoning}
This search returned the series page and cast members, which are plausibly relevant for the actor-with-most-appearances facet. I'm not adding generic spillover.

Angle is still film series list language
but we still need a cleaner confirmation of which actor appears most, and then that actor's commencement address in 2012.
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 5 tool call(s)}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [
        "https://en.wikipedia.org/wiki/American_Pie_(film)",
        "https://en.wikipedia.org/wiki/Shannon_Elizabeth",
        "https://en.wikipedia.org/wiki/John_Cho",
        "https://en.wikipedia.org/wiki/Dan_Petronijevic"
      ],
      "importance": {
        "https://en.wikipedia.org/wiki/American_Pie_(film)": "high",
        "https://en.wikipedia.org/wiki/Shannon_Elizabeth": "fair",
        "https://en.wikipedia.org/wiki/John_Cho": "fair",
        "https://en.wikipedia.org/wiki/Dan_Petronijevic": "low"
      }
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 5 tool return 0}
RETURN 0.text:
Curated set updated (21/30): https://en.wikipedia.org/wiki/American_Pie_(film)[high], https://en.wikipedia.org/wiki/American_Pie_(film_series)[high], https://en.wikipedia.org/wiki/Eugene_Levy[high], https://en.wikipedia.org/wiki/List_of_American_Pie_characters[high], https://en.wikipedia.org/wiki/Seann_William_Scott[high], https://en.wikipedia.org/wiki/Ben_Carson[fair], https://en.wikipedia.org/wiki/Bradley_Cooper[fair], https://en.wikipedia.org/wiki/Chris_Owen_(actor)[fair], https://en.wikipedia.org/wiki/Ellis_Paul[fair], https://en.wikipedia.org/wiki/Jason_Biggs[fair], https://en.wikipedia.org/wiki/John_Cho[fair], https://en.wikipedia.org/wiki/Magic_Johnson[fair], https://en.wikipedia.org/wiki/Shannon_Elizabeth[fair], https://en.wikipedia.org/wiki/Steven_Curtis_Chapman[fair], https://en.wikipedia.org/wiki/Susan_Rice[fair], https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas[fair], https://en.wikipedia.org/wiki/Tim_Reid[fair], https://en.wikipedia.org/wiki/Tucker_Carlson[fair], https://en.wikipedia.org/wiki/Chris_Klein_(actor)[low], https://en.wikipedia.org/wiki/Dan_Petronijevic[low], https://en.wikipedia.org/wiki/Eugene_Levy_(politician)[low]
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 5 working-memory snapshot after harness update}
pool_size: 53
curated_size: 21 / 30
importance_counts: very_high=0, high=5, fair=13, low=3
curated_set:
  - https://en.wikipedia.org/wiki/American_Pie_(film) [high]
  - https://en.wikipedia.org/wiki/American_Pie_(film_series) [high]
  - https://en.wikipedia.org/wiki/Eugene_Levy [high]
  - https://en.wikipedia.org/wiki/List_of_American_Pie_characters [high]
  - https://en.wikipedia.org/wiki/Seann_William_Scott [high]
  - https://en.wikipedia.org/wiki/Ben_Carson [fair]
  - https://en.wikipedia.org/wiki/Bradley_Cooper [fair]
  - https://en.wikipedia.org/wiki/Chris_Owen_(actor) [fair]
  - https://en.wikipedia.org/wiki/Ellis_Paul [fair]
  - https://en.wikipedia.org/wiki/Jason_Biggs [fair]
  - https://en.wikipedia.org/wiki/John_Cho [fair]
  - https://en.wikipedia.org/wiki/Magic_Johnson [fair]
  - https://en.wikipedia.org/wiki/Shannon_Elizabeth [fair]
  - https://en.wikipedia.org/wiki/Steven_Curtis_Chapman [fair]
  - https://en.wikipedia.org/wiki/Susan_Rice [fair]
  - https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas [fair]
  - https://en.wikipedia.org/wiki/Tim_Reid [fair]
  - https://en.wikipedia.org/wiki/Tucker_Carlson [fair]
  - https://en.wikipedia.org/wiki/Chris_Klein_(actor) [low]
  - https://en.wikipedia.org/wiki/Dan_Petronijevic [low]
  - https://en.wikipedia.org/wiki/Eugene_Levy_(politician) [low]
\end{trajectorylisting}

\subsubsection*{Turn 6: \CaseTool{toolSearch}{search\_corpus}}
\begin{trajectorylisting}{toolNeutral}{Turn 6 model reasoning}
Gap: I need a cleaner source that tiebreaks the actor count; Seann William Scott is likely but Eugene Levy also appears in many. I'm switching angle to a biographical facet on Seann William Scott announcing a commencement address, because the university may be pinned to that doc rather than a generic series film count doc.
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 6 tool call(s)}
[
  {
    "tool": "search_corpus",
    "params": {
      "query": "Seann William Scott commencement address 2012 university"
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 6 tool return 0}
RETURN 0.text:

# DOCUMENT ID: https://en.wikipedia.org/wiki/List_of_NYU_Tisch_School_of_the_Arts_people (55 tokens)
List of NYU Tisch School of the Arts people - Wikipedia
Academy Award (1978), Annie Hall (1986); Hannah and her Sisters (2012); Midnight in Paris. Sean Baker, Director, producer, screenwriter, editor, B.F.A. ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Heath_Ledger (41 tokens)
Heath Ledger - Wikipedia
Heath Andrew Ledger (4 April 1979 - 22 January 2008) was an Australian actor. Known for his versatility across independent and major studio films, ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Jonathan_Franzen (42 tokens)
Jonathan Franzen - Wikipedia
Jonathan Earl Franzen (born August 17, 1959) is an American novelist and essayist. His 2001 novel The Corrections drew widespread critical acclaim, ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Joss_Whedon (43 tokens)
Joss Whedon - Wikipedia
Joseph Hill "Joss" Whedon is an American filmmaker, comic book writer, and composer. He is best known as the creator of several television series: the ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Wes_Craven (50 tokens)
Wes Craven - Wikipedia
Wesley Earl Craven (August 2, 1939 - August 30, 2015) was an American filmmaker. Amongst his prolific filmography, Craven worked primarily in the horror ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/List_of_Ethical_Culture_Fieldston_School_alumni (40 tokens)
List of Ethical Culture Fieldston School alumni - Wikipedia
This list of alumni of Ethical Culture Fieldston School includes graduates and non-graduate former students. Jill Abramson - former executive editor of The ...
[Context: 6623/30720]

RETURN 0.metadata:
{
  "metadata": {
    "returned_chunk_ids": [
      "https://en.wikipedia.org/wiki/List_of_NYU_Tisch_School_of_the_Arts_people",
      "https://en.wikipedia.org/wiki/Heath_Ledger",
      "https://en.wikipedia.org/wiki/Jonathan_Franzen",
      "https://en.wikipedia.org/wiki/Joss_Whedon",
      "https://en.wikipedia.org/wiki/Wes_Craven",
      "https://en.wikipedia.org/wiki/List_of_Ethical_Culture_Fieldston_School_alumni"
    ],
    "pre_rerank_chunk_ids": null
  }
}
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 6 working-memory snapshot after harness update}
pool_size: 59
curated_size: 21 / 30
importance_counts: very_high=0, high=5, fair=13, low=3
curated_set:
  - https://en.wikipedia.org/wiki/American_Pie_(film) [high]
  - https://en.wikipedia.org/wiki/American_Pie_(film_series) [high]
  - https://en.wikipedia.org/wiki/Eugene_Levy [high]
  - https://en.wikipedia.org/wiki/List_of_American_Pie_characters [high]
  - https://en.wikipedia.org/wiki/Seann_William_Scott [high]
  - https://en.wikipedia.org/wiki/Ben_Carson [fair]
  - https://en.wikipedia.org/wiki/Bradley_Cooper [fair]
  - https://en.wikipedia.org/wiki/Chris_Owen_(actor) [fair]
  - https://en.wikipedia.org/wiki/Ellis_Paul [fair]
  - https://en.wikipedia.org/wiki/Jason_Biggs [fair]
  - https://en.wikipedia.org/wiki/John_Cho [fair]
  - https://en.wikipedia.org/wiki/Magic_Johnson [fair]
  - https://en.wikipedia.org/wiki/Shannon_Elizabeth [fair]
  - https://en.wikipedia.org/wiki/Steven_Curtis_Chapman [fair]
  - https://en.wikipedia.org/wiki/Susan_Rice [fair]
  - https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas [fair]
  - https://en.wikipedia.org/wiki/Tim_Reid [fair]
  - https://en.wikipedia.org/wiki/Tucker_Carlson [fair]
  - https://en.wikipedia.org/wiki/Chris_Klein_(actor) [low]
  - https://en.wikipedia.org/wiki/Dan_Petronijevic [low]
  - https://en.wikipedia.org/wiki/Eugene_Levy_(politician) [low]
\end{trajectorylisting}

\subsubsection*{Turn 7: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolNeutral}{Turn 7 model reasoning}
This search angle is exhausted so far, yielding NYU people/spillover and no Seann William Scott commencement doc. We need to curate whatever is plausibly relevant from the last search results before changing angle.

The missed facet: maybe the actor is Eugene Levy, not Seann; maybe the commencement was at an institution like Syracuse University, but the search directly on Seann William Scott + commencement address is not returning. We are at angle exhaustion; let me curate before abandoning the actor with most appearances facet and try a different decomposition.
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 7 tool call(s)}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [
        "https://en.wikipedia.org/wiki/Heath_Ledger",
        "https://en.wikipedia.org/wiki/Jonathan_Franzen",
        "https://en.wikipedia.org/wiki/Joss_Whedon",
        "https://en.wikipedia.org/wiki/Wes_Craven",
        "https://en.wikipedia.org/wiki/List_of_NYU_Tisch_School_of_the_Arts_people"
      ],
      "importance": {
        "https://en.wikipedia.org/wiki/Heath_Ledger": "low",
        "https://en.wikipedia.org/wiki/Jonathan_Franzen": "low",
        "https://en.wikipedia.org/wiki/Joss_Whedon": "low",
        "https://en.wikipedia.org/wiki/Wes_Craven": "low",
        "https://en.wikipedia.org/wiki/List_of_NYU_Tisch_School_of_the_Arts_people": "low"
      }
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 7 tool return 0}
RETURN 0.text:
Curated set updated (26/30): https://en.wikipedia.org/wiki/American_Pie_(film)[high], https://en.wikipedia.org/wiki/American_Pie_(film_series)[high], https://en.wikipedia.org/wiki/Eugene_Levy[high], https://en.wikipedia.org/wiki/List_of_American_Pie_characters[high], https://en.wikipedia.org/wiki/Seann_William_Scott[high], https://en.wikipedia.org/wiki/Ben_Carson[fair], https://en.wikipedia.org/wiki/Bradley_Cooper[fair], https://en.wikipedia.org/wiki/Chris_Owen_(actor)[fair], https://en.wikipedia.org/wiki/Ellis_Paul[fair], https://en.wikipedia.org/wiki/Jason_Biggs[fair], https://en.wikipedia.org/wiki/John_Cho[fair], https://en.wikipedia.org/wiki/Magic_Johnson[fair], https://en.wikipedia.org/wiki/Shannon_Elizabeth[fair], https://en.wikipedia.org/wiki/Steven_Curtis_Chapman[fair], https://en.wikipedia.org/wiki/Susan_Rice[fair], https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas[fair], https://en.wikipedia.org/wiki/Tim_Reid[fair], https://en.wikipedia.org/wiki/Tucker_Carlson[fair], https://en.wikipedia.org/wiki/Chris_Klein_(actor)[low], https://en.wikipedia.org/wiki/Dan_Petronijevic[low], https://en.wikipedia.org/wiki/Eugene_Levy_(politician)[low], https://en.wikipedia.org/wiki/Heath_Ledger[low], https://en.wikipedia.org/wiki/Jonathan_Franzen[low], https://en.wikipedia.org/wiki/Joss_Whedon[low], https://en.wikipedia.org/wiki/List_of_NYU_Tisch_School_of_the_Arts_people[low], https://en.wikipedia.org/wiki/Wes_Craven[low]
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 7 working-memory snapshot after harness update}
pool_size: 59
curated_size: 26 / 30
importance_counts: very_high=0, high=5, fair=13, low=8
curated_set:
  - https://en.wikipedia.org/wiki/American_Pie_(film) [high]
  - https://en.wikipedia.org/wiki/American_Pie_(film_series) [high]
  - https://en.wikipedia.org/wiki/Eugene_Levy [high]
  - https://en.wikipedia.org/wiki/List_of_American_Pie_characters [high]
  - https://en.wikipedia.org/wiki/Seann_William_Scott [high]
  - https://en.wikipedia.org/wiki/Ben_Carson [fair]
  - https://en.wikipedia.org/wiki/Bradley_Cooper [fair]
  - https://en.wikipedia.org/wiki/Chris_Owen_(actor) [fair]
  - https://en.wikipedia.org/wiki/Ellis_Paul [fair]
  - https://en.wikipedia.org/wiki/Jason_Biggs [fair]
  - https://en.wikipedia.org/wiki/John_Cho [fair]
  - https://en.wikipedia.org/wiki/Magic_Johnson [fair]
  - https://en.wikipedia.org/wiki/Shannon_Elizabeth [fair]
  - https://en.wikipedia.org/wiki/Steven_Curtis_Chapman [fair]
  - https://en.wikipedia.org/wiki/Susan_Rice [fair]
  - https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas [fair]
  - https://en.wikipedia.org/wiki/Tim_Reid [fair]
  - https://en.wikipedia.org/wiki/Tucker_Carlson [fair]
  - https://en.wikipedia.org/wiki/Chris_Klein_(actor) [low]
  - https://en.wikipedia.org/wiki/Dan_Petronijevic [low]
  - https://en.wikipedia.org/wiki/Eugene_Levy_(politician) [low]
  - https://en.wikipedia.org/wiki/Heath_Ledger [low]
  - https://en.wikipedia.org/wiki/Jonathan_Franzen [low]
  - https://en.wikipedia.org/wiki/Joss_Whedon [low]
  - https://en.wikipedia.org/wiki/List_of_NYU_Tisch_School_of_the_Arts_people [low]
  - https://en.wikipedia.org/wiki/Wes_Craven [low]
\end{trajectorylisting}

\subsubsection*{Turn 8: \CaseTool{toolGrep}{grep\_corpus}}
\begin{trajectorylisting}{toolNeutral}{Turn 8 model reasoning}
Current angle is exhausted. What isn't working is Seann William Scott link phrases to commencement address. Re-reading the query: actor with most American Pie appearances (incl. spinoffs, up to 2020) -> likely Eugene Levy or Seann William Scott; commencement address in 2012 -> a person/homepage/commencement list. Gap: I need the specific actor count and commencement address as separate narrow facets; using person biographies for commencement likely better than Seann search. New strategy: search grep on Eugene William Scott + commencement/address and separately on Eugene Levy + commencement to see if university appears in their bio pages.
\end{trajectorylisting}

\begin{trajectorylisting}{toolGrep}{Turn 8 tool call(s)}
[
  {
    "tool": "grep_corpus",
    "params": {
      "pattern": "Seann William Scott commencement|Eugene Levy commencement|Seann William Scott address|Eugene Levy address|2012 commencement"
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolGrep}{Turn 8 tool return 0}
RETURN 0.text:

# DOCUMENT ID: https://en.wikipedia.org/wiki/Donald_Sutherland (44 tokens)
Donald Sutherland - Wikipedia
Donald McNichol Sutherland (17 July 1935 - 20 June 2024) was a Canadian actor. With a career spanning six decades, he received numerous accolades, ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Good_Will_Hunting (43 tokens)
Good Will Hunting - Wikipedia
Good Will Hunting is a 1997 American drama film directed by Gus Van Sant and written by Ben Affleck and Matt Damon. It stars Damon, Affleck, Robin Williams, ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Bradley_Whitford (37 tokens)
Bradley Whitford - Wikipedia
He delivered the commencement address at the University of Wisconsin-Madison in 2004. He was the keynote speaker for Class Day at Princeton University ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/John_Lithgow (36 tokens)
John Lithgow - Wikipedia
John Arthur Lithgow is an American actor. He studied at Harvard University and the London Academy of Music and Dramatic Art before becoming known for his ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/List_of_University_at_Buffalo_people (43 tokens)
List of University at Buffalo people - Wikipedia
This is a list of people connected to the University at Buffalo. There are more than 260,000 living alumni of UB. Notable alumni include the CEOs of ...
[Context: 6824/30720]

RETURN 0.metadata:
{
  "metadata": {
    "returned_chunk_ids": [
      "https://en.wikipedia.org/wiki/Donald_Sutherland",
      "https://en.wikipedia.org/wiki/Good_Will_Hunting",
      "https://en.wikipedia.org/wiki/Bradley_Whitford",
      "https://en.wikipedia.org/wiki/John_Lithgow",
      "https://en.wikipedia.org/wiki/List_of_University_at_Buffalo_people"
    ]
  }
}
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 8 working-memory snapshot after harness update}
pool_size: 64
curated_size: 26 / 30
importance_counts: very_high=0, high=5, fair=13, low=8
curated_set:
  - https://en.wikipedia.org/wiki/American_Pie_(film) [high]
  - https://en.wikipedia.org/wiki/American_Pie_(film_series) [high]
  - https://en.wikipedia.org/wiki/Eugene_Levy [high]
  - https://en.wikipedia.org/wiki/List_of_American_Pie_characters [high]
  - https://en.wikipedia.org/wiki/Seann_William_Scott [high]
  - https://en.wikipedia.org/wiki/Ben_Carson [fair]
  - https://en.wikipedia.org/wiki/Bradley_Cooper [fair]
  - https://en.wikipedia.org/wiki/Chris_Owen_(actor) [fair]
  - https://en.wikipedia.org/wiki/Ellis_Paul [fair]
  - https://en.wikipedia.org/wiki/Jason_Biggs [fair]
  - https://en.wikipedia.org/wiki/John_Cho [fair]
  - https://en.wikipedia.org/wiki/Magic_Johnson [fair]
  - https://en.wikipedia.org/wiki/Shannon_Elizabeth [fair]
  - https://en.wikipedia.org/wiki/Steven_Curtis_Chapman [fair]
  - https://en.wikipedia.org/wiki/Susan_Rice [fair]
  - https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas [fair]
  - https://en.wikipedia.org/wiki/Tim_Reid [fair]
  - https://en.wikipedia.org/wiki/Tucker_Carlson [fair]
  - https://en.wikipedia.org/wiki/Chris_Klein_(actor) [low]
  - https://en.wikipedia.org/wiki/Dan_Petronijevic [low]
  - https://en.wikipedia.org/wiki/Eugene_Levy_(politician) [low]
  - https://en.wikipedia.org/wiki/Heath_Ledger [low]
  - https://en.wikipedia.org/wiki/Jonathan_Franzen [low]
  - https://en.wikipedia.org/wiki/Joss_Whedon [low]
  - https://en.wikipedia.org/wiki/List_of_NYU_Tisch_School_of_the_Arts_people [low]
  - https://en.wikipedia.org/wiki/Wes_Craven [low]
\end{trajectorylisting}

\subsubsection*{Turn 9: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolNeutral}{Turn 9 model reasoning}
The grep result is stale and weak; it found no Seann/Eugene commencement docs. Still need to curate aggressively now because of the required rhythm. Plausibly relevant are person/bio/address spillover docs from the grep set. The missed facet: biography/commencement address linkage rather than main page text.
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 9 tool call(s)}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [
        "https://en.wikipedia.org/wiki/David_Sutherland",
        "https://en.wikipedia.org/wiki/Donald_Sutherland",
        "https://en.wikipedia.org/wiki/John_Lithgow",
        "https://en.wikipedia.org/wiki/Bradley_Whitford",
        "https://en.wikipedia.org/wiki/List_of_University_at_Buffalo_people"
      ],
      "importance": {
        "https://en.wikipedia.org/wiki/David_Sutherland": "low",
        "https://en.wikipedia.org/wiki/Donald_Sutherland": "low",
        "https://en.wikipedia.org/wiki/John_Lithgow": "low",
        "https://en.wikipedia.org/wiki/Bradley_Whitford": "low",
        "https://en.wikipedia.org/wiki/List_of_University_at_Buffalo_people": "low"
      }
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 9 tool return 0}
RETURN 0.text:
Curated set updated (30/30): https://en.wikipedia.org/wiki/American_Pie_(film)[high], https://en.wikipedia.org/wiki/American_Pie_(film_series)[high], https://en.wikipedia.org/wiki/Eugene_Levy[high], https://en.wikipedia.org/wiki/List_of_American_Pie_characters[high], https://en.wikipedia.org/wiki/Seann_William_Scott[high], https://en.wikipedia.org/wiki/Ben_Carson[fair], https://en.wikipedia.org/wiki/Bradley_Cooper[fair], https://en.wikipedia.org/wiki/Chris_Owen_(actor)[fair], https://en.wikipedia.org/wiki/Ellis_Paul[fair], https://en.wikipedia.org/wiki/Jason_Biggs[fair], https://en.wikipedia.org/wiki/John_Cho[fair], https://en.wikipedia.org/wiki/Magic_Johnson[fair], https://en.wikipedia.org/wiki/Shannon_Elizabeth[fair], https://en.wikipedia.org/wiki/Steven_Curtis_Chapman[fair], https://en.wikipedia.org/wiki/Susan_Rice[fair], https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas[fair], https://en.wikipedia.org/wiki/Tim_Reid[fair], https://en.wikipedia.org/wiki/Tucker_Carlson[fair], https://en.wikipedia.org/wiki/Bradley_Whitford[low], https://en.wikipedia.org/wiki/Chris_Klein_(actor)[low], https://en.wikipedia.org/wiki/Dan_Petronijevic[low], https://en.wikipedia.org/wiki/David_Sutherland[low], https://en.wikipedia.org/wiki/Donald_Sutherland[low], https://en.wikipedia.org/wiki/Eugene_Levy_(politician)[low], https://en.wikipedia.org/wiki/Heath_Ledger[low], https://en.wikipedia.org/wiki/John_Lithgow[low], https://en.wikipedia.org/wiki/Jonathan_Franzen[low], https://en.wikipedia.org/wiki/Joss_Whedon[low], https://en.wikipedia.org/wiki/List_of_NYU_Tisch_School_of_the_Arts_people[low], https://en.wikipedia.org/wiki/Wes_Craven[low]
[CAPACITY] Set is FULL and no evictable lower-importance docs - 1 doc(s) NOT added: https://en.wikipedia.org/wiki/List_of_University_at_Buffalo_people
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 9 working-memory snapshot after harness update}
pool_size: 64
curated_size: 30 / 30
importance_counts: very_high=0, high=5, fair=13, low=12
curated_set:
  - https://en.wikipedia.org/wiki/American_Pie_(film) [high]
  - https://en.wikipedia.org/wiki/American_Pie_(film_series) [high]
  - https://en.wikipedia.org/wiki/Eugene_Levy [high]
  - https://en.wikipedia.org/wiki/List_of_American_Pie_characters [high]
  - https://en.wikipedia.org/wiki/Seann_William_Scott [high]
  - https://en.wikipedia.org/wiki/Ben_Carson [fair]
  - https://en.wikipedia.org/wiki/Bradley_Cooper [fair]
  - https://en.wikipedia.org/wiki/Chris_Owen_(actor) [fair]
  - https://en.wikipedia.org/wiki/Ellis_Paul [fair]
  - https://en.wikipedia.org/wiki/Jason_Biggs [fair]
  - https://en.wikipedia.org/wiki/John_Cho [fair]
  - https://en.wikipedia.org/wiki/Magic_Johnson [fair]
  - https://en.wikipedia.org/wiki/Shannon_Elizabeth [fair]
  - https://en.wikipedia.org/wiki/Steven_Curtis_Chapman [fair]
  - https://en.wikipedia.org/wiki/Susan_Rice [fair]
  - https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas [fair]
  - https://en.wikipedia.org/wiki/Tim_Reid [fair]
  - https://en.wikipedia.org/wiki/Tucker_Carlson [fair]
  - https://en.wikipedia.org/wiki/Bradley_Whitford [low]
  - https://en.wikipedia.org/wiki/Chris_Klein_(actor) [low]
  - https://en.wikipedia.org/wiki/Dan_Petronijevic [low]
  - https://en.wikipedia.org/wiki/David_Sutherland [low]
  - https://en.wikipedia.org/wiki/Donald_Sutherland [low]
  - https://en.wikipedia.org/wiki/Eugene_Levy_(politician) [low]
  - https://en.wikipedia.org/wiki/Heath_Ledger [low]
  - https://en.wikipedia.org/wiki/John_Lithgow [low]
  - https://en.wikipedia.org/wiki/Jonathan_Franzen [low]
  - https://en.wikipedia.org/wiki/Joss_Whedon [low]
  - https://en.wikipedia.org/wiki/List_of_NYU_Tisch_School_of_the_Arts_people [low]
  - https://en.wikipedia.org/wiki/Wes_Craven [low]
\end{trajectorylisting}

\subsubsection*{Turn 10: \CaseTool{toolVerify}{verify}}
\begin{trajectorylisting}{toolNeutral}{Turn 10 model reasoning}
Gap: I'm stuck on the commencement address facet; searching by name + address is failing. Re-reading the query, another missed facet is the second entity: 'most movies in the series (including spinoffs, as of 2020)'. That likely points to Eugene Levy (appears in much of the series) rather than Seann. So before changing angle more strongly, I should verify which actor appears most. Using verify now on the biographical docs directly tied to the likely actors could strengthen the actor facet and allow independent searches on the commencement facet from a better source.
\end{trajectorylisting}

\begin{trajectorylisting}{toolVerify}{Turn 10 tool call(s)}
[
  {
    "tool": "verify",
    "params": {
      "doc_ids": [
        "https://en.wikipedia.org/wiki/Seann_William_Scott",
        "https://en.wikipedia.org/wiki/Eugene_Levy"
      ],
      "claim": "Seann William Scott or Eugene Levy has appeared in more American Pie films (including spinoffs up to 2020) than any other American Pie actor"
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolVerify}{Turn 10 tool return 0}
RETURN 0.text:
verify: no matching docs found in memory.
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 10 working-memory snapshot after harness update}
pool_size: 64
curated_size: 30 / 30
importance_counts: very_high=0, high=5, fair=13, low=12
curated_set:
  - https://en.wikipedia.org/wiki/American_Pie_(film) [high]
  - https://en.wikipedia.org/wiki/American_Pie_(film_series) [high]
  - https://en.wikipedia.org/wiki/Eugene_Levy [high]
  - https://en.wikipedia.org/wiki/List_of_American_Pie_characters [high]
  - https://en.wikipedia.org/wiki/Seann_William_Scott [high]
  - https://en.wikipedia.org/wiki/Ben_Carson [fair]
  - https://en.wikipedia.org/wiki/Bradley_Cooper [fair]
  - https://en.wikipedia.org/wiki/Chris_Owen_(actor) [fair]
  - https://en.wikipedia.org/wiki/Ellis_Paul [fair]
  - https://en.wikipedia.org/wiki/Jason_Biggs [fair]
  - https://en.wikipedia.org/wiki/John_Cho [fair]
  - https://en.wikipedia.org/wiki/Magic_Johnson [fair]
  - https://en.wikipedia.org/wiki/Shannon_Elizabeth [fair]
  - https://en.wikipedia.org/wiki/Steven_Curtis_Chapman [fair]
  - https://en.wikipedia.org/wiki/Susan_Rice [fair]
  - https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas [fair]
  - https://en.wikipedia.org/wiki/Tim_Reid [fair]
  - https://en.wikipedia.org/wiki/Tucker_Carlson [fair]
  - https://en.wikipedia.org/wiki/Bradley_Whitford [low]
  - https://en.wikipedia.org/wiki/Chris_Klein_(actor) [low]
  - https://en.wikipedia.org/wiki/Dan_Petronijevic [low]
  - https://en.wikipedia.org/wiki/David_Sutherland [low]
  - https://en.wikipedia.org/wiki/Donald_Sutherland [low]
  - https://en.wikipedia.org/wiki/Eugene_Levy_(politician) [low]
  - https://en.wikipedia.org/wiki/Heath_Ledger [low]
  - https://en.wikipedia.org/wiki/John_Lithgow [low]
  - https://en.wikipedia.org/wiki/Jonathan_Franzen [low]
  - https://en.wikipedia.org/wiki/Joss_Whedon [low]
  - https://en.wikipedia.org/wiki/List_of_NYU_Tisch_School_of_the_Arts_people [low]
  - https://en.wikipedia.org/wiki/Wes_Craven [low]
\end{trajectorylisting}

\subsubsection*{Turn 11: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolNeutral}{Turn 11 model reasoning}
I just verified, but that does not bypass the required curvature after searching. The verify result is a non-search step, but the last real search that produced text was grep on '2012 commencement', whose result set is stale. I should curate the plausibly relevant leftovers from the last search angle before changing to commencement-date searching on the actor instead. The corridor doc is likely Eugene Levy as the actor count; I need a better commencement link angle on that actor or an alternative actor.
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 11 tool call(s)}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [
        "https://en.wikipedia.org/wiki/Eugene_Levy_(politician)"
      ],
      "importance": {
        "https://en.wikipedia.org/wiki/Eugene_Levy_(politician)": "low"
      }
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 11 tool return 0}
RETURN 0.text:
Curated set updated (30/30): https://en.wikipedia.org/wiki/American_Pie_(film)[high], https://en.wikipedia.org/wiki/American_Pie_(film_series)[high], https://en.wikipedia.org/wiki/Eugene_Levy[high], https://en.wikipedia.org/wiki/List_of_American_Pie_characters[high], https://en.wikipedia.org/wiki/Seann_William_Scott[high], https://en.wikipedia.org/wiki/Ben_Carson[fair], https://en.wikipedia.org/wiki/Bradley_Cooper[fair], https://en.wikipedia.org/wiki/Chris_Owen_(actor)[fair], https://en.wikipedia.org/wiki/Ellis_Paul[fair], https://en.wikipedia.org/wiki/Jason_Biggs[fair], https://en.wikipedia.org/wiki/John_Cho[fair], https://en.wikipedia.org/wiki/Magic_Johnson[fair], https://en.wikipedia.org/wiki/Shannon_Elizabeth[fair], https://en.wikipedia.org/wiki/Steven_Curtis_Chapman[fair], https://en.wikipedia.org/wiki/Susan_Rice[fair], https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas[fair], https://en.wikipedia.org/wiki/Tim_Reid[fair], https://en.wikipedia.org/wiki/Tucker_Carlson[fair], https://en.wikipedia.org/wiki/Bradley_Whitford[low], https://en.wikipedia.org/wiki/Chris_Klein_(actor)[low], https://en.wikipedia.org/wiki/Dan_Petronijevic[low], https://en.wikipedia.org/wiki/David_Sutherland[low], https://en.wikipedia.org/wiki/Donald_Sutherland[low], https://en.wikipedia.org/wiki/Eugene_Levy_(politician)[low], https://en.wikipedia.org/wiki/Heath_Ledger[low], https://en.wikipedia.org/wiki/John_Lithgow[low], https://en.wikipedia.org/wiki/Jonathan_Franzen[low], https://en.wikipedia.org/wiki/Joss_Whedon[low], https://en.wikipedia.org/wiki/List_of_NYU_Tisch_School_of_the_Arts_people[low], https://en.wikipedia.org/wiki/Wes_Craven[low]
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 11 working-memory snapshot after harness update}
pool_size: 64
curated_size: 30 / 30
importance_counts: very_high=0, high=5, fair=13, low=12
curated_set:
  - https://en.wikipedia.org/wiki/American_Pie_(film) [high]
  - https://en.wikipedia.org/wiki/American_Pie_(film_series) [high]
  - https://en.wikipedia.org/wiki/Eugene_Levy [high]
  - https://en.wikipedia.org/wiki/List_of_American_Pie_characters [high]
  - https://en.wikipedia.org/wiki/Seann_William_Scott [high]
  - https://en.wikipedia.org/wiki/Ben_Carson [fair]
  - https://en.wikipedia.org/wiki/Bradley_Cooper [fair]
  - https://en.wikipedia.org/wiki/Chris_Owen_(actor) [fair]
  - https://en.wikipedia.org/wiki/Ellis_Paul [fair]
  - https://en.wikipedia.org/wiki/Jason_Biggs [fair]
  - https://en.wikipedia.org/wiki/John_Cho [fair]
  - https://en.wikipedia.org/wiki/Magic_Johnson [fair]
  - https://en.wikipedia.org/wiki/Shannon_Elizabeth [fair]
  - https://en.wikipedia.org/wiki/Steven_Curtis_Chapman [fair]
  - https://en.wikipedia.org/wiki/Susan_Rice [fair]
  - https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas [fair]
  - https://en.wikipedia.org/wiki/Tim_Reid [fair]
  - https://en.wikipedia.org/wiki/Tucker_Carlson [fair]
  - https://en.wikipedia.org/wiki/Bradley_Whitford [low]
  - https://en.wikipedia.org/wiki/Chris_Klein_(actor) [low]
  - https://en.wikipedia.org/wiki/Dan_Petronijevic [low]
  - https://en.wikipedia.org/wiki/David_Sutherland [low]
  - https://en.wikipedia.org/wiki/Donald_Sutherland [low]
  - https://en.wikipedia.org/wiki/Eugene_Levy_(politician) [low]
  - https://en.wikipedia.org/wiki/Heath_Ledger [low]
  - https://en.wikipedia.org/wiki/John_Lithgow [low]
  - https://en.wikipedia.org/wiki/Jonathan_Franzen [low]
  - https://en.wikipedia.org/wiki/Joss_Whedon [low]
  - https://en.wikipedia.org/wiki/List_of_NYU_Tisch_School_of_the_Arts_people [low]
  - https://en.wikipedia.org/wiki/Wes_Craven [low]
\end{trajectorylisting}

\subsubsection*{Turn 12: \CaseTool{toolSearch}{search\_corpus}}
\begin{trajectorylisting}{toolNeutral}{Turn 12 model reasoning}
My current search angle is exhausted. Let me rethink. The missed facet is the full biography/commencement link rather than phrase searching. The actor tied to the most American Pie films is Eugene Levy; Seann William appears in 4, Eugene in 12+. Eugene has also done Phoenix film premieres and biographical speeches, but the address was delivered at a university in 2012. A different angle: search commencement/address by Eugene Levy + 2012, or search a university that had a commencement speaker in 2012 and is linked to Eugene Levy. Also consider that the actor could be Seann William Scott if Eugene Levy is not counted as 'most' under some definition, so search Seann 2012 commencement separately but through a biography-angle query rather than fit-term.
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 12 tool call(s)}
[
  {
    "tool": "search_corpus",
    "params": {
      "query": "Eugene Levy 2012 commencement address university biographical speaker 2012"
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 12 tool return 0}
RETURN 0.text:

# DOCUMENT ID: https://en.wikipedia.org/wiki/Princeton_University (38 tokens)
Princeton University - Wikipedia
Princeton University is a private Ivy League research university in Princeton, New Jersey, United States. Founded in 1746 in Elizabeth as the College of New ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/List_of_University_of_Michigan_alumni (41 tokens)
List of University of Michigan alumni - Wikipedia
The following is a list of University of Michigan alumni. There are more than 640,000 living alumni of the University of Michigan in 180 countries across ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/List_of_Cornell_University_alumni (31 tokens)
List of Cornell University alumni - Wikipedia
This list of Cornell University alumni includes notable graduates, non-graduate former students, and current students of Cornell University.

# DOCUMENT ID: https://en.wikipedia.org/wiki/University_of_St._Thomas_(Minnesota) (37 tokens)
University of St. Thomas (Minnesota) - Wikipedia
The University of St. Thomas is a private Catholic research university with campuses in Saint Paul and Minneapolis, Minnesota, United States.

# DOCUMENT ID: https://en.wikipedia.org/wiki/List_of_Queens_College_people (43 tokens)
List of Queens College people - Wikipedia
This is a list of notable alumni and faculty of Queens College, City University of New York. Contents. 1 Business; 2 Education; 3 Entertainment and media ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/California_Institute_of_Technology (36 tokens)
California Institute of Technology - Wikipedia
The California Institute of Technology (branded as Caltech) is a private research university/institute of technology in Pasadena, California, United States.

# DOCUMENT ID: https://en.wikipedia.org/wiki/List_of_Massachusetts_Institute_of_Technology_alumni (34 tokens)
List of Massachusetts Institute of Technology alumni - Wikipedia
This list of Massachusetts Institute of Technology alumni includes students who studied as undergraduates or graduate students at MIT's School of Engineering

# DOCUMENT ID: https://en.wikipedia.org/wiki/Steve_Jobs (44 tokens)
Steve Jobs - Wikipedia
Steven Paul Jobs (February 24, 1955 - October 5, 2011) was an American businessman, inventor, and investor. A pioneer of the personal computer revolution of ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Prem_Rawat (40 tokens)
Prem Rawat - Wikipedia
Prem Pal Singh Rawat (born 10 December 1957), formerly known as Maharaji, is an Indian international speaker and author. His teachings include a meditation ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/John_H._Johnson (47 tokens)
John H. Johnson - Wikipedia
John Harold Johnson (January 19, 1918 - August 8, 2005) was an American business executive and publisher. He was the founder in 1942 of the Johnson ...
[Context: 7403/30720]

RETURN 0.metadata:
{
  "metadata": {
    "returned_chunk_ids": [
      "https://en.wikipedia.org/wiki/Princeton_University",
      "https://en.wikipedia.org/wiki/List_of_University_of_Michigan_alumni",
      "https://en.wikipedia.org/wiki/List_of_Cornell_University_alumni",
      "https://en.wikipedia.org/wiki/University_of_St._Thomas_(Minnesota)",
      "https://en.wikipedia.org/wiki/List_of_Queens_College_people",
      "https://en.wikipedia.org/wiki/California_Institute_of_Technology",
      "https://en.wikipedia.org/wiki/List_of_Massachusetts_Institute_of_Technology_alumni",
      "https://en.wikipedia.org/wiki/Steve_Jobs",
      "https://en.wikipedia.org/wiki/Prem_Rawat",
      "https://en.wikipedia.org/wiki/John_H._Johnson"
    ],
    "pre_rerank_chunk_ids": null
  }
}
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 12 working-memory snapshot after harness update}
pool_size: 74
curated_size: 30 / 30
importance_counts: very_high=0, high=5, fair=13, low=12
curated_set:
  - https://en.wikipedia.org/wiki/American_Pie_(film) [high]
  - https://en.wikipedia.org/wiki/American_Pie_(film_series) [high]
  - https://en.wikipedia.org/wiki/Eugene_Levy [high]
  - https://en.wikipedia.org/wiki/List_of_American_Pie_characters [high]
  - https://en.wikipedia.org/wiki/Seann_William_Scott [high]
  - https://en.wikipedia.org/wiki/Ben_Carson [fair]
  - https://en.wikipedia.org/wiki/Bradley_Cooper [fair]
  - https://en.wikipedia.org/wiki/Chris_Owen_(actor) [fair]
  - https://en.wikipedia.org/wiki/Ellis_Paul [fair]
  - https://en.wikipedia.org/wiki/Jason_Biggs [fair]
  - https://en.wikipedia.org/wiki/John_Cho [fair]
  - https://en.wikipedia.org/wiki/Magic_Johnson [fair]
  - https://en.wikipedia.org/wiki/Shannon_Elizabeth [fair]
  - https://en.wikipedia.org/wiki/Steven_Curtis_Chapman [fair]
  - https://en.wikipedia.org/wiki/Susan_Rice [fair]
  - https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas [fair]
  - https://en.wikipedia.org/wiki/Tim_Reid [fair]
  - https://en.wikipedia.org/wiki/Tucker_Carlson [fair]
  - https://en.wikipedia.org/wiki/Bradley_Whitford [low]
  - https://en.wikipedia.org/wiki/Chris_Klein_(actor) [low]
  - https://en.wikipedia.org/wiki/Dan_Petronijevic [low]
  - https://en.wikipedia.org/wiki/David_Sutherland [low]
  - https://en.wikipedia.org/wiki/Donald_Sutherland [low]
  - https://en.wikipedia.org/wiki/Eugene_Levy_(politician) [low]
  - https://en.wikipedia.org/wiki/Heath_Ledger [low]
  - https://en.wikipedia.org/wiki/John_Lithgow [low]
  - https://en.wikipedia.org/wiki/Jonathan_Franzen [low]
  - https://en.wikipedia.org/wiki/Joss_Whedon [low]
  - https://en.wikipedia.org/wiki/List_of_NYU_Tisch_School_of_the_Arts_people [low]
  - https://en.wikipedia.org/wiki/Wes_Craven [low]
\end{trajectorylisting}

\subsubsection*{Turn 13: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolNeutral}{Turn 13 model reasoning}
The last search was a biography/bio-address angle on Eugene Levy. It surfaced several university/general alumni/link pages likely not directly his commencement, but they are plausibly relevant incoming links because many ceremony pages link biographical pages. The missed facet is average/conservative reading of groom constraints: need to capture the actor-under-commencement entity link, not just the actor identity. Since reception found primarily university pages, these could connect to Eugene Levy via a commencement/speech biography note. This is a completely different angle from exact commencement-address search: linking university not the actor.
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 13 tool call(s)}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [
        "https://en.wikipedia.org/wiki/Princeton_University",
        "https://en.wikipedia.org/wiki/List_of_University_of_Michigan_alumni",
        "https://en.wikipedia.org/wiki/List_of_Cornell_University_alumni",
        "https://en.wikipedia.org/wiki/University_of_St._Thomas_(Minnesota)",
        "https://en.wikipedia.org/wiki/List_of_Queens_Colege_people"
      ],
      "importance": {
        "https://en.wikipedia.org/wiki/Princeton_University": "fair",
        "https://en.wikipedia.org/wiki/List_of_University_of_Michigan_alumni": "low",
        "https://en.wikipedia.org/wiki/List_of_Cornell_University_alumni": "low",
        "https://en.wikipedia.org/wiki/University_of_St._Thomas_(Minnesota)": "low",
        "https://en.wikipedia.org/wiki/List_of_Queens_Colege_people": "low"
      }
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 13 tool return 0}
RETURN 0.text:
Curated set updated (30/30): https://en.wikipedia.org/wiki/American_Pie_(film)[high], https://en.wikipedia.org/wiki/American_Pie_(film_series)[high], https://en.wikipedia.org/wiki/Eugene_Levy[high], https://en.wikipedia.org/wiki/List_of_American_Pie_characters[high], https://en.wikipedia.org/wiki/Seann_William_Scott[high], https://en.wikipedia.org/wiki/Ben_Carson[fair], https://en.wikipedia.org/wiki/Bradley_Cooper[fair], https://en.wikipedia.org/wiki/Chris_Owen_(actor)[fair], https://en.wikipedia.org/wiki/Ellis_Paul[fair], https://en.wikipedia.org/wiki/Jason_Biggs[fair], https://en.wikipedia.org/wiki/John_Cho[fair], https://en.wikipedia.org/wiki/Magic_Johnson[fair], https://en.wikipedia.org/wiki/Princeton_University[fair], https://en.wikipedia.org/wiki/Shannon_Elizabeth[fair], https://en.wikipedia.org/wiki/Steven_Curtis_Chapman[fair], https://en.wikipedia.org/wiki/Susan_Rice[fair], https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas[fair], https://en.wikipedia.org/wiki/Tim_Reid[fair], https://en.wikipedia.org/wiki/Tucker_Carlson[fair], https://en.wikipedia.org/wiki/Bradley_Whitford[low], https://en.wikipedia.org/wiki/Dan_Petronijevic[low], https://en.wikipedia.org/wiki/David_Sutherland[low], https://en.wikipedia.org/wiki/Donald_Sutherland[low], https://en.wikipedia.org/wiki/Eugene_Levy_(politician)[low], https://en.wikipedia.org/wiki/Heath_Ledger[low], https://en.wikipedia.org/wiki/John_Lithgow[low], https://en.wikipedia.org/wiki/Jonathan_Franzen[low], https://en.wikipedia.org/wiki/Joss_Whedon[low], https://en.wikipedia.org/wiki/List_of_NYU_Tisch_School_of_the_Arts_people[low], https://en.wikipedia.org/wiki/Wes_Craven[low]
[EVICTED low-importance] 1 doc(s): https://en.wikipedia.org/wiki/Chris_Klein_(actor)
[CAPACITY] Set is FULL and no evictable lower-importance docs - 4 doc(s) NOT added: https://en.wikipedia.org/wiki/List_of_University_of_Michigan_alumni, https://en.wikipedia.org/wiki/List_of_Cornell_University_alumni, https://en.wikipedia.org/wiki/University_of_St._Thomas_(Minnesota), https://en.wikipedia.org/wiki/List_of_Queens_Colege_people
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 13 working-memory snapshot after harness update}
pool_size: 74
curated_size: 30 / 30
importance_counts: very_high=0, high=5, fair=14, low=11
curated_set:
  - https://en.wikipedia.org/wiki/American_Pie_(film) [high]
  - https://en.wikipedia.org/wiki/American_Pie_(film_series) [high]
  - https://en.wikipedia.org/wiki/Eugene_Levy [high]
  - https://en.wikipedia.org/wiki/List_of_American_Pie_characters [high]
  - https://en.wikipedia.org/wiki/Seann_William_Scott [high]
  - https://en.wikipedia.org/wiki/Ben_Carson [fair]
  - https://en.wikipedia.org/wiki/Bradley_Cooper [fair]
  - https://en.wikipedia.org/wiki/Chris_Owen_(actor) [fair]
  - https://en.wikipedia.org/wiki/Ellis_Paul [fair]
  - https://en.wikipedia.org/wiki/Jason_Biggs [fair]
  - https://en.wikipedia.org/wiki/John_Cho [fair]
  - https://en.wikipedia.org/wiki/Magic_Johnson [fair]
  - https://en.wikipedia.org/wiki/Princeton_University [fair]
  - https://en.wikipedia.org/wiki/Shannon_Elizabeth [fair]
  - https://en.wikipedia.org/wiki/Steven_Curtis_Chapman [fair]
  - https://en.wikipedia.org/wiki/Susan_Rice [fair]
  - https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas [fair]
  - https://en.wikipedia.org/wiki/Tim_Reid [fair]
  - https://en.wikipedia.org/wiki/Tucker_Carlson [fair]
  - https://en.wikipedia.org/wiki/Bradley_Whitford [low]
  - https://en.wikipedia.org/wiki/Dan_Petronijevic [low]
  - https://en.wikipedia.org/wiki/David_Sutherland [low]
  - https://en.wikipedia.org/wiki/Donald_Sutherland [low]
  - https://en.wikipedia.org/wiki/Eugene_Levy_(politician) [low]
  - https://en.wikipedia.org/wiki/Heath_Ledger [low]
  - https://en.wikipedia.org/wiki/John_Lithgow [low]
  - https://en.wikipedia.org/wiki/Jonathan_Franzen [low]
  - https://en.wikipedia.org/wiki/Joss_Whedon [low]
  - https://en.wikipedia.org/wiki/List_of_NYU_Tisch_School_of_the_Arts_people [low]
  - https://en.wikipedia.org/wiki/Wes_Craven [low]
\end{trajectorylisting}

\subsubsection*{Turn 14: \CaseTool{toolRead}{read\_document}}
\begin{trajectorylisting}{toolNeutral}{Turn 14 model reasoning}
Current angle: link between comedy actor and university via commencement. Still not seeing the commencement itself. Maybe the university is the actual speaker: the question asks, "Which university did the actor ... deliver a commencement address at in 2012?" So the link is the university where the actor spoke. We need actor-to-university links. A more direct search: "was commencement speaker" with name. Maybe do a person-centric search for Eugene Levy speeches. However my assumption that Eugene is the actor may be wrong; the actor with the most American Pie films (including spinoffs) as of 2020 is actually Eugene Levy (24?); Seann in 4. So Eugene is likely. Alternatively, if the question refers to the actor most films, that would be Eugene Levy. Need to find his 2012 commencement address. Maybe Wikipedia lists speeches in his bio. We can read his article fully.
\end{trajectorylisting}

\begin{trajectorylisting}{toolRead}{Turn 14 tool call(s)}
[
  {
    "tool": "read_document",
    "params": {
      "doc_id": "https://en.wikipedia.org/wiki/Eugene_Levy"
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolRead}{Turn 14 tool return 0}
RETURN 0.text:
# Document (2460 tokens)
# Eugene Levy

## Summary
Eugene Levy (born December 17, 1946) is a Canadian actor and comedian.  He often plays flustered and unconventional figures. He is best known for appearing in the sketch comedy series SCTV, which aired from 1976 until 1984, and the American Pie series of films.  He is a regular collaborator of actor-director Christopher Guest, appearing in and co-writing four of his films, commencing with Waiting for Guffman (1996). From 2015 to 2020, he starred as Johnny Rose in Schitt's Creek, a comedy series that he co-created with his son and co-star Dan Levy.
Levy won a Grammy Award for Best Song Written for Visual Media in 2004 for "A Mighty Wind" from the film of the same name that he co-wrote. He received the Governor General's Performing Arts Award, Canada's highest honour in the performing arts, in 2008. He was appointed to the Order of Canada in 2011. In 2019 and 2020, he was nominated for the Primetime Emmy Award for Outstanding Lead Actor in a Comedy Series, which he won in 2020.

## Full Text
Eugene Levy (born December 17, 1946) is a Canadian actor and comedian.  He often plays flustered and unconventional figures. He is best known for appearing in the sketch comedy series SCTV, which aired from 1976 until 1984, and the American Pie series of films.  He is a regular collaborator of actor-director Christopher Guest, appearing in and co-writing four of his films, commencing with Waiting for Guffman (1996). From 2015 to 2020, he starred as Johnny Rose in Schitt's Creek, a comedy series that he co-created with his son and co-star Dan Levy.
Levy won a Grammy Award for Best Song Written for Visual Media in 2004 for "A Mighty Wind" from the film of the same name that he co-wrote. He received the Governor General's Performing Arts Award, Canada's highest honour in the performing arts, in 2008. He was appointed to the Order of Canada in 2011. In 2019 and 2020, he was nominated for the Primetime Emmy Award for Outstanding Lead Actor in a Comedy Series, which he won in 2020.

Early life and education
Levy was born to a Jewish family in downtown Hamilton, Ontario. His mother, Rebecca (nee Kudlatz; 1910-1988), was a homemaker, and his father, Joseph (1909-1985),  was a foreman at a car factory. He has a brother, Fred, and sister, Barbara. His mother was born in the Gorbals area of Glasgow, Scotland, to Polish Jewish parents, and later moved to Canada. His father was Sephardi Jewish, with ancestors from Spain and Bulgaria.
Levy attended Westdale Secondary School, where he was student council president. He faced antisemitic bullying, with his campaign posters defaced with the word "Jew", which he refused to take down. He subsequently attended McMaster University, graduating in 1969 with a Bachelor of Arts in sociology. He was vice-president of the McMaster Film Board, a student film group, where he met filmmaker Ivan Reitman.

Career
1972-1989: Godspell and SCTV
The 1972-1973 Toronto production of the hit musical Godspell opened at the Royal Alexandra Theatre and was intended to be a run of a few dozen performances for a subscription audience. The cast was drawn entirely from local performers, instead of a touring cast. The Toronto production launched the careers of many actors, including Levy, Victor Garber, Andrea Martin, Gilda Radner, Dave Thomas, and Martin Short, as well as the show's musical director, Paul Shaffer. Howard Shore played saxophone for this production. After an enthusiastic response from the audience, the scheduled run at the Royal Alexandra ended, and the show moved uptown to the Bayview Playhouse in Leaside. The Bayview Playhouse production ran until August 1973, with a then-record run of 488 performances.
An alumnus of both the Second City, Toronto and the sketch comedy series Second City Television, Levy often plays unusual supporting characters with nerdy streaks. Perhaps his best-known role on SCTV is the dimwitted Earl Camembert, a news anchor for the "SCTV News" and a parody of real-life Canadian newsman Earl Cameron. Celebrities impersonated by Levy on SCTV include Perry Como, Ricardo Montalban, Alex Trebek, Gino Vannelli, Sean Connery, Howard Cosell, Henry Kissinger, Menachem Begin, Bud Abbott, Milton Berle, John Charles Daly, Gene Shalit, Judd Hirsch, Jack Carter, Muammar al-Gaddafi, Tony Dow, James Caan, Lorne Greene, Rex Reed, Ralph Young (of Sandler and Young), F. Lee Bailey, Ernest Borgnine, former Ontario chief coroner and talk show host Dr. Morton Shulman, Norman Mailer, Neil Sedaka and Howard McNear as Floyd the Barber.
Original Levy characterizations on SCTV are news reporter Earl Camembert, comic Bobby Bittman, scandal sheet entrepreneur Dr. Raoul Withers, "report on business" naif Brian Johns, 3-D horror auteur Woody Tobias Jr., cheerful Leutonian accordionist Stan Schmenge, lecherous dream interpreter Raoul Wilson, hammer-voiced sports broadcaster Lou Jaffe, diminutive union patriarch Sid Dithers ("San Francisckie! Did you drove or did you flew?"), fey current-events commentator Joel Weiss, buttoned-down panel show moderator Dougal Currie, smarmy Just for Fun emcee Stan Kanter, energetic used car salesman Al Peck, guileless security guard Gus Gustofferson, Phil the Garment King (also of Phil's Nails), and the inept teen dance show host Rockin' Mel Slirrup.

1990-2014: American Pie and other comedy films
Though he has been the "above the title" star in only two films, Armed and Dangerous (1986) and The Man (2005), he has featured prominently in many films. He is the co-writer and frequent cast member of Christopher Guest's mockumentary features, particularly A Mighty Wind (2003), where his sympathetic performance as emotionally unstable folksinger Mitch Cohen won kudos; his accolades included a Satellite Award for Best Supporting Actor - Musical or Comedy and the prestigious New York Film Critics Circle Award for Best Supporting Actor. Other collaborations with Guest include Waiting for Guffman (1996), Best in Show (2000), and For Your Consideration (2006).
From the 1980s through the 2010s, Levy appeared in National Lampoon's Vacation (1983), Splash (1984), Club Paradise (1986), Father of the Bride (1991), Father of the Bride Part II (1995), Stay Tuned (1996), Multiplicity (1996), the American Pie film series (1999-2012), Serendipity (2001), Bringing Down the House (2003), Cheaper by the Dozen 2 (2005), Madea's Witness Protection (2012), and other comedies. He also voiced characters in films such as Over the Hedge (2006), Night at the Museum: Battle of the Smithsonian (2009), and Finding Dory (2016). Levy was the creator of Maniac Mansion, a television sitcom based on the LucasArts video game of the same name. He was also seriously considered for the role of Toby Ziegler on The West Wing, a role that went to actor Richard Schiff.

2015-present: Schitt's Creek and acclaim
Levy, along with his son Dan Levy, was co-creator of the CBC/Pop TV sitcom Schitt's Creek which ran from 2015-2020. He also starred in the show alongside his son as head of the Rose family, Johnny Rose. His daughter, Sarah Levy, portrayed Twyla Sands, the waitress at the Schitt's Creek diner. Eugene Levy's brother Fred was also a producer on the show.
Levy hosted and executive produced an Apple Original travel series titled The Reluctant Traveler (2023) on Apple TV+, which is now in its third season.
In 2024, Levy attended a ceremony honouring him with a star on the Hollywood Walk of Fame.

Personal life
Levy married Deborah Divine in 1977. Divine's career has been in TV production. The couple have two children whom they raised in Toronto: actors Dan and Sarah, both of whom starred alongside their father on Schitt's Creek.
Levy is an advocate for autism awareness and treatment, and supports ABA methods. He was a close friend of actor and fellow SCTV cast member John Candy. Levy is a member of the Canadian charity Artists Against Racism.
In 2021, he was named honorary mayor of Pacific Palisades. In October 2022, Levy was one of the honorees of Creative Community For Peace's 10th annual gala, and also spoke at the event. 
In 2025, his home in the neighbourhood was destroyed in the Palisades wildfire.

Filmography
Film
Television
Theatre
Audio
Awards and nominations
Levy, along with Christopher Guest and Michael McKean, was awarded the 2003 Grammy Award for Best Song Written for a Motion Picture, Television or Other Visual Media for the title song from A Mighty Wind. Levy received the Governor General's Performing Arts Award, Canada's highest honour in the performing arts, in 2008.
In March 2006, it was announced that he would receive a star on Canada's Walk of Fame. In 2002, the entire cast of SCTV was given a group star, and although Levy is not mentioned on the actual star, he was still inducted as a part of the group. This makes him one of only four two-time honourees, alongside fellow SCTV alumni John Candy, Martin Short, and Catherine O'Hara. Levy is one of only a handful of people who have won at least five Canadian Comedy Awards, including two for Best Writing (Best in Show in 2001 and A Mighty Wind in 2004) and three for Best Male Performer (Best in Show, American Pie 2 in 2002, and A Mighty Wind).
In 2008, the governor general of Canada presented Levy with the Governor General's Performing Arts Awards (GGPAA), a lifetime achievement award considered "for their outstanding body of work and enduring contribution to the performing arts in Canada.". In 2010, Levy was awarded the ACTRA Award by the union representing Canada's actors. In 2011, Levy was made a Member of the Order of Canada "for his contributions as a comic actor and writer, and for his dedication to charitable causes" and promoted to the rank of Companion in 2022.
On May 22, 2012, Levy delivered a commencement address at Dalhousie University, in Halifax, Nova Scotia, and was awarded the degree Doctor of Laws (honoris causa). On June 11, 2012, Levy was presented with the Queen Elizabeth II Diamond Jubilee Medal by the lieutenant governor of Ontario.
On March 13, 2016, Levy took home the award for "Best Performance by an Actor in a Continuing Leading Comedic Role" at the 4th Annual Canadian Screen Awards, for his performance as Johnny Rose in the CBC/Pop TV sitcom Schitt's Creek.

References
External links

Eugene Levy at IMDb
Eugene Levy at the Internet Broadway Database
Eugene Levy discography at Discogs
Article at thecanadianencyclopedia.ca
Eugene Levy on X
[Context: 9839/30720]
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 14 working-memory snapshot after harness update}
pool_size: 74
curated_size: 30 / 30
importance_counts: very_high=0, high=5, fair=14, low=11
curated_set:
  - https://en.wikipedia.org/wiki/American_Pie_(film) [high]
  - https://en.wikipedia.org/wiki/American_Pie_(film_series) [high]
  - https://en.wikipedia.org/wiki/Eugene_Levy [high]
  - https://en.wikipedia.org/wiki/List_of_American_Pie_characters [high]
  - https://en.wikipedia.org/wiki/Seann_William_Scott [high]
  - https://en.wikipedia.org/wiki/Ben_Carson [fair]
  - https://en.wikipedia.org/wiki/Bradley_Cooper [fair]
  - https://en.wikipedia.org/wiki/Chris_Owen_(actor) [fair]
  - https://en.wikipedia.org/wiki/Ellis_Paul [fair]
  - https://en.wikipedia.org/wiki/Jason_Biggs [fair]
  - https://en.wikipedia.org/wiki/John_Cho [fair]
  - https://en.wikipedia.org/wiki/Magic_Johnson [fair]
  - https://en.wikipedia.org/wiki/Princeton_University [fair]
  - https://en.wikipedia.org/wiki/Shannon_Elizabeth [fair]
  - https://en.wikipedia.org/wiki/Steven_Curtis_Chapman [fair]
  - https://en.wikipedia.org/wiki/Susan_Rice [fair]
  - https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas [fair]
  - https://en.wikipedia.org/wiki/Tim_Reid [fair]
  - https://en.wikipedia.org/wiki/Tucker_Carlson [fair]
  - https://en.wikipedia.org/wiki/Bradley_Whitford [low]
  - https://en.wikipedia.org/wiki/Dan_Petronijevic [low]
  - https://en.wikipedia.org/wiki/David_Sutherland [low]
  - https://en.wikipedia.org/wiki/Donald_Sutherland [low]
  - https://en.wikipedia.org/wiki/Eugene_Levy_(politician) [low]
  - https://en.wikipedia.org/wiki/Heath_Ledger [low]
  - https://en.wikipedia.org/wiki/John_Lithgow [low]
  - https://en.wikipedia.org/wiki/Jonathan_Franzen [low]
  - https://en.wikipedia.org/wiki/Joss_Whedon [low]
  - https://en.wikipedia.org/wiki/List_of_NYU_Tisch_School_of_the_Arts_people [low]
  - https://en.wikipedia.org/wiki/Wes_Craven [low]
\end{trajectorylisting}

\subsubsection*{Turn 15: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolNeutral}{Turn 15 model reasoning}
I read the full Eugene Levy article, and it explicitly contains the commencement address info: May 22, 2012, at Dalhousie University. That doc is clearly highly relevant. I must curate the doc now before any further search. I also might add the Dalhousie University page (the doc that got linked). The search result didn't include it, but I know from this doc that Dalhousie is relevant. I'll curate the current doc as very_high and add Dalhousie link as high.
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 15 tool call(s)}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [
        "https://en.wikipedia.org/wiki/Eugene_Levy",
        "https://en.wikipedia.org/wiki/Dalhousie_University"
      ],
      "importance": {
        "https://en.wikipedia.org/wiki/Eugene_Levy": "very_high",
        "https://en.wikipedia.org/wiki/Dalhousie_University": "high"
      }
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 15 tool return 0}
RETURN 0.text:
Curated set updated (30/30): https://en.wikipedia.org/wiki/Eugene_Levy[very_high], https://en.wikipedia.org/wiki/American_Pie_(film)[high], https://en.wikipedia.org/wiki/American_Pie_(film_series)[high], https://en.wikipedia.org/wiki/Dalhousie_University[high], https://en.wikipedia.org/wiki/List_of_American_Pie_characters[high], https://en.wikipedia.org/wiki/Seann_William_Scott[high], https://en.wikipedia.org/wiki/Ben_Carson[fair], https://en.wikipedia.org/wiki/Bradley_Cooper[fair], https://en.wikipedia.org/wiki/Chris_Owen_(actor)[fair], https://en.wikipedia.org/wiki/Ellis_Paul[fair], https://en.wikipedia.org/wiki/Jason_Biggs[fair], https://en.wikipedia.org/wiki/John_Cho[fair], https://en.wikipedia.org/wiki/Magic_Johnson[fair], https://en.wikipedia.org/wiki/Princeton_University[fair], https://en.wikipedia.org/wiki/Shannon_Elizabeth[fair], https://en.wikipedia.org/wiki/Steven_Curtis_Chapman[fair], https://en.wikipedia.org/wiki/Susan_Rice[fair], https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas[fair], https://en.wikipedia.org/wiki/Tim_Reid[fair], https://en.wikipedia.org/wiki/Tucker_Carlson[fair], https://en.wikipedia.org/wiki/Bradley_Whitford[low], https://en.wikipedia.org/wiki/Dan_Petronijevic[low], https://en.wikipedia.org/wiki/David_Sutherland[low], https://en.wikipedia.org/wiki/Donald_Sutherland[low], https://en.wikipedia.org/wiki/Heath_Ledger[low], https://en.wikipedia.org/wiki/John_Lithgow[low], https://en.wikipedia.org/wiki/Jonathan_Franzen[low], https://en.wikipedia.org/wiki/Joss_Whedon[low], https://en.wikipedia.org/wiki/List_of_NYU_Tisch_School_of_the_Arts_people[low], https://en.wikipedia.org/wiki/Wes_Craven[low]
[EVICTED low-importance] 1 doc(s): https://en.wikipedia.org/wiki/Eugene_Levy_(politician)
\end{trajectorylisting}

\begin{trajectorylisting}{toolNeutral}{Turn 15 working-memory snapshot after harness update}
pool_size: 74
curated_size: 30 / 30
importance_counts: very_high=1, high=5, fair=14, low=10
curated_set:
  - https://en.wikipedia.org/wiki/Eugene_Levy [very_high]
  - https://en.wikipedia.org/wiki/American_Pie_(film) [high]
  - https://en.wikipedia.org/wiki/American_Pie_(film_series) [high]
  - https://en.wikipedia.org/wiki/Dalhousie_University [high]
  - https://en.wikipedia.org/wiki/List_of_American_Pie_characters [high]
  - https://en.wikipedia.org/wiki/Seann_William_Scott [high]
  - https://en.wikipedia.org/wiki/Ben_Carson [fair]
  - https://en.wikipedia.org/wiki/Bradley_Cooper [fair]
  - https://en.wikipedia.org/wiki/Chris_Owen_(actor) [fair]
  - https://en.wikipedia.org/wiki/Ellis_Paul [fair]
  - https://en.wikipedia.org/wiki/Jason_Biggs [fair]
  - https://en.wikipedia.org/wiki/John_Cho [fair]
  - https://en.wikipedia.org/wiki/Magic_Johnson [fair]
  - https://en.wikipedia.org/wiki/Princeton_University [fair]
  - https://en.wikipedia.org/wiki/Shannon_Elizabeth [fair]
  - https://en.wikipedia.org/wiki/Steven_Curtis_Chapman [fair]
  - https://en.wikipedia.org/wiki/Susan_Rice [fair]
  - https://en.wikipedia.org/wiki/Thomas_Ian_Nicholas [fair]
  - https://en.wikipedia.org/wiki/Tim_Reid [fair]
  - https://en.wikipedia.org/wiki/Tucker_Carlson [fair]
  - https://en.wikipedia.org/wiki/Bradley_Whitford [low]
  - https://en.wikipedia.org/wiki/Dan_Petronijevic [low]
  - https://en.wikipedia.org/wiki/David_Sutherland [low]
  - https://en.wikipedia.org/wiki/Donald_Sutherland [low]
  - https://en.wikipedia.org/wiki/Heath_Ledger [low]
  - https://en.wikipedia.org/wiki/John_Lithgow [low]
  - https://en.wikipedia.org/wiki/Jonathan_Franzen [low]
  - https://en.wikipedia.org/wiki/Joss_Whedon [low]
  - https://en.wikipedia.org/wiki/List_of_NYU_Tisch_School_of_the_Arts_people [low]
  - https://en.wikipedia.org/wiki/Wes_Craven [low]
\end{trajectorylisting}



==> case_study_hotpot_snl_long.tex <==
\subsection{Full Trajectory D: HotpotQA SNL/Martin Query (unabridged)}
\label{app:case-hotpot-snl-long}
\begin{promptbox}{hotpotqa\_subset query 5ab30336554299166977417c}
\textbf{Query.} Which American comedian starred in the original cast of Saturday Night Live and played Stan Winters in the sitcom Martin?\\[2pt]
\textbf{Gold answer.} Garrett Morris
\end{promptbox}
\begin{trajectorylisting}{toolNeutral}{Top-level trajectory fields}
{
  "query_id": "5ab30336554299166977417c",
  "query_text": "Which American comedian starred in the original cast of Saturday Night Live and played Stan Winters in the sitcom Martin?",
  "dataset": "hotpotqa_subset",
  "curated_ids": [
    "https://en.wikipedia.org/wiki/Garrett_Morris",
    "https://en.wikipedia.org/wiki/Second_City_Television",
    "https://en.wikipedia.org/wiki/Andrea_Martin",
    "https://en.wikipedia.org/wiki/Bobby_Moynihan",
    "https://en.wikipedia.org/wiki/Victoria_Jackson",
    "https://en.wikipedia.org/wiki/Will_Forte",
    "https://en.wikipedia.org/wiki/Don_Novello",
    "https://en.wikipedia.org/wiki/Richard_Lewis_(comedian)",
    "https://en.wikipedia.org/wiki/Saturday_Night_Live_15th_Anniversary_Special",
    "https://en.wikipedia.org/wiki/List_of_Saturday_Night_Live_cast_members",
    "https://en.wikipedia.org/wiki/Saturday_Night_Live_season_1",
    "https://en.wikipedia.org/wiki/Saturday_Night_Live_season_3",
    "https://en.wikipedia.org/wiki/Martin_(TV_series)",
    "https://en.wikipedia.org/wiki/Scott_William_Winters"
  ],
  "curated_importance": {
    "https://en.wikipedia.org/wiki/Garrett_Morris": "high",
    "https://en.wikipedia.org/wiki/Second_City_Television": "fair",
    "https://en.wikipedia.org/wiki/Andrea_Martin": "fair",
    "https://en.wikipedia.org/wiki/Bobby_Moynihan": "fair",
    "https://en.wikipedia.org/wiki/Victoria_Jackson": "fair",
    "https://en.wikipedia.org/wiki/Will_Forte": "fair",
    "https://en.wikipedia.org/wiki/Don_Novello": "fair",
    "https://en.wikipedia.org/wiki/Richard_Lewis_(comedian)": "fair",
    "https://en.wikipedia.org/wiki/Saturday_Night_Live_15th_Anniversary_Special": "high",
    "https://en.wikipedia.org/wiki/List_of_Saturday_Night_Live_cast_members": "high",
    "https://en.wikipedia.org/wiki/Saturday_Night_Live_season_1": "fair",
    "https://en.wikipedia.org/wiki/Saturday_Night_Live_season_3": "fair",
    "https://en.wikipedia.org/wiki/Martin_(TV_series)": "fair",
    "https://en.wikipedia.org/wiki/Scott_William_Winters": "low"
  },
  "evidence_graph": {
    "entity_to_docs": {},
    "doc_to_entities": {}
  },
  "reward": 2.8181818181818183,
  "metrics": {
    "recall": 1.0,
    "precision": 0.14285714285714285,
    "f_beta": 0.4545454545454545,
    "final_answer_recall": 1.0,
    "final_answer_found": 1.0,
    "trajectory_recall": 1.0,
    "trajectory_fa_recall": 1.0,
    "final_answer_bonus": 1.0,
    "fa_dense_reward": 1.2000000000000002,
    "fa_miss_gap": 0.0,
    "fa_miss_penalty": 0.0,
    "pool_curated_gap": 0.0,
    "gap_penalty": 0.0,
    "turn_penalty": 0.0,
    "pre_penalty_reward": 2.8181818181818183,
    "num_curated_docs": 14.0,
    "used_curate": 1.0,
    "total_curate_calls": 5.0,
    "curate_rate": 0.45454545454545453,
    "curate_rate_bonus": 0.0,
    "tool_diversity": 5.0,
    "tool_diversity_bonus": 0.0,
    "num_turns": 11,
    "final_reward": 2.8181818181818183,
    "no_error": 1.0,
    "max_turns_reached": 0.0
  }
}
\end{trajectorylisting}

\subsubsection*{Turn 0: \CaseTool{toolSearch}{search\_corpus}}
\begin{trajectorylisting}{toolNeutral}{Turn 0 reasoning}
Key constraints: American comedian; original cast of Saturday Night Live; played Stan Winters in Martin. Distinctive facts suggest a single person. Likely Donnell Rawlings or someone else from SNL; need the name and both roles. Searching for name associated with both SNL original cast and Martin Stan Winters should be unique.
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 0 tool call}
[
  {
    "tool": "search_corpus",
    "params": {
      "query": "Stan Winters Martin SNL original cast comedian"
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 0 tool returns}

# DOCUMENT ID: https://en.wikipedia.org/wiki/Garrett_Morris (46 tokens)
Garrett Morris - Wikipedia
He is also known for his role in the sitcom Martin as Stan Winters, from 1992 to 1995, until he suffered an injury. Also, he made two guest appearances on The ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Second_City_Television (44 tokens)
Second City Television - Wikipedia
The original SCTV cast consisted of John Candy, Joe Flaherty, Eugene Levy, Andrea Martin, Catherine O'Hara, Harold Ramis, and Dave Thomas. All also served ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Andrea_Martin (40 tokens)
Andrea Martin - Wikipedia
Andrea Louise Martin (born January 15, 1947) is an American and Canadian actress and comedian, best known for her work in the television series SCTV and ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Bobby_Moynihan (48 tokens)
Bobby Moynihan - Wikipedia
He was a cast member and writer for the NBC sketch comedy series Saturday Night Live from 2008 to 2017. Bobby Moynihan. Moynihan in 2007. Born ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Victoria_Jackson (44 tokens)
Victoria Jackson - Wikipedia
Victoria Jackson (born August 2, 1959) is an American actress and comedian. She was a cast member on the series Saturday Night Live from 1986 to 1992.

# DOCUMENT ID: https://en.wikipedia.org/wiki/Will_Forte (38 tokens)
Will Forte - Wikipedia
Orville Willis Forte IV is an American actor, comedian, writer, and producer. He was a cast member and writer on the NBC sketch comedy series Saturday Night ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Don_Novello (47 tokens)
Don Novello - Wikipedia
Novello appeared on NBC's Saturday Night Live as the character Father Guido Sarducci from 1978 to 1980 and 1985 to 1986. He appeared as Sarducci in television ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Richard_Lewis_(comedian) (53 tokens)
Richard Lewis (comedian) - Wikipedia
Richard Philip Lewis (June 29, 1947 - February 27, 2024) was an American stand-up comedian, actor, and writer. Lewis came to prominence in the 1980s and ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Robert_Klein (40 tokens)
Robert Klein - Wikipedia
Robert Klein (born February 8, 1942) is an American stand-up comedian, singer, and actor. He is known for his appearances on stage and screen.

# DOCUMENT ID: https://en.wikipedia.org/wiki/Sid_Caesar (42 tokens)
Sid Caesar - Wikipedia
Isaac Sidney Caesar (September 8, 1922 - February 12, 2014) was an American comic actor and comedian. With a career spanning 60 years,

[AUTO-POPULATED] Top 8 docs from this search have been added to your curated set at 'fair' importance. Use `curate` with `importance` to promote/demote and `remove_ids` to drop irrelevant ones.
[Context: 690/30720]
\end{trajectorylisting}

\subsubsection*{Turn 1: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolCurate}{Turn 1 tool call}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [
        "https://en.wikipedia.org/wiki/Garrett_Morris",
        "https://en.wikipedia.org/wiki/Second_City_Television",
        "https://en.wikipedia.org/wiki/Andrea_Martin",
        "https://en.wikipedia.org/wiki/Bobby_Moynihan",
        "https://en.wikipedia.org/wiki/Victoria_Jackson",
        "https://en.wikipedia.org/wiki/Will_Forte",
        "https://en.wikipedia.org/wiki/Don_Novello",
        "https://en.wikipedia.org/wiki/Richard_Lewis_(comedian)"
      ],
      "importance": {
        "https://en.wikipedia.org/wiki/Garrett_Morris": "high",
        "https://en.wikipedia.org/wiki/Victoria_Jackson": "fair",
        "https://en.wikipedia.org/wiki/Will_Forte": "fair"
      }
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 1 tool returns}
Curated set updated (8/30): https://en.wikipedia.org/wiki/Garrett_Morris[high], https://en.wikipedia.org/wiki/Andrea_Martin[fair], https://en.wikipedia.org/wiki/Bobby_Moynihan[fair], https://en.wikipedia.org/wiki/Don_Novello[fair], https://en.wikipedia.org/wiki/Richard_Lewis_(comedian)[fair], https://en.wikipedia.org/wiki/Second_City_Television[fair], https://en.wikipedia.org/wiki/Victoria_Jackson[fair], https://en.wikipedia.org/wiki/Will_Forte[fair]
\end{trajectorylisting}

\subsubsection*{Turn 2: \CaseTool{toolSearch}{search\_corpus}}
\begin{trajectorylisting}{toolNeutral}{Turn 2 reasoning}
Got the likely answer: Garrett Morris. Need docs that also connect him to original SNL cast, not just Martin. There's a gap: we know he played Stan Winters from Garrett Morris result, but need a doc tying him to original SNL cast. My current angle is mostly found just the Martin facet. The current search angle is exhausted for new info on Stan Winters because we already saw the key doc; let me rethink. Re-read query: American comedian, original Saturday Night Live cast member, played Stan Winters in Martin. The constraint not yet fully bridged is SNL original cast. I will search that facet separately by name and role reference.
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 2 tool call}
[
  {
    "tool": "search_corpus",
    "params": {
      "query": "Garrett Morris Saturday Night Live original cast"
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 2 tool returns}

# DOCUMENT ID: https://en.wikipedia.org/wiki/Saturday_Night_Live_15th_Anniversary_Special (46 tokens)
Saturday Night Live 15th Anniversary Special - Wikipedia
The special was SNL's first anniversary celebration; it featured original cast members Chevy Chase, Dan Aykroyd, Jane Curtin, Garrett Morris, and Laraine ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/List_of_Saturday_Night_Live_cast_members (54 tokens)
List of Saturday Night Live cast members - Wikipedia
Original cast (from left to right): Laraine Newman, John Belushi, Jane Curtin, Gilda Radner, Dan Aykroyd, Garrett Morris, and Chevy Chase. Contents. 1 List.

# DOCUMENT ID: https://en.wikipedia.org/wiki/Saturday_Night_Live_season_1 (56 tokens)
Saturday Night Live season 1 - Wikipedia
Starring. Dan Aykroyd * John Belushi * Chevy Chase * George Coe * Jane Curtin * Garrett Morris * Laraine Newman * Michael O'Donoghue * Gilda Radner ; No. of ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Saturday_Night_Live_season_3 (40 tokens)
Saturday Night Live season 3 - Wikipedia
Cast * Dan Aykroyd * John Belushi * Jane Curtin * Garrett Morris * Bill Murray * Laraine Newman * Gilda Radner.

# DOCUMENT ID: https://en.wikipedia.org/wiki/Saturday_Night_Live_season_4 (40 tokens)
Saturday Night Live season 4 - Wikipedia
Cast * Dan Aykroyd * John Belushi * Jane Curtin * Garrett Morris * Bill Murray * Laraine Newman * Gilda Radner.

# DOCUMENT ID: https://en.wikipedia.org/wiki/Saturday_Night_Live_season_2 (59 tokens)
Saturday Night Live season 2 - Wikipedia
Cast roster * Dan Aykroyd * John Belushi * Chevy Chase (final episode: October 30, 1976) * Jane Curtin * Garrett Morris * Bill Murray (first episode: January 15, 1977) ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Saturday_Night_Live_season_5 (52 tokens)
Saturday Night Live season 5 - Wikipedia
Cast * Jane Curtin * Garrett Morris * Bill Murray * Laraine Newman * Gilda Radner * Harry Shearer (first episode: October 20, 1979; upgraded to repertory status: ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/The_Last_Voyage_of_the_Starship_Enterprise (40 tokens)
The Last Voyage of the Starship Enterprise - Wikipedia
In ranking every single Saturday Night Live cast member by talent in 2015 ... Garrett Morris. They announce that the Star Trek series has been ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Jane_Curtin (36 tokens)
Jane Curtin - Wikipedia
is an American actress and comedian. First coming to prominence as an original cast member on the hit TV comedy series Saturday Night Live in 1975.
[Context: 4162/30720]
\end{trajectorylisting}

\subsubsection*{Turn 3: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolNeutral}{Turn 3 reasoning}
We have a new search result directly tying Garrett Morris to SNL and original cast. That matches the SNL facet. The gap is still bridging both sides, but first we must curate these new results per rhythm.
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 3 tool call}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [
        "https://en.wikipedia.org/wiki/Saturday_Night_Live_15th_Anniversary_Special",
        "https://en.wikipedia.org/wiki/List_of_Saturday_Night_Live_cast_members",
        "https://en.wikipedia.org/wiki/Saturday_Night_Live_season_1",
        "https://en.wikipedia.org/wiki/Saturday_Night_Live_season_3"
      ],
      "importance": {
        "https://en.wikipedia.org/wiki/Saturday_Night_Live_15th_Anniversary_Special": "high",
        "https://en.wikipedia.org/wiki/List_of_Saturday_Night_Live_cast_members": "high",
        "https://en.wikipedia.org/wiki/Saturday_Night_Live_season_1": "fair",
        "https://en.wikipedia.org/wiki/Saturday_Night_Live_season_3": "fair"
      }
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 3 tool returns}
Curated set updated (12/30): https://en.wikipedia.org/wiki/Garrett_Morris[high], https://en.wikipedia.org/wiki/List_of_Saturday_Night_Live_cast_members[high], https://en.wikipedia.org/wiki/Saturday_Night_Live_15th_Anniversary_Special[high], https://en.wikipedia.org/wiki/Andrea_Martin[fair], https://en.wikipedia.org/wiki/Bobby_Moynihan[fair], https://en.wikipedia.org/wiki/Don_Novello[fair], https://en.wikipedia.org/wiki/Richard_Lewis_(comedian)[fair], https://en.wikipedia.org/wiki/Saturday_Night_Live_season_1[fair], https://en.wikipedia.org/wiki/Saturday_Night_Live_season_3[fair], https://en.wikipedia.org/wiki/Second_City_Television[fair], https://en.wikipedia.org/wiki/Victoria_Jackson[fair], https://en.wikipedia.org/wiki/Will_Forte[fair]
\end{trajectorylisting}

\subsubsection*{Turn 4: \CaseTool{toolRead}{read\_document}}
\begin{trajectorylisting}{toolNeutral}{Turn 4 reasoning}
The current angle is working: we found Garrett Morris tied to original SNL cast via SNL-season docs. Remaining gap is need a document also tying him to playing Stan Winters in Martin, but Garrett Morris doc probably already has that. Grep could find the exact phrase in the corpus if needed for very_high verification. Probably just read the Garrett Morris doc fully to surface the Martin sentence and the SNL facet if present. That doc should satisfy both facets in one source.
\end{trajectorylisting}

\begin{trajectorylisting}{toolRead}{Turn 4 tool call}
[
  {
    "tool": "read_document",
    "params": {
      "doc_id": "https://en.wikipedia.org/wiki/Garrett_Morris"
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolRead}{Turn 4 tool returns}
# Document (2665 tokens)
# Garrett Morris

## Summary
Garrett Isaac Morris (born February 1, 1937) is an American actor, comedian and singer. He was part of the original cast and was the first Black cast member of the sketch comedy program Saturday Night Live, appearing from 1975 to 1980.
He also played Jimmy on The Jeffersons (1983-1984). Morris had one of the starring roles, as Junior "Uncle Junior" King, on the sitcom The Jamie Foxx Show, which aired from 1996 to 2001. Morris also had a regular role as Earl Washington on the CBS sitcom 2 Broke Girls, from 2011 to 2017.
He is also known for his role in the sitcom Martin as Stan Winters, from 1992 to 1995, until he suffered an injury. Also, he made two guest appearances on The Wayans Bros. in season one, episode one as himself and again on episode ten as the brothers' uncle Leon (1995). He played a concerned teacher in the film Cooley High (1975), Slide in Car Wash (1976), and Carl in The Census Taker (1984).
In 2024, Morris was honored with his own star on the Hollywood Walk of Fame.

## Full Text
Garrett Isaac Morris (born February 1, 1937) is an American actor, comedian and singer. He was part of the original cast and was the first Black cast member of the sketch comedy program Saturday Night Live, appearing from 1975 to 1980.
He also played Jimmy on The Jeffersons (1983-1984). Morris had one of the starring roles, as Junior "Uncle Junior" King, on the sitcom The Jamie Foxx Show, which aired from 1996 to 2001. Morris also had a regular role as Earl Washington on the CBS sitcom 2 Broke Girls, from 2011 to 2017.
He is also known for his role in the sitcom Martin as Stan Winters, from 1992 to 1995, until he suffered an injury. Also, he made two guest appearances on The Wayans Bros. in season one, episode one as himself and again on episode ten as the brothers' uncle Leon (1995). He played a concerned teacher in the film Cooley High (1975), Slide in Car Wash (1976), and Carl in The Census Taker (1984).
In 2024, Morris was honored with his own star on the Hollywood Walk of Fame.

Early life and education
Morris was born on February 1, 1937, in New Orleans, Louisiana, and grew up in the poverty-stricken Gert Town neighborhood.  A church-choir singer from his youth, he trained at the Juilliard School of Music and graduated from Dillard University in 1958. Early in his career, he performed with The Belafonte Folk Singers. In 1960, Morris recorded South African Freedom Songs (EPC-601) with Pete Seeger and Guy Carawan for Folkways Records.

Saturday Night Live
Morris had written a play that Lorne Michaels read and liked, which got Morris hired on as a writer for a program he was developing for Saturday night. Morris was asked about bringing in black actors to potentially serve as cast members, such as asking Bill Duke. Duke wasn't cast, but a suggestion by ones who were cast led Michaels to view a film that had Morris in it, Cooley High, which Morris later stated "played a hand" in getting him cast on Saturday Night Live, as produced by Michaels.
Periodically on SNL he sang classical music: once a Mozart aria "Dalla Sua Pace", Don Ottavio's aria from Don Giovanni when guest-host Walter Matthau designated him as a "musical guest...in place of the usual crap", and once a Schubert lied while the titles on the screen expressed his colleagues' purported displeasure at having to accommodate a misguided request by him. In February 1977, he sang Tchaikovsky's Nur wer die Sehnsucht kennt barefoot in colorful Caribbean dress while subtitles explained he had just returned from Jamaica where he had picked up a girl by claiming to be Harry Belafonte.
One of Morris' best known characters on SNL was the Dominican baseball player Chico Escuela. Chico spoke only limited and halting English, so the joke centered on his responding to almost any question with his catch phrase: "Baseball... been berra berra good... to me". Another recurring bit, used in the newscast segment Weekend Update, involved Morris being presented as "Headmaster of the New York School for the hard of hearing" and assisting the newscaster by shouting the main headlines, in a parody of the then-common practice of providing sign language interpretation in an inset on the screen as an aid to the deaf viewer.
According to the book Saturday Night: A Backstage History of Saturday Night Live, Morris was frequently unhappy during his tenure on SNL from 1975 to 1980, and expressed the opinion that he was usually typecast in stereotypical roles.  In 2024's Saturday Night, directed by Jason Reitman, which dramatically details SNL's opening night, Morris's restless unhappiness is portrayed by actor Lamorne Morris (no relation).
Black performers who have followed Morris on SNL have at times been publicly concerned with experiencing the same fate Morris did. Eddie Murphy, for example, told TV Guide in the early 1980s that SNL producer Jean Doumanian "had tried to Garrett Morris me".
Morris, then at 38, was the eldest of the original cast members when SNL debuted in 1975.  He is also the eldest surviving cast member.

Recurring characters
Chico Escuela, a Dominican baseball player for the New York Mets
Cliff, the streetwise friend to the Festrunk Brothers (Dan Aykroyd and Steve Martin)
Grant Robinson Jr., one of The Nerds
Hodo, one of Miles Cowperthwaite's cronies
Merkon, the leader of the Coneheads
Weekend Update's "News for the Hard of Hearing" translator, who simply repeated each line while shouting with his hands cupped around his mouth.

Career
Theater
He performed in a number of Broadway musicals, including Hallelujah, Baby! and Ain't Supposed to Die a Natural Death. In 1965, he worked alongside Amiri Baraka, Sun Ra, Albert Ayler and Sonia Sanchez at the Black Arts Repertory Theatre/School in Harlem; during this period, the theater was frequently raided and surveilled by the New York City Police Department and the Federal Bureau of Investigation.

Television
In 1971, he had a small role as a police sergeant in The Anderson Tapes and was a cast member in the short-lived CBS sitcom, Roll Out. He also appeared as a high school teacher in the 1975 film Cooley High. In 1976, Morris appeared in the film Car Wash, playing the role of Slide the bookmaker. In 1983 and 1984, Morris appeared in five episodes of The Jeffersons, playing a character named Jimmy. He starred in the 1984 film The Census Taker, a 1984 black comedy directed by Bruce R. Cook.
In 1985, he guested on Murder, She Wrote as Lafayette Duquesne. In 1986, Morris began playing Arnold "Sporty" James, on the NBC cop drama Hunter, starring Fred Dryer and Stepfanie Kramer through 1989. Morris appeared in Married... with Children as Russ, one of Al's poker buddies, in "The Poker Game", in a 1987 season 1 episode and again in the season 3 episode "Requiem for a Dead Barber". He also appeared in the 1992 horror comedy Severed Ties starring Oliver Reed.
Morris also had regular roles on Diff'rent Strokes, The Jeffersons, Hill Street Blues, 227, and Roc. He also appeared in an episode of Who's the Boss, "Sam's Car" (1989), playing the role of Officer Audette. He was a regular cast member on The Jamie Foxx Show, playing Jamie's uncle, Junior King.
In 1998, Morris appeared as himself in the fourth episode of the fifth season of the TV series, Space Ghost Coast to Coast. In 2002, Morris made a cameo appearance on an episode of Saturday Night Live hosted by Brittany Murphy. In 2006, Morris reprised his role as "Headmaster of the New York School for the Hard of Hearing" in a cameo on the TV series Family Guy, in the episode "Barely Legal."
In August 2008, Morris played the role of Reverend Pratt in the family comedy drama film, The Longshots, starring Ice Cube and Keke Palmer.
In 2011, Morris had a cameo role as a Catholic priest on the episode "Three Boys" on the Showtime series Shameless. He was cast as Earl in the CBS comedy 2 Broke Girls, which premiered on September 19, 2011. During the second season he faced a lawsuit from the Global Agency accusing him of not paying 10% of his income from the show as agreed. However, a rep from the show stated that he had not actually failed to do so.
In 2018, Morris appeared in the NBC show This Is Us. In 2019, Morris appeared in the fifth episode of A Black Lady Sketch Show, titled "Why Are Her Pies Wet, Lord?"

Mugging
In 1994, he was shot by a would-be robber (whom he attempted to fight off) but recovered as he discussed on the January 14, 2016, episode of Marc Maron's podcast WTF. On Howard Stern's radio show on July 20, 1995, Morris said the culprit was imprisoned not for the shooting, but for parole violations for other crimes. In another radio interview, he mentioned that the robber who shot him was eventually convicted and incarcerated. In prison, inmates who happened to be fans of Morris teamed up and beat up the robber in revenge.
At the time of the shooting, Morris was starring on Martin as Martin's first boss, Stan Winters. Morris' shooting rendered him temporarily unable to continue in the role; he was written out of the show by having the character become a national fugitive. The scene where he is about to undergo plastic surgery was shot on the hospital bed Morris occupied while recuperating from the 1994 assault. He made a final appearance as Stan during the show's third season, walking with a cane due to Morris' real injuries, but the reason given for Stan was that he had crashed his car during a police chase.

Film
1980 Garrett appeared in "How to Beat the High Cost of Living" a comedy caper starting Susan Saint James, Jane Curtin, and Jessica Lange. Garrett played the Power and Light Man. In 1985, he appeared in Larry Cohen's science fiction horror film The Stuff, playing cookie magnate Chocolate Chip Charlie, a parody of Famous Amos. In 2015, Morris appeared as a cameo in Ant-Man, referencing an old SNL sketch in which he played the first live-action incarnation of the character.

Commercials
In 2009, Morris appeared in two TV commercials for the Nintendo DS-one featuring Mario Kart DS, and the other featuring Brain Age: Train Your Brain in Minutes a Day!. In 2010, Morris appeared in a television commercial for Miller Lite. The national commercial, titled "PopPop", features Morris alongside actors Stacey Dash and Jason Weaver. The commercial takes a light-hearted look at a family relationship with Morris playing the grandfather, PopPop, and Weaver as his grandson. Since summer 2010, Morris has appeared in an ad for Orbit gum in the United States.
He also operated and was the host of his own comedy club, The Downtown Comedy Club, in downtown Los Angeles. On February 9, 2007, Los Angeles mayor Antonio Villaraigosa honored Garrett Morris for his work and contributions to the black community. He declared February 9, 2007, Garrett Morris Day and named The Downtown Comedy Club the official club of Los Angeles.

Other career endeavors
On September 9, 2016, Morris and his family appeared on the ABC's game show Celebrity Family Feud, playing against Alfonso Ribeiro and Ribeiro's friends.
In 2024, Morris was honored with his own star on the Hollywood Walk of Fame.

Filmography
Film
Television
References
External links
Garrett Morris at IMDb
Garrett Morris at the Internet Broadway Database 
Garrett Morris at the Internet Off-Broadway Database (archived)
Garrett Morris at The Interviews: An Oral History of Television
Video: Colfax roasting Garrett Morris on YouTube
Garrett Morris as Chico on Weekend Update
The Downtown Comedy Club
[Context: 7644/30720]
\end{trajectorylisting}

\subsubsection*{Turn 5: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolNeutral}{Turn 5 reasoning}
We just read the full Garrett Morris doc, not searched, so no new docs added by search. But the read had no new curated docs from the search; still, this is a resubmit to curate; according to rhythm, we need to curate after reading the last doc if we had just searched. Actually we didn't search; we read. The instruction only says after search, curate. This was read, not search. But still need to curate the doc if it's obviously relevant. Should we curate the Garrett Morris doc now? It's the strongest bridge doc. Yes, we should curate this doc as a very relevant source tying both facets in one.
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 5 tool call}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [
        "https://en.wikipedia.org/wiki/Garrett_Morris"
      ],
      "remove_ids": [],
      "importance": {
        "https://en.wikipedia.org/wiki/Garrett_Morris": "high"
      }
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 5 tool returns}
Curated set updated (12/30): https://en.wikipedia.org/wiki/Garrett_Morris[high], https://en.wikipedia.org/wiki/List_of_Saturday_Night_Live_cast_members[high], https://en.wikipedia.org/wiki/Saturday_Night_Live_15th_Anniversary_Special[high], https://en.wikipedia.org/wiki/Andrea_Martin[fair], https://en.wikipedia.org/wiki/Bobby_Moynihan[fair], https://en.wikipedia.org/wiki/Don_Novello[fair], https://en.wikipedia.org/wiki/Richard_Lewis_(comedian)[fair], https://en.wikipedia.org/wiki/Saturday_Night_Live_season_1[fair], https://en.wikipedia.org/wiki/Saturday_Night_Live_season_3[fair], https://en.wikipedia.org/wiki/Second_City_Television[fair], https://en.wikipedia.org/wiki/Victoria_Jackson[fair], https://en.wikipedia.org/wiki/Will_Forte[fair]
\end{trajectorylisting}

\subsubsection*{Turn 6: \CaseTool{toolGrep}{grep\_corpus}}
\begin{trajectorylisting}{toolNeutral}{Turn 6 reasoning}
We have the full evidence bridge doc and two facet docs; the gap is minimal. The current query is a simple identity question. We have direct docs: Garrett Morris wiki plus SNL-original-cast doc. What else can strengthen? Could verify in the query pipeline: we might verify with verify to confirm the doc directly satisfies the multi-constraint query. That's perhaps overkill but useful to tag very_high. Alternatively, search for another doc specifically saying he was SNL original cast AND Martin. But we already have the bridge doc. Still, grep_corpus could catch the exact phrase 'Stan Winters' Martin SNL; that would produce a different docs angle. Let's try grep with exact phrase 'Stan Winters' Martin SNL.
\end{trajectorylisting}

\begin{trajectorylisting}{toolGrep}{Turn 6 tool call}
[
  {
    "tool": "grep_corpus",
    "params": {
      "pattern": "Stan Winters"
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolGrep}{Turn 6 tool returns}

# DOCUMENT ID: https://en.wikipedia.org/wiki/Garrett_Morris (45 tokens)
Garrett Morris - Wikipedia
He is also known for his role in the sitcom Martin as Stan Winters, from 1992 to 1995, until he suffered an injury. Also, he made two guest appearances on ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Scott_William_Winters (46 tokens)
Scott William Winters - Wikipedia
Scott William Winters (born August 5, 1965) is an American actor. Winters is of Irish and Italian descent, [1] and grew up on Long Island and in Scottsdale, ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/Jonathan_Winters (43 tokens)
Jonathan Winters - Wikipedia
Jonathan Harshman Winters III (November 11, 1925 - April 11, 2013) was an American comedian, actor, author, television host, and artist.

# DOCUMENT ID: https://en.wikipedia.org/wiki/Martin_(TV_series) (55 tokens)
Martin (TV series) - Wikipedia
Garrett Morris as Stan Winters (seasons 1-2; guest season 3). Supporting characters. edit * Reginald Ballard as Bruh-Man (Brother Man) (seasons 2-4); Tracy ...

# DOCUMENT ID: https://en.wikipedia.org/wiki/It%27s_a_Mad,_Mad,_Mad,_Mad_World (45 tokens)
It's a Mad, Mad, Mad, Mad World - Wikipedia
The film, starring Spencer Tracy with an all-star cast composed largely of comedians, is about the madcap pursuit of a suitcase full of stolen cash by a ...
[Context: 8105/30720]
\end{trajectorylisting}

\subsubsection*{Turn 7: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolNeutral}{Turn 7 reasoning}
We just did a grep and got new docs directly linking Stan Winters in Martin and Arthur Winters. The relevant docs are the Garrett Morris document, the Martin series page, and maybe Scott Winters for name disambiguation, but the key is the Martin doc. Curate now.
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 7 tool call}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [
        "https://en.wikipedia.org/wiki/Martin_(TV_series)",
        "https://en.wikipedia.org/wiki/Scott_William_Winters"
      ],
      "importance": {
        "https://en.wikipedia.org/wiki/Martin_(TV_series)": "fair",
        "https://en.wikipedia.org/wiki/Scott_William_Winters": "low"
      }
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 7 tool returns}
Curated set updated (14/30): https://en.wikipedia.org/wiki/Garrett_Morris[high], https://en.wikipedia.org/wiki/List_of_Saturday_Night_Live_cast_members[high], https://en.wikipedia.org/wiki/Saturday_Night_Live_15th_Anniversary_Special[high], https://en.wikipedia.org/wiki/Andrea_Martin[fair], https://en.wikipedia.org/wiki/Bobby_Moynihan[fair], https://en.wikipedia.org/wiki/Don_Novello[fair], https://en.wikipedia.org/wiki/Martin_(TV_series)[fair], https://en.wikipedia.org/wiki/Richard_Lewis_(comedian)[fair], https://en.wikipedia.org/wiki/Saturday_Night_Live_season_1[fair], https://en.wikipedia.org/wiki/Saturday_Night_Live_season_3[fair], https://en.wikipedia.org/wiki/Second_City_Television[fair], https://en.wikipedia.org/wiki/Victoria_Jackson[fair], https://en.wikipedia.org/wiki/Will_Forte[fair], https://en.wikipedia.org/wiki/Scott_William_Winters[low]
\end{trajectorylisting}

\subsubsection*{Turn 8: \CaseTool{toolVerify}{verify}}
\begin{trajectorylisting}{toolNeutral}{Turn 8 reasoning}
We have a very direct linkage: Garrett Morris doc confirms he was in original SNL cast and played Stan Winters in Martin. We also have Martin series page linking him as Stan Winters. The identity answer is clearly Garrett Morris. Remaining gap is minimal; the next best step is verify immediate docs on the single multi-constraint query before tagging very_high or concluding.
\end{trajectorylisting}

\begin{trajectorylisting}{toolVerify}{Turn 8 tool call}
[
  {
    "tool": "verify",
    "params": {
      "doc_ids": [
        "https://en.wikipedia.org/wiki/Garrett_Morris",
        "https://en.wikipedia.org/wiki/Martin_(TV_series)"
      ],
      "claim": "This doc states that Garrett Morris was part of the original cast of Saturday Night Live and played Stan Winters in the sitcom Martin."
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolVerify}{Turn 8 tool returns}
verify: no matching docs found in memory.
\end{trajectorylisting}

\subsubsection*{Turn 9: \CaseTool{toolSearch}{search\_corpus}}
\begin{trajectorylisting}{toolNeutral}{Turn 9 reasoning}
My current search angle is exhausted. Let me rethink. The verify step was actually after read, not search; the last search was grep, which we already curated. The gap is not research angle, it's tag hierarchy: we verified claims via read, but verify didn't match because we didn't run a search for that exact query. Instead, we'll do a direct search on the exact relational facet 'Stan Winters Martin comedian born' to get a document specifically naming him in Martin context without SNL churn.
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 9 tool call}
[
  {
    "tool": "search_corpus",
    "params": {
      "query": "Stan WintersMartin comedian original SNL cast"
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 9 tool returns}
No new results found (all results already seen)
[Context: 7478/30720]
\end{trajectorylisting}

\subsubsection*{Turn 10: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolNeutral}{Turn 10 reasoning}
The last search returned no new results, so there are no new docs to curate. But technically we need to comply with the search->curate rhythm after the search. Curate zero additions to maintain rhythm.
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 10 tool call}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [],
      "remove_ids": [],
      "importance": {}
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 10 tool returns}
Curated set updated (14/30): https://en.wikipedia.org/wiki/Garrett_Morris[high], https://en.wikipedia.org/wiki/List_of_Saturday_Night_Live_cast_members[high], https://en.wikipedia.org/wiki/Saturday_Night_Live_15th_Anniversary_Special[high], https://en.wikipedia.org/wiki/Andrea_Martin[fair], https://en.wikipedia.org/wiki/Bobby_Moynihan[fair], https://en.wikipedia.org/wiki/Don_Novello[fair], https://en.wikipedia.org/wiki/Martin_(TV_series)[fair], https://en.wikipedia.org/wiki/Richard_Lewis_(comedian)[fair], https://en.wikipedia.org/wiki/Saturday_Night_Live_season_1[fair], https://en.wikipedia.org/wiki/Saturday_Night_Live_season_3[fair], https://en.wikipedia.org/wiki/Second_City_Television[fair], https://en.wikipedia.org/wiki/Victoria_Jackson[fair], https://en.wikipedia.org/wiki/Will_Forte[fair], https://en.wikipedia.org/wiki/Scott_William_Winters[low]
\end{trajectorylisting}



==> case_study_sec497_long.tex <==
\subsection{Full Trajectory C: SEC Query 497\_0 (unabridged)}
\label{app:case-sec497-long}
\begin{promptbox}{sec query 497\_0}
\textbf{Query.} There is a company where a senior financial executive with over two decades of consumer packaged goods experience joined as a senior vice president in the early spring of the mid-2020s. Around the early summer of the same year, a different long-serving financial executive concluded their tenure after announcing their decision to step down several months earlier. That same date marked when the spring hire assumed the top financial role, succeeding the retiring executive.
On what date did this leadership transition in the financial executive role become effective?\\[2pt]
\textbf{Gold answer.} July 3, 2025
\end{promptbox}
\begin{trajectorylisting}{toolNeutral}{Top-level trajectory fields}
{
  "query_id": "497_0",
  "query_text": "There is a company where a senior financial executive with over two decades of consumer packaged goods experience joined as a senior vice president in the early spring of the mid-2020s. Around the early summer of the same year, a different long-serving financial executive concluded their tenure after announcing their decision to step down several months earlier. That same date marked when the spring hire assumed the top financial role, succeeding the retiring executive.\nOn what date did this leadership transition in the financial executive role become effective?",
  "dataset": "sec",
  "curated_ids": [
    "0001104659-25-006698_0",
    "0001104659-25-053287_0",
    "0001673985-25-000053_24",
    "0001364954-25-000039_57",
    "0001530950-25-000260_18",
    "0001104659-25-121934_20",
    "0000909832-25-000101_19",
    "0001104659-25-121934_21",
    "0001104659-25-121934_42"
  ],
  "curated_importance": {
    "0001104659-25-006698_0": "high",
    "0001104659-25-053287_0": "high",
    "0001673985-25-000053_24": "fair",
    "0001364954-25-000039_57": "fair",
    "0001530950-25-000260_18": "low",
    "0001104659-25-121934_20": "high",
    "0000909832-25-000101_19": "fair",
    "0001104659-25-121934_21": "high",
    "0001104659-25-121934_42": "high"
  },
  "evidence_graph": {
    "entity_to_docs": {},
    "doc_to_entities": {}
  },
  "reward": 3.103448275862069,
  "metrics": {
    "recall": 1.0,
    "precision": 0.5555555555555556,
    "f_beta": 0.8620689655172413,
    "final_answer_recall": 1.0,
    "final_answer_found": 1.0,
    "trajectory_recall": 1.0,
    "trajectory_fa_recall": 1.0,
    "final_answer_bonus": 1.0,
    "fa_dense_reward": 1.2000000000000002,
    "fa_miss_gap": 0.0,
    "fa_miss_penalty": 0.0,
    "pool_curated_gap": 0.0,
    "gap_penalty": 0.0,
    "turn_penalty": 0.0,
    "pre_penalty_reward": 3.103448275862069,
    "num_curated_docs": 9.0,
    "used_curate": 1.0,
    "total_curate_calls": 5.0,
    "curate_rate": 0.5555555555555556,
    "curate_rate_bonus": 0.0,
    "tool_diversity": 5.0,
    "tool_diversity_bonus": 0.0,
    "num_turns": 9,
    "final_reward": 3.103448275862069,
    "no_error": 1.0,
    "max_turns_reached": 0.0
  }
}
\end{trajectorylisting}

\subsubsection*{Turn 0: \CaseTool{toolSearch}{search\_corpus}}
\begin{trajectorylisting}{toolNeutral}{Turn 0 reasoning}
Key constraints: company where new senior vice president starts in early spring of mid-2020s, likely joined CFO role with over 20 years in consumer packaged goods. In early summer that same year, a long-serving financial executive stepped down after announcing decision months earlier, and that same date was effective for the transition. Likely pattern: a major CPG company CEO-chosen CFO supplants retiring CFO. Distinctive facet: 20+ years CPG experience for hire, senior vice president, effective date overlapping retirement announcement. The date likely publicized in a corporate press release about effective CFO transition. My first search angle is evaporating around generic CFO transition language; what's not working is broad CFO transitions; need more specific facet: early spring hire as SVP, 20+ years CPG, mid-2020s, effective date in early summer.
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 0 tool call}
[
  {
    "tool": "search_corpus",
    "params": {
      "query": "spring 2024 senior vice president food consumer packaged goods 20 years CPG effective CFO transition summer 2024 retire step down senior financial executive announced decision months earlier"
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolSearch}{Turn 0 tool returns}

# DOCUMENT ID: 0001104659-25-006698_0 (387 tokens) 
Company: Simply Good Foods Co
Filing Date: 2025-01-28
Form: 8-K
Item: Item 5.02
Chunk 0
---
Item 5.02 Departure of Directors or Certain Officers; Election of
Directors; Appointment of Certain Officers; Compensatory Arrangements of Certain Officers.

(b) On January 27, 2025, Shaun P. Mara, Chief Financial Officer
of The Simply Good Foods Company (the " Company"), notified the Company of his decision to retire effective July 3, 2025.
Mr. Mara will remain as Chief Financial Officer through the date of his retirement, at which time he will resign from all positions
with the Company and its subsidiaries.

In connection with Mr. Mara's retirement, on January 28,
2025, the Company announced the hiring of Mr. Christopher J. Bealer as Senior Vice President of Finance of the Company, as of
April 1, 2025. Mr. Bealer is expected to succeed Mr. Mara as Chief Financial Officer upon Mr. Mara's retirement
on July 3, 2025.

Mr. Bealer has almost 23 years of experience in consumer packaged
goods and consumer durables in North America and global markets. In his most recent executive leadership position as EVP Corporate Controller
at Reckitt Benckiser Group PLC (" Reckitt"), Mr. Bealer leads a global team of over 600 employees accountable for global
controls, financial shared services, group reporting and accounting, as well as leading the functional operating model transformation.
Prior to his current and prior roles at Reckitt, Mr. Bealer served as Regional CFO for Whirlpool Corporation for both the North American
and Europe, Middle East and Africa (EMEA) businesses. He also held finance positions at Big Heart Pet Brands, Del Monte Foods, and H. J.
Heinz Company.

# DOCUMENT ID: 0001104659-25-053287_0 (537 tokens) 
Company: Simply Good Foods Co
Filing Date: 2025-05-28
Form: 8-K
Item: Item 5.02
Chunk 0
---
Item 5.02

Departure of Directors or Certain Officers; Election of Directors; Appointment of Certain Officers; Compensatory Arrangements of Certain Officers.

Appointment of New CFO

In connection with the previously announced Chief Financial Officer
transition, on May 23, 2025, The Simply Good Foods Company (the " Company") appointed Christopher J. Bealer as the Company's
Chief Financial Officer effective July 3, 2025. Mr. Bealer is currently serving as the Company's Senior Vice President,
Finance having joined the Company on April 1, 2025. As Chief Financial Officer, Mr. Bealer will continue to report to Geoff
E. Tanner, the Company's President and Chief Executive Officer.

Mr. Bealer, age 48, has almost 23 years of experience in consumer-packaged
goods and consumer durables in North America and Global markets. Mr. Bealer was most recently EVP Corporate Controller at Reckitt
Benckiser Group PLC (" Reckitt") from March 2024 to March 31, 2025, and CFO Health at Reckitt from April 2021
to February 2024. In his EVP Corporate Controller role with Reckitt, Mr. Bealer led a global team of over 600 employees accountable
for global controls, financial shared services, group reporting and accounting, as well as leading the functional operating model transformation.
Prior to his roles at Reckitt, Mr. Bealer served as Vice President and CFO Europe, Middle East and Africa Region from August 2018
to March 2021 and Vice President and CFO North America Region from November 2015 to August 2018 for Whirlpool Corporation.
Earlier in his career, Bealer held various finance roles at Big Heart Pet Brands, Del Monte Foods, and H. J. Heinz Company. Mr. Bealer
is a Certified Public Accountant in the United States and a qualified Associate Chartered Accountant in the United Kingdom. Mr. Bealer
received his Bachelor's Degree with Honours - Geography from the University of Birmingham, U. K.

As Chief Financial Officer, Mr. Bealer will receive an initial
annual base salary of $500,000 (" Base Salary"), subject to future adjustment by the Company. Mr. Bealer will be eligible
to participate in the Company's long term equity incentive program, with an annual target opportunity of one hundred fifty percent
(150%) of his Base Salary.

In addition, Mr.

# DOCUMENT ID: 0001673985-25-000053_24 (539 tokens) 
Company: AdvanSix Inc.
Filing Date: 2025-04-29
Form: DEF 14A
Chunk 24
---
                                                                                                                                                                                                                                                                                                                                                                                                                              
 Stockholders, as well as other interested parties, may communicate directly with the Board Chair, the non-employee directors as a group, or individual directors by writing to: AdvanSix Inc., c/o Corporate Secretary, 300 Kimball Drive, Suite 101, Parsippany, New Jersey 07054.                                                                                                                                                                                                                                                                                                                       
 AdvanSix's Corporate Secretary reviews and promptly forwards communications to the directors as appropriate. Communications involving substantive accounting or auditing matters are forwarded to the Chair of the Audit Committee. Certain items that are unrelated to the duties and responsibilities of the Board will not be forwarded such as: business solicitation or advertisements; product or service-related inquiries; junk mail or mass mailings; resumes or other job-related inquiries; spam; and overly hostile, threatening, potentially illegal or similarly unsuitable communications. |

| 21 |     | Proxy and Notice of Annual Meeting of Stockholders |     | 2025 |

### EXECUTIVE COMPENSATION

### COMPENSATION DISCUSSION AND ANALYSIS
In this Compensation Discussion and Analysis ("CD&A"), we discuss the compensation philosophy, programs and practices adopted by the C&LD Committee for senior executive officers and review the various objectives and elements of AdvanSix's executive compensation program, its alignment with performance and the 2024 compensation decisions regarding our Named Executive Officers ("NEOs"). Michael Preston retired as the Company's Senior Vice President and Chief Financial Officer, effective as of October 1, 2024, and remained at the Company through year-end 2024 to help facilitate the transition of his responsibilities to his successor. Effective as of October 1, 2024, the Board appointed Siddharth Manjeshwar as Senior Vice President and Chief Financial Officer to succeed Mr. Preston. Effective as of March 17, 2025, Christopher Gramm was appointed to serve as Vice President, Financial Planning and Analysis of the Company. In connection with his new role, Mr. Gramm will step down from his current role as the Company's Vice President, Controller and will no longer serve as an executive officer of the Company.

For purposes of this CD&A and the disclosure that follows, the following are AdvanSix's NEOs for 2024:

| Erin N. Kane            |     | President and Chief Executive Officer (CEO)                    |
| Siddharth Manjeshwar    |     | Senior Vice President and Chief Financial Officer (CFO)        |
| Michael Preston         |     | Former Senior Vice President and Chief

# DOCUMENT ID: 0001364954-25-000039_57 (536 tokens) 
Company: CHEGG, INC
Filing Date: 2025-04-17
Form: DEF 14A
Chunk 57
---
 of June 1, 2024, Dan Rosensweig resigned from his positions as President and CEO and was appointed as our Executive Chair. Mr. Rosensweig is continuing to serve as a Co-Chairperson of the Board. In connection with his appointment as Executive Chair, Mr. Rosensweig received (i) a base salary of $850,000, (ii) RSUs with an approximate grant date value of $1,077,188, and (iii) PSUs with an approximate grant value of $359,063, which will only vest upon achievement of specified goals. The RSUs vest over three years, with 50% vesting on the first anniversary of the vesting commencement date and the remainder vesting in eight equal quarterly installments for 24 months thereafter, subject to Mr. Rosensweig's continued service on the applicable vesting dates. The PSUs are allocated to a single tranche, become earned and eligible to vest upon the achievement of certain performance goals, as determined by the Compensation Committee, and are subject to a total three-year time-based vesting period (to the extent earned), subject to Mr. Rosensweig's continued service on the applicable vesting dates.

David Longo Transition - New Chief Financial Officer Upon Andrew Brown's Retirement

Effective February 21, 2024, David Longo was appointed as our Chief Financial Officer, Principal Financial Officer, Principal Accounting Officer, and Treasurer. Mr. Longo replaced Andrew Brown, who resigned effective February 21, 2024 and, as part of a planned transition, remained an employee of the Company until his retirement on June 7, 2024. Prior to his appointment as Chief Financial Officer, Mr. Longo served as the Company's Vice President, Chief Accounting Officer, Corporate Controller, Assistant Treasurer, and Principal Accounting Officer since December 2021. In connection with his new appointment, Mr. Longo received (i) a base salary of $680,000 and (ii) RSUs with an approximate grant date value of $1,900,000 million. The RSUs vested in full in March 2025, with such vesting subject to Mr. Longo's continued service through the vesting date.

#### Esther Lem Retirement
Esther Lem resigned from her position as Chief Marketing Officer, effective April 5, 2024, after spending 13 years in the role. Ms. Lem remained an employee of the Company through July 5, 2024,

# DOCUMENT ID: 0001530950-25-000260_18 (537 tokens) 
Company: Post Holdings, Inc.
Filing Date: 2025-11-21
Form: 10-K
Item: Item 1A
Chunk 18
---
 and Chief Administrative Officer from November 2014 until November 2017. Ms. Gray served as our Senior Vice President-Legal starting in December 2011 and was promoted to Senior Vice President, General Counsel in September 2012. Prior to joining Post, Ms. Gray served as associate general counsel and assistant secretary at MEMC Electronic Materials, Inc. (now SunEdison, Inc.), which, at the time, was a semiconductor and solar wafer manufacturing company, from 2010 to 2011. Previously, Ms. Gray was an attorney at Bryan Cave LLP (now Bryan Cave Leighton Paisner LLP) from 2003 to 2010.

Mark W. Westphal, age 60, has served as President, Foodservice (formerly known as Michael Foods) since January 2018. Until January 2018, Mr. Westphal served as Chief Financial Officer of Michael Foods for nearly ten years. Prior to joining Michael Foods in 1995, Mr. Westphal worked for Grant Thornton LLP, an audit and assurance, tax and advisory services firm.

Jeff A. Zadoks, age 60, has served as an Executive Vice President since November 2017 and as our Chief Operating Officer since December 2022. As previously announced, Mr. Zadoks plans to retire from his current roles effective January 2026. Mr. Zadoks also served as our Interim President and Chief Executive Officer from November 2023 to January 2024, in connection with a medical leave of absence of Mr. Vitale. Mr. Zadoks previously served as our Executive Vice President and Chief Financial Officer from November 2017 until December 2022, and our Senior Vice President and Chief Financial Officer from November 2014 until November 2017. Mr. Zadoks served as our Senior Vice President and Chief Accounting Officer from January 2014 until November 2014, and as our Corporate Controller from October 2011 until November 2014. Mr. Zadoks also served as the chairman of the board of directors of PHPC, our former publicly-traded affiliate that was a special purpose acquisition company, from January 2021 until June 2023. Prior to joining Post, Mr. Zadoks served as senior vice president and chief accounting officer at RehabCare Group, Inc. ("RehabCare Group"), which, at the time, was a provider of post-acute care in hospitals and skilled nursing facilities, from February 2010

# DOCUMENT ID: 0001104659-25-121934_20 (536 tokens) 
Company: Simply Good Foods Co
Filing Date: 2025-12-17
Form: DEF 14A
Chunk 20
---
 consumer-packaged goods and consumer durables in North America and Global markets. Mr. Bealer was most recently EVP Corporate Controller at Reckitt Benckiser Group PLC ("Reckitt") from March 2024 to March 31, 2025, and CFO Health at Reckitt from April 2021 to February 2024. In his EVP Corporate Controller role with Reckitt, Mr. Bealer led a global team of over 600 employees accountable for global controls, financial shared services, group reporting and accounting, as well as leading the functional operating model transformation. 
                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       
 -                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      
 Prior to his roles at Reckitt, Mr. Bealer served as Vice President and CFO Europe, Middle East and Africa Region from August 2018 to March 2021 and Vice President and CFO North America Region from November 2015 to August 2018 for Whirlpool Corporation.                                                                                                                                                                                                                                                                                                                                           
                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       |  
  |  
  | Age:49                                                                                                                                 
 Chief Financial Officer                                                                                                                
 -                                                                                                                                      
 Earlier in his career, Bealer held various finance roles at Big Heart Pet Brands, Del Monte Foods, and H.J. Heinz Company.             
                                                                                                                                       
 -                                                                                                                                      
 Mr. Bealer is a Certified Public Accountant in the United States and a qualified Associate Chartered Accountant in the United Kingdom. 
                                                                                                                                       |  
  |
|:--|:-------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------|:--|:--|:---------------------------------------------------------------------------------------------------------------------------------------|:--|
|  | EDUCATION                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              
 -                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      
 Mr. Bealer received his Bachelor's Degree with Honours - Geography from the University of Birmingham, U.K.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             
                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       |   |   |                                                                                                                                        |  |

36 2026 Proxy Statement

TABLE OF CONTENTS

|  
  | Michael L. Clawson                                                                                                                                                                                                                                                                                                                                                                                     
 EXPERIENCE                                                                                                                                                                                                                                                                                                                                                                                             
 -                                                                                                                                                                                                                                                                                                                                                                                                      
 Michael L. Clawson has served as our Chief Commercial Officer since November 14, 2025. Prior to that, Mr. Clawson served as our Chief Customer Officer from October 14, 2024, when he joined the Company to November 14, 2025. Prior to that, Mr. Clawson was General Manager, Vice President, Meals Business Unit the largest

# DOCUMENT ID: 0000909832-25-000101_19 (548 tokens) 
Company: COSTCO WHOLESALE CORP /NEW
Filing Date: 2025-10-08
Form: 10-K
Item: Item 1
Chunk 19
---
 2024 and, prior to that, as Chief Executive Officer of Kroger Personal Finance since July 2010.202454Russ MillerSenior Executive Vice President, U.S. Operations. Mr. Miller was Executive Vice President, Chief Operating Officer, Southwest Division and Mexico, from January 2018 to May 2022. Mr. Miller was Senior Vice President, Western Canada Region, from 2001 to January 2018. Mr. Miller will be retiring from the Company effective February 2026.201868Claudine AdamoExecutive Vice President, Merchandising. Ms. Adamo was Senior Vice President, Non-Foods, from 2018 to February 2022, and Vice President, Non-Foods, from 2013 to 2018.202255Patrick CallansExecutive Vice President, Administration. Mr. Callans was Senior Vice President, Human Resources and Risk Management, from 2013 to December 2018.201963Caton FratesExecutive Vice President, Chief Operating Officer, Southwest Division. Mr. Frates was Senior Vice President, Los Angeles Region, from 2015 to May 2022. Mr. Frates will be appointed Senior Executive Vice President, Warehouse Operations - U.S. and Mexico, effective February 2026.202257Teresa JonesExecutive Vice President, Global Depots and Traffic. Ms. Jones was Senior Vice President, Depot Operations from August 2022 to July 2024, and Vice President, Depot Operations, from 2018 to 2022.202456Jim C. KlauerExecutive Vice President, Chief Operating Officer, Northern Division. Mr. Klauer was Senior Vice President, Non-Foods and E-commerce Merchandise, from 2013 to January 2018.201863Javier PolitExecutive Vice President, Chief Information and Digital Officer. Mr. Polit previously served as Chief Information Officer for Mondelez International (formerly Kraft Foods) from 2022 to 2024. From 2017 to 2022, he was Chief Information Officer for The Procter & Gamble Company. Prior to that role, he served as Group Chief Information Officer for The Coca-Cola Company from 2007 to 2017.202361Pierre RielExecutive Vice President, Chief Operating Officer, International Division. Mr. Riel was Senior Vice President, Country Manager, Canada, from 2019 to March 2022, and Senior Vice President, Eastern Canada Region, from 2001 to 2019.202262

[AUTO-POPULATED] Top 7 docs from this search have been added to your curated set at 'fair' importance. Use `curate` with `importance` to promote/demote and `remove_ids` to drop irrelevant ones.
[Context: 3823/30720]
\end{trajectorylisting}

\subsubsection*{Turn 1: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolCurate}{Turn 1 tool call}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [
        "0001104659-25-006698_0",
        "0001104659-25-053287_0",
        "0001530950-25-000260_18",
        "0001104659-25-121934_20"
      ],
      "importance": {
        "0001104659-25-006698_0": "high",
        "0001104659-25-053287_0": "high",
        "0001530950-25-000260_18": "low",
        "0001104659-25-121934_20": "high"
      }
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 1 tool returns}
Curated set updated (7/30): 0001104659-25-006698_0[high], 0001104659-25-053287_0[high], 0001104659-25-121934_20[high], 0000909832-25-000101_19[fair], 0001364954-25-000039_57[fair], 0001673985-25-000053_24[fair], 0001530950-25-000260_18[low]
\end{trajectorylisting}

\subsubsection*{Turn 2: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolNeutral}{Turn 2 reasoning}
Found a very promising candidate: Simply Good Foods Co. Docs 0001104659-25-006698_0 and 0001104659-25-053287_0 clearly match the described transition: Christopher J. Bealer hired as senior vice president of finance April 1, 2025, with CPG experience, effective as CFO on July 3, 2025; Michael Mara announced retirement effective that same date in early summer. Key missing piece is the exact effective date of the transition. docs already likely contain it, but need to verify the claim against the exact transition date. I'm curating now because Search->Curate is required after the search; then I can read docs directly to extract the transition effective date before verifying.
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 2 tool call}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [],
      "remove_ids": [],
      "importance": {}
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 2 tool returns}
Curated set updated (7/30): 0001104659-25-006698_0[high], 0001104659-25-053287_0[high], 0001104659-25-121934_20[high], 0000909832-25-000101_19[fair], 0001364954-25-000039_57[fair], 0001673985-25-000053_24[fair], 0001530950-25-000260_18[low]
\end{trajectorylisting}

\subsubsection*{Turn 3: \CaseTool{toolRead}{read\_document}}
\begin{trajectorylisting}{toolNeutral}{Turn 3 reasoning}
The current angle is likely exhausted: the first search already pointed strongly to Simply Good Foods and the concept is almost solved. What's not working is our need to get the exact official effective date, which likely already appears in those SEC filing documents. I'm choosing read_document on the most directly relevant file fragment linked to the transition announcement, instead of searching again, because reading should let me extract the precise date from the full context.
\end{trajectorylisting}

\begin{trajectorylisting}{toolRead}{Turn 3 tool call}
[
  {
    "tool": "read_document",
    "params": {
      "doc_id": "0001104659-25-053287_0"
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolRead}{Turn 3 tool returns}
# Document (1500 tokens)
Company: Simply Good Foods Co
Filing Date: 2025-05-28
Form: 8-K
Item: Item 5.02
Chunk 0
---
Item 5.02

Departure of Directors or Certain Officers; Election of Directors; Appointment of Certain Officers; Compensatory Arrangements of Certain Officers.

Appointment of New CFO

In connection with the previously announced Chief Financial Officer
transition, on May 23, 2025, The Simply Good Foods Company (the " Company") appointed Christopher J. Bealer as the Company's
Chief Financial Officer effective July 3, 2025. Mr. Bealer is currently serving as the Company's Senior Vice President,
Finance having joined the Company on April 1, 2025. As Chief Financial Officer, Mr. Bealer will continue to report to Geoff
E. Tanner, the Company's President and Chief Executive Officer.

Mr. Bealer, age 48, has almost 23 years of experience in consumer-packaged
goods and consumer durables in North America and Global markets. Mr. Bealer was most recently EVP Corporate Controller at Reckitt
Benckiser Group PLC (" Reckitt") from March 2024 to March 31, 2025, and CFO Health at Reckitt from April 2021
to February 2024. In his EVP Corporate Controller role with Reckitt, Mr. Bealer led a global team of over 600 employees accountable
for global controls, financial shared services, group reporting and accounting, as well as leading the functional operating model transformation.
Prior to his roles at Reckitt, Mr. Bealer served as Vice President and CFO Europe, Middle East and Africa Region from August 2018
to March 2021 and Vice President and CFO North America Region from November 2015 to August 2018 for Whirlpool Corporation.
Earlier in his career, Bealer held various finance roles at Big Heart Pet Brands, Del Monte Foods, and H. J. Heinz Company. Mr. Bealer
is a Certified Public Accountant in the United States and a qualified Associate Chartered Accountant in the United Kingdom. Mr. Bealer
received his Bachelor's Degree with Honours - Geography from the University of Birmingham, U. K.

As Chief Financial Officer, Mr. Bealer will receive an initial
annual base salary of $500,000 (" Base Salary"), subject to future adjustment by the Company. Mr. Bealer will be eligible
to participate in the Company's long term equity incentive program, with an annual target opportunity of one hundred fifty percent
(150%) of his Base Salary.

In addition, Mr.Company: Simply Good Foods Co
Filing Date: 2025-05-28
Form: 8-K
Item: Item 5.02
Chunk 1
---
 Bealer will be eligible to participate in the
Company's annual short term cash incentive program, as and if established by the Board (or a committee thereof), with an annual
target bonus opportunity of seventy five percent (75%) of his Base Salary, based on the achievement of pre-established performance goals
established by the Board (or a committee thereof). Mr. Bealer is also eligible to participate in the Company's executive severance
and other benefit programs available to Company employees and will be entitled to unlimited paid time off to be taken in accordance with
Company policy.

There are no arrangements or understandings between Mr. Bealer
and any other persons outside of the Company pursuant to which he was selected as an executive officer of the Company, and there are no
family relationships between any director, executive officer, or person nominated or chosen by the Company to become a director or executive
officer of the Company and Mr. Bealer. Mr. Bealer has no direct or indirect material interest in any transaction required to
be disclosed pursuant to Item 404(a) of Regulation S-K.

Amendment to the Executive Severance Plan

On May 23, 2025, the Company's Board of Directors (the " Board"),
based on a unanimous recommendation from the Board's Compensation Committee, amended and restated The Simply Good Foods Company
Second Amended and Restated Executive Severance Plan (as amended to date, the " Third Amended and Restated Plan"), effective
on the same date. The adoption of the Third Amended and Restated Plan resulted from the Board's Compensation Committee's regular
review of the various aspects of the Company's compensation program, was developed in consultation with the Compensation Committee's
independent compensation consultant and with the advice of counsel, and is intended to continue to promote the recruitment and retention
of key executives. Capitalized terms used in this description without definition have the meaning given those terms in the Third Amended
and Restated Plan.

The Third Amended and Restated Plan modifies the rate at which cash
severance is payable to the Company's President and Chief Executive Officer, Chief Financial Officer, Chief Legal Officer and Chief
Human Resources Officer only upon a Qualifying Termination in connection with a Change in Control. No other changes were made to the plan
as previously in effect.

Pursuant to the Third Amended and Restated Plan, upon a Qualifying
Termination in connection with a Change in Control, the amount of cash severance payable will beCompany: Simply Good Foods Co
Filing Date: 2025-05-28
Form: 8-K
Item: Item 5.02
Chunk 2
---
 determined by multiplying the following
for the Company's President and Chief Executive Officer by a rate of three (3) times and for each of the Company's Chief
Financial Officer, Chief Legal Officer and Chief Human Resources Officer by a rate of two (2) times:

  the individual's Base Salary, plus  

  Target Annual Bonus Amount, plus  

  an amount equal to the cost of COBRA coverage for a period of one year assuming                                               

These changes apply to the following current Named Executive
Officers: Messrs. Geoff E. Tanner (President and Chief Executive Officer), Shaun P. Mara (Chief Financial Officer), Timothy R.
Kraft (Chief Legal and Corporate Affairs Officer) and Ms. Amy C. Held (Senior Vice President and Chief Human Resources
Officer).

The foregoing summary is qualified in its entirety by reference to
the Plan as filed as Exhibit 10.1 to this Current Report on Form 8-K and incorporated herein by reference.

  Item 9.01      Financial Statements and Exhibits  

(d) Exhibits

  Exhibit No.      Description                                                                         
 
         10.1      The Simply Good Foods Company Third Amended and Restated Executive Severance Plan.  
          104      Cover Page Interactive Data File (embedded within the Inline XBRL document)         

SIGNATURE

Pursuant to the requirements
of the Securities Exchange Act of 1934, the registrant has duly caused this report to be signed on its behalf by the undersigned hereunto
duly authorized.

  Date:      May 28, 2025      By:         /s/ Shaun P. Mara              
 
                               Name:       Shaun P. Mara                  
                               Title:      Chief Financial Officer        
                                           (Principal Financial Officer)
[Context: 7680/30720]
\end{trajectorylisting}

\subsubsection*{Turn 4: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolNeutral}{Turn 4 reasoning}
We read a strongly relevant transition doc; the search angle is exhausted and the problem is now extracting the exact effective date from the current evidence. The document we just read explicitly gives the effective date as July 3, 2025, but we need to curate that doc immediately before changing strategy.
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 4 tool call}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [
        "0001104659-25-053287_0"
      ],
      "importance": {
        "0001104659-25-053287_0": "high"
      }
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 4 tool returns}
Curated set updated (7/30): 0001104659-25-006698_0[high], 0001104659-25-053287_0[high], 0001104659-25-121934_20[high], 0000909832-25-000101_19[fair], 0001364954-25-000039_57[fair], 0001673985-25-000053_24[fair], 0001530950-25-000260_18[low]
\end{trajectorylisting}

\subsubsection*{Turn 5: \CaseTool{toolVerify}{verify}}
\begin{trajectorylisting}{toolNeutral}{Turn 5 reasoning}
We have gathered the likely solution: Simple Good Foods transition, and we already read the SEC filing that explicitly says Christopher J. Bealer was appointed CFO effective July 3, 2025. With only one more result to search for, best to verify the exact claim via the verify tool rather than search again.
\end{trajectorylisting}

\begin{trajectorylisting}{toolVerify}{Turn 5 tool call}
[
  {
    "tool": "verify",
    "params": {
      "doc_ids": [
        "0001104659-25-053287_0"
      ],
      "claim": "This doc says Christopher J. Bealer was appointed CFO of Simply Good Foods effective July 3, 2025."
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolVerify}{Turn 5 tool returns}
verify: no matching docs found in memory.
\end{trajectorylisting}

\subsubsection*{Turn 6: \CaseTool{toolGrep}{grep\_corpus}}
\begin{trajectorylisting}{toolNeutral}{Turn 6 reasoning}
The last search was actually a verification step and not a corpus search, but a thin-angle grep/specific-date check is still a useful search angle before ending. The strong evidence is on hand, but I need one more corpus check for the exact effective date doc without changing context, then curate immediately. I'm choosing grep for an exact phrase likely repeated elsewhere: 'effective July 3, 2025' in a CFO transition document.
\end{trajectorylisting}

\begin{trajectorylisting}{toolGrep}{Turn 6 tool call}
[
  {
    "tool": "grep_corpus",
    "params": {
      "pattern": "effective July 3, 2025"
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolGrep}{Turn 6 tool returns}

# DOCUMENT ID: 0001104659-25-121934_21 (548 tokens) 
Company: Simply Good Foods Co
Filing Date: 2025-12-17
Form: DEF 14A
Chunk 21
---
, and our three most highly compensated executive officers for fiscal year 2025 other than our Chief Executive Officer and Chief Financial Officer. For fiscal year 2025, our NEOs were:

|  |  | GEOFF E.                              
 TANNER                                |  |  |  | CHRISTOPHER J.          
 BEALER                  |  |  |  | TIMOTHY R.                                    
 KRAFT                                         |  |  |  | AMY C.                                
 HELD                                  |  |  |  | RYAN A.                 
 THOMAS                  |  |  |  | SHAUN P.                       
 MARA                           |  |
|  |  | President and Chief Executive Officer |  |  |  | Chief Financial Officer |  |  |  | Chief Legal and Corporate Development Officer |  |  |  | SVP and Chief Human Resources Officer |  |  |  | SVP and General         
 Manager Atkins and OWYN |  |  |  | Former Chief Financial Officer |  |

Mr. Bealer became an NEO for the first time in fiscal year 2025. Mr. Bealer was hired on March 31, 2025. Mr. Mara retired as our Chief Financial Officer and resigned effective July 3, 2025. Mr. Mara's executive compensation is outlined further in the compensation tables beginning on page 54 but is otherwise not discussed with other NEOs except where noted. Executive Summary Our compensation program for our NEOs and other executive officers is designed to meet the following primary objectives:

|  |  | Management Development and Continuity.                                                                                                                                                                                                   
 Attract, retain and motivate individuals of superior ability and managerial talent to develop, grow and manage our business by offering competitive compensation opportunities with both short-term and significant long-term components |  |  |  | Pay for Performance.                                                                                                                                                                                                                                               
 Align executive officer compensation with the achievement of our short- and long-term corporate strategies and business objectives, along with the long-term interests of our stockholders through the use of performance-based and variable compensation elements |  |  |  | Long-Term Focus on Stockholder Value.                                                                                                                                                         
 Align executives with stockholder value creation by delivering a significant portion of our executive officers' compensation in the form of equity-based awards that vest over multiple years |  |

We believe compensation should be structured to ensure that a significant portion of the total compensation opportunity for our NEOs is directly related to our performance and other factors that directly and indirectly influence stockholder value. The

# DOCUMENT ID: 0001104659-25-121934_42 (549 tokens) 
Company: Simply Good Foods Co
Filing Date: 2025-12-17
Form: DEF 14A
Chunk 42
---
 |  |  |                                            |  | 5,052 |  |  |

(6) Mr. Bealer became an NEO for the first time in fiscal year 2025 upon being named our Chief Financial Officer effective July 3, 2025. Mr. Bealer was hired on March 31, 2025. (7) Mr. Mara resigned as our Chief Financial Officer effective July 3, 2025.

2026 Proxy Statement55

TABLE OF CONTENTS Grants of Plan-Based Awards Table The following table sets forth information regarding plan-based awards granted to our NEOs during fiscal year 2025. See "Narrative Disclosure to Summary Compensation Table and Grants of Plan-Based Awards Table," below for information with respect to vesting dates.

|  | Name                 |  |  | AwardDescription |  |          | ApprovalDate |   |   |   |  |          | GrantDate  |   |   |   |  |  | Estimated FuturePayouts UnderNon-EquityIncentive Plan Awards(1) |   |         |   |   |   |           |   |         |   |   |   |            |   |           |   |  |      | Estimated FuturePayouts UnderEquityIncentive Plan Awards(2) |   |   |   |   |        |   |   |   |   |   |        |   |   |   |   |  |       | All OtherStockAwards:Number ofShares ofStock orUnits(#) |   |   |   |  |       | All OtherOptionAwards:Number ofSecuritiesUnderlyingOptions(#) |   |   |   |  |      | Exerciseor BasePrice ofOptionAwards($) |   |   |   |  |          | GrantDateFairValue ofStockandOptionAwards($)(3) |   |   |   |  |
|  | Threshold($)         |   |   |                  |  |          | Target($)    |   |   |   |  |          | Maximum($) |   |   |   |  |  | Threshold(#)                                                    |   |         |   |  |  | Target(#) |   |         |   |  |  | Maximum(#) |   |           |   |  |       |                                                             |   |   |   |   |        |   |   |   |   |   |        |

# DOCUMENT ID: 0001104659-25-053287_0 (537 tokens) 
Company: Simply Good Foods Co
Filing Date: 2025-05-28
Form: 8-K
Item: Item 5.02
Chunk 0
---
Item 5.02

Departure of Directors or Certain Officers; Election of Directors; Appointment of Certain Officers; Compensatory Arrangements of Certain Officers.

Appointment of New CFO

In connection with the previously announced Chief Financial Officer
transition, on May 23, 2025, The Simply Good Foods Company (the " Company") appointed Christopher J. Bealer as the Company's
Chief Financial Officer effective July 3, 2025. Mr. Bealer is currently serving as the Company's Senior Vice President,
Finance having joined the Company on April 1, 2025. As Chief Financial Officer, Mr. Bealer will continue to report to Geoff
E. Tanner, the Company's President and Chief Executive Officer.

Mr. Bealer, age 48, has almost 23 years of experience in consumer-packaged
goods and consumer durables in North America and Global markets. Mr. Bealer was most recently EVP Corporate Controller at Reckitt
Benckiser Group PLC (" Reckitt") from March 2024 to March 31, 2025, and CFO Health at Reckitt from April 2021
to February 2024. In his EVP Corporate Controller role with Reckitt, Mr. Bealer led a global team of over 600 employees accountable
for global controls, financial shared services, group reporting and accounting, as well as leading the functional operating model transformation.
Prior to his roles at Reckitt, Mr. Bealer served as Vice President and CFO Europe, Middle East and Africa Region from August 2018
to March 2021 and Vice President and CFO North America Region from November 2015 to August 2018 for Whirlpool Corporation.
Earlier in his career, Bealer held various finance roles at Big Heart Pet Brands, Del Monte Foods, and H. J. Heinz Company. Mr. Bealer
is a Certified Public Accountant in the United States and a qualified Associate Chartered Accountant in the United Kingdom. Mr. Bealer
received his Bachelor's Degree with Honours - Geography from the University of Birmingham, U. K.

As Chief Financial Officer, Mr. Bealer will receive an initial
annual base salary of $500,000 (" Base Salary"), subject to future adjustment by the Company. Mr. Bealer will be eligible
to participate in the Company's long term equity incentive program, with an annual target opportunity of one hundred fifty percent
(150%) of his Base Salary.

In addition, Mr.

# DOCUMENT ID: 0001104659-25-006698_0 (387 tokens) 
Company: Simply Good Foods Co
Filing Date: 2025-01-28
Form: 8-K
Item: Item 5.02
Chunk 0
---
Item 5.02 Departure of Directors or Certain Officers; Election of
Directors; Appointment of Certain Officers; Compensatory Arrangements of Certain Officers.

(b) On January 27, 2025, Shaun P. Mara, Chief Financial Officer
of The Simply Good Foods Company (the " Company"), notified the Company of his decision to retire effective July 3, 2025.
Mr. Mara will remain as Chief Financial Officer through the date of his retirement, at which time he will resign from all positions
with the Company and its subsidiaries.

In connection with Mr. Mara's retirement, on January 28,
2025, the Company announced the hiring of Mr. Christopher J. Bealer as Senior Vice President of Finance of the Company, as of
April 1, 2025. Mr. Bealer is expected to succeed Mr. Mara as Chief Financial Officer upon Mr. Mara's retirement
on July 3, 2025.

Mr. Bealer has almost 23 years of experience in consumer packaged
goods and consumer durables in North America and global markets. In his most recent executive leadership position as EVP Corporate Controller
at Reckitt Benckiser Group PLC (" Reckitt"), Mr. Bealer leads a global team of over 600 employees accountable for global
controls, financial shared services, group reporting and accounting, as well as leading the functional operating model transformation.
Prior to his current and prior roles at Reckitt, Mr. Bealer served as Regional CFO for Whirlpool Corporation for both the North American
and Europe, Middle East and Africa (EMEA) businesses. He also held finance positions at Big Heart Pet Brands, Del Monte Foods, and H. J.
Heinz Company.

# DOCUMENT ID: 0001514281-25-000086_100 (549 tokens) 
Company: TPG Mortgage Investment Trust, Inc.
Filing Date: 2025-08-05
Form: 10-Q
Item: Part I, Item 1
Chunk 100
---
457 8.71 %10.69 %0.425/6/202577.22 %NYLoan D (7)22,204 (168)22,036 112 - 22,148 7.89 %8.73 %0.688/6/202542.50 %CTTotal$67,204 $(563)$66,641 $364 $- $67,005 8.44 %10.04 %0.5063.69 %(1)The Company has the contractual right to receive a balloon payment for each loan.(2)Each commercial loan investment is a first mortgage loan.(3)The weighted average yields are calculated based on the amortized cost of the underlying loans. (4)Actual maturities of commercial loans may be shorter or longer than stated contractual maturities. Maturities are affected by prepayments of principal. (5)Represents the LTV at acquisition. The total LTV on commercial loans is presented based on fair value.(6)Loans A, B, and C have a floating rate coupon equal to 4.20% plus one-month SOFR and are collateralized by hotels. The borrower for Loans A, B and C is currently in default. In May 2025, the administrative agent on behalf of the lenders (including the Company) of Loans A, B and C entered into short-term forbearance agreements with the borrower, which were subsequently terminated effective July 3, 2025. For the three months ended June 30, 2025, these loans were placed on non-accrual status. The borrower for such loans is in the process of selling the hotels collateralizing the loans; however, no assurances can be made that any such sale will be completed on the terms contemplated or at all. The lender on the Company's financing arrangements on Loans A, B and C is permitted to request a full repayment of the debt with respect to such assets. The Company does not currently expect its lender to request a full repayment of the related outstanding financing arrangements. 

(7)Loan D has a floating rate coupon equal to 3.38% plus one-month SOFR and is collateralized by a retail property. Loan D has a current payment status. The maturity date represents the last possible extension option.

16

AG Mortgage Investment Trust Inc. and SubsidiariesNotes to Consolidated Financial Statements (Unaudited)June 30
[Context: 8326/30720]
\end{trajectorylisting}

\subsubsection*{Turn 7: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolNeutral}{Turn 7 reasoning}
We just used grep on the exact effective-date phrase and found several confirmatory documents, mostly SEC filings for the same company. What isn't working is the current search angle: after picking up the exact phrase, there are few new sources left, and the solution is already essentially known. The gap is just backtracking from the last search: we should curate the new grep results before ending, since we have fresh evidence now.
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 7 tool call}
[
  {
    "tool": "curate",
    "params": {
      "add_ids": [
        "0001104659-25-121934_21",
        "0001104659-25-121934_42",
        "0001104659-25-006698_0"
      ],
      "importance": {
        "0001104659-25-006698_0": "high",
        "0001104659-25-121934_21": "high",
        "0001104659-25-121934_42": "high"
      }
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 7 tool returns}
Curated set updated (9/30): 0001104659-25-006698_0[high], 0001104659-25-053287_0[high], 0001104659-25-121934_20[high], 0001104659-25-121934_21[high], 0001104659-25-121934_42[high], 0000909832-25-000101_19[fair], 0001364954-25-000039_57[fair], 0001673985-25-000053_24[fair], 0001530950-25-000260_18[low]
\end{trajectorylisting}

\subsubsection*{Turn 8: \CaseTool{toolCurate}{curate}}
\begin{trajectorylisting}{toolNeutral}{Turn 8 reasoning}
We have direct SEC filings of the single company that document both the spring senior-vice-president hire and the July retirement; the effective CFO transition date is clearly July 3, 2025. The last grep angle is exhausted, and the remaining task is to conclude search rather than find new sources. What isn't working is further searching because our evidence is already sufficient and exact-perspective queries are repeating the known company/final-date angle. The gap is only closing out with the most relevant documents properly curated; it would be better to preserve the exact filings than risk them being evicted.
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 8 tool call}
[
  {
    "tool": "curate",
    "params": {
      "doc_ids": [
        "0001104659-25-121934_21",
        "0001104659-25-121934_42"
      ],
      "remove_ids": [],
      "importance": {
        "0001104659-25-121934_21": "high",
        "0001104659-25-121934_42": "high"
      }
    }
  }
]
\end{trajectorylisting}

\begin{trajectorylisting}{toolCurate}{Turn 8 tool returns}
Curated set updated (9/30): 0001104659-25-006698_0[high], 0001104659-25-053287_0[high], 0001104659-25-121934_20[high], 0001104659-25-121934_21[high], 0001104659-25-121934_42[high], 0000909832-25-000101_19[fair], 0001364954-25-000039_57[fair], 0001673985-25-000053_24[fair], 0001530950-25-000260_18[low]
\end{trajectorylisting}


